Resurgence Analysis of Quantum Invariants of Seifert Fibered Homology Spheres

For a Seifert fibered homology sphere we show that the q-series Z-hat invariant introduced by Gukov, Pei, Putrov and Vafa is a resummation of the Ohtsuki serie. We show that for every even level k there exists a full asymptotic expansion of Z-hat for q tending to a certain k'th root of unity and in particular that the limit exists and is equal to the WRT quantum invariant. We show that the poles of the Borel transform of the Ohtsuki series coincide with the classical complex Chern-Simons values, which we further show classifies the corresponding components of the moduli space of flat SL(2, C)-connections.

==> bibo.tex <==
@ARTICLE{BodenCurtis2006,
	author = {{Boden}, Hans U. and {Curtis}, Cynthia L.},
	title = "{The SL(2,C) Casson invariant for Seifert fibered homology spheres and surgeries on twist knots}",
	journal = {arXiv Mathematics e-prints},
	keywords = {Mathematics - Geometric Topology, 57M27, 57M25, 57M05},
	year = 2006,
	month = feb,
	eid = {math/0602023},
	pages = {math/0602023},
	archivePrefix = {arXiv},
	eprint = {math/0602023},
	primaryClass = {math.GT},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2006math......2023B},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@phdthesis{williamelbaekmistegardQuantumInvariantsChernSimons2019,
	title = {Quantum {{Invariants}} and {{Chern}}-{{Simons Theory}}},
	author = {{Mistegård}, William Elbæk},
	year = {2019},
	school = {Aarhus University}
}


@ARTICLE{AndersenRes2020,
	title = {Resurgence Analysis of the WRT-TQFT, Online seminar https://sites.google.com/view/gaugesummerwithbv/home/abstracts#h.rcu9ixszi7xk},
	author = {{Andersen}, Jørgen Ellegaard},
	year = {2020},
	month = june,
}

@ARTICLE{MisteRes2020,
	title = {Quantum Modularity and Resurgence},
	author = {{Mistegård}, William Elbæk},
	year = {2020},
	month = may,
	adsurl={https://www.researchgate.net/publication/341574789_Quantum_Modularity_and_Resurgence},
}

@ARTICLE{Hiroyuki,
       author = {{Fuji}, Hiroyuki and {Iwaki}, Kohei and {Murakami}, Hitoshi and
         {Terashima}, Yuji},
        title = "{Witten-Reshetikhin-Turaev function for a knot in Seifert manifolds}",
      journal = {arXiv e-prints},
     keywords = {Mathematics - Geometric Topology, High Energy Physics - Theory, Mathematical Physics, 57K31, 57K16, 57K10},
         year = 2020,
        month = jul,
          eid = {arXiv:2007.15872},
        pages = {arXiv:2007.15872},
archivePrefix = {arXiv},
       eprint = {2007.15872},
 primaryClass = {math.GT},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv200715872F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@misc{garoufalidis2020resurgent,
    title={The resurgent structure of quantum knot invariants},
    author={Stavros Garoufalidis and Jie Gu and Marcos Marino},
    year={2020},
    eprint={2007.10190},
    archivePrefix={arXiv},
    primaryClass={hep-th}
}

@ARTICLE{hikami2003qseries,
	title={q-series and L-functions related to half-derivatives of the Andrews--Gordon identity},
	author={Kazuhiro Hikami},
	year={2003},
	eprint={math/0303250},
	archivePrefix={arXiv},
	primaryClass={math.NT}
}

@ARTICLE{2019arXiv190913002P,
	author = {{Park}, Sunghyuk},
	title = "{Higher rank $\hat{Z}$ and $F_K$}",
	journal = {arXiv e-prints},
	keywords = {Mathematics - Geometric Topology, High Energy Physics - Theory, Mathematical Physics, Mathematics - Quantum Algebra},
	year = "2019",
	month = "Sep",
	eid = {arXiv:1909.13002},
	pages = {arXiv:1909.13002},
	archivePrefix = {arXiv},
	eprint = {1909.13002},
	primaryClass = {math.GT},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190913002P},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ChungHJ18,
	author = {{Chung}, Hee-Joong},
	title = "{BPS Invariants for Seifert Manifolds}",
	journal = {arXiv e-prints},
	keywords = {High Energy Physics - Theory, Mathematics - Geometric Topology, Mathematics - Number Theory},
	year = "2018",
	month = "Nov",
	eid = {arXiv:1811.08863},
	pages = {arXiv:1811.08863},
	archivePrefix = {arXiv},
	eprint = {1811.08863},
	primaryClass = {hep-th},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2018arXiv181108863C},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019arXiv191108456C,
	author = {{Chun}, Sungbong and {Gukov}, Sergei and {Park}, Sunghyuk and
	{Sopenko}, Nikita},
	title = "{3d-3d correspondence for mapping tori}",
	journal = {arXiv e-prints},
	keywords = {High Energy Physics - Theory, Mathematics - Geometric Topology, Mathematics - Quantum Algebra},
	year = "2019",
	month = "Nov",
	eid = {arXiv:1911.08456},
	pages = {arXiv:1911.08456},
	archivePrefix = {arXiv},
	eprint = {1911.08456},
	primaryClass = {hep-th},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv191108456C},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@misc{BKM17,
	title={Higher depth quantum modular forms, multiple Eichler integrals, and $\frak{sl}_3$ false theta functions},
	author={Kathrin Bringmann and Jonas Kaszian and Antun Milas},
	year={2017},
	eprint={1704.06891},
	archivePrefix={arXiv},
	primaryClass={math.NT}
}

@ARTICLE{BMA18,
	author = {{Bringmann}, Kathrin and {Mahlburg}, Karl and {Milas}, Antun},
	title = "{Quantum modular forms and plumbing graphs of 3-manifolds}",
	journal = {arXiv e-prints},
	keywords = {Mathematics - Quantum Algebra, Mathematics - Number Theory, 11F27, 11F37, 14N35, 57M27, 57R56},
	year = "2018",
	month = "Oct",
	eid = {arXiv:1810.05612},
	pages = {arXiv:1810.05612},
	archivePrefix = {arXiv},
	eprint = {1810.05612},
	primaryClass = {math.QA},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2018arXiv181005612B},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{BMA19june,
	author = {{Bringmann}, Kathrin and {Mahlburg}, Karl and {Milas}, Antun},
	title = "{Higher depth quantum modular forms and plumbed $3$-manifolds}",
	journal = {arXiv e-prints},
	keywords = {Mathematics - Number Theory, Mathematics - Geometric Topology, Mathematics - Quantum Algebra, 11F27, 11F37, 14N35, 57M27, 57R56},
	year = "2019",
	month = "Jun",
	eid = {arXiv:1906.10722},
	pages = {arXiv:1906.10722},
	archivePrefix = {arXiv},
	eprint = {1906.10722},
	primaryClass = {math.NT},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190610722B},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article {Brieskorn70,
    AUTHOR = {Brieskorn, Egbert},
     TITLE = {Die {M}onodromie der isolierten {S}ingularit\"{a}ten von
              {H}yperfl\"{a}chen},
   JOURNAL = {Manuscripta Math.},
  FJOURNAL = {Manuscripta Mathematica},
    VOLUME = {2},
      YEAR = {1970},
     PAGES = {103--161},
      ISSN = {0025-2611},
   MRCLASS = {57.60},
  MRNUMBER = {0267607},
MRREVIEWER = {J. P. Levine},
       DOI = {10.1007/BF01155695},
       URL = {https://doi.org/10.1007/BF01155695},
}

@article {Jeffrey94,
    AUTHOR = {Jeffrey, Lisa C.},
     TITLE = {Extended moduli spaces of flat connections on {R}iemann
              surfaces},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {298},
      YEAR = {1994},
    NUMBER = {4},
     PAGES = {667--692},
      ISSN = {0025-5831},
   MRCLASS = {58D27 (14H55 32G13 58F05)},
  MRNUMBER = {1268599},
MRREVIEWER = {William Goldman},
       DOI = {10.1007/BF01459756},
       URL = {https://doi.org/10.1007/BF01459756},
}

@book {Akbulut16,
    AUTHOR = {Akbulut, Selman},
     TITLE = {4-manifolds},
    SERIES = {Oxford Graduate Texts in Mathematics},
    VOLUME = {25},
 PUBLISHER = {Oxford University Press, Oxford},
      YEAR = {2016},
     PAGES = {xii+262},
      ISBN = {978-0-19-878486-9},
   MRCLASS = {57N13 (57-02)},
  MRNUMBER = {3559604},
MRREVIEWER = {Jonathan D. Williams},
       DOI = {10.1093/acprof:oso/9780198784869.001.0001},
       URL = {https://doi.org/10.1093/acprof:oso/9780198784869.001.0001},
}

@ARTICLE{BDSSU2015,
       author = {{Behtash}, Alireza and {Dunne}, Gerald V. and {Schaefer}, Thomas and
         {Sulejmanpasic}, Tin and {Unsal}, Mithat},
        title = "{Toward Picard-Lefschetz Theory of Path Integrals, Complex Saddles and Resurgence}",
      journal = {arXiv e-prints},
     keywords = {High Energy Physics - Theory},
         year = "2015",
        month = "Oct",
          eid = {arXiv:1510.03435},
        pages = {arXiv:1510.03435},
archivePrefix = {arXiv},
       eprint = {1510.03435},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015arXiv151003435B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book {Pham67,
    AUTHOR = {Pham, F.},
     TITLE = {Introduction \`a l'\'{e}tude topologique des singularit\'{e}s de
              {L}andau},
    SERIES = {M\'{e}morial des Sciences Math\'{e}matiques, Fasc. 164},
 PUBLISHER = {Gauthier-Villars \'{E}diteur, Paris},
      YEAR = {1967},
     PAGES = {ii+142},
   MRCLASS = {57.50},
  MRNUMBER = {0229263},
MRREVIEWER = {H. Suzuki},
}

@ARTICLE{Gukov10,
       author = {{Gukov}, Sergei},
        title = "{Quantization via Mirror Symmetry}",
      journal = {arXiv e-prints},
     keywords = {High Energy Physics - Theory, Mathematical Physics, Mathematics - Algebraic Geometry, Mathematics - Quantum Algebra},
         year = "2010",
        month = "Nov",
          eid = {arXiv:1011.2218},
        pages = {arXiv:1011.2218},
archivePrefix = {arXiv},
       eprint = {1011.2218},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010arXiv1011.2218G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article {GukovWitten13,
    AUTHOR = {Gukov, Sergei and Witten, Edward},
     TITLE = {Branes and quantization},
   JOURNAL = {Adv. Theor. Math. Phys.},
  FJOURNAL = {Advances in Theoretical and Mathematical Physics},
    VOLUME = {13},
      YEAR = {2009},
    NUMBER = {5},
     PAGES = {1445--1518},
      ISSN = {1095-0761},
   MRCLASS = {81S10 (53D50 53D55 81T30 81T45)},
  MRNUMBER = {2672467},
MRREVIEWER = {Douglas J. Smith},
       URL = {http://projecteuclid.org/euclid.atmp/1282054099},
}

@article {Gualtieri11,
    AUTHOR = {Gualtieri, Marco},
     TITLE = {Generalized complex geometry},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {174},
      YEAR = {2011},
    NUMBER = {1},
     PAGES = {75--123},
      ISSN = {0003-486X},
   MRCLASS = {53D18},
  MRNUMBER = {2811595},
MRREVIEWER = {Frederik Witt},
       DOI = {10.4007/annals.2011.174.1.3},
       URL = {https://doi.org/10.4007/annals.2011.174.1.3},
}

@article {Hitchin03,
    AUTHOR = {Hitchin, Nigel},
     TITLE = {Generalized {C}alabi-{Y}au manifolds},
   JOURNAL = {Q. J. Math.},
  FJOURNAL = {The Quarterly Journal of Mathematics},
    VOLUME = {54},
      YEAR = {2003},
    NUMBER = {3},
     PAGES = {281--308},
      ISSN = {0033-5606},
   MRCLASS = {32Q25 (14J32 53C29 53C56)},
  MRNUMBER = {2013140},
MRREVIEWER = {Richard P. Thomas},
       DOI = {10.1093/qjmath/54.3.281},
       URL = {https://doi.org/10.1093/qjmath/54.3.281},
}

@article {BriniEynardMarino12,
    AUTHOR = {Brini, Andrea and Eynard, Bertrand and Mari\~{n}o, Marcos},
     TITLE = {Torus knots and mirror symmetry},
   JOURNAL = {Ann. Henri Poincar\'{e}},
  FJOURNAL = {Annales Henri Poincar\'{e}. A Journal of Theoretical and
              Mathematical Physics},
    VOLUME = {13},
      YEAR = {2012},
    NUMBER = {8},
     PAGES = {1873--1910},
      ISSN = {1424-0637},
   MRCLASS = {81T45 (14J33 57M27)},
  MRNUMBER = {2994763},
MRREVIEWER = {Arkady L. Kholodenko},
       DOI = {10.1007/s00023-012-0171-2},
       URL = {https://doi.org/10.1007/s00023-012-0171-2},
}

@ARTICLE{CostinDunne19,
       author = {{Costin}, Ovidiu and {Dunne}, Gerald V.},
        title = "{Resurgent Extrapolation: Rebuilding a Function from Asymptotic Data. Painleve I}",
      journal = {arXiv e-prints},
     keywords = {High Energy Physics - Theory, Mathematical Physics},
         year = "2019",
        month = "Apr",
          eid = {arXiv:1904.11593},
        pages = {arXiv:1904.11593},
archivePrefix = {arXiv},
       eprint = {1904.11593},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190411593C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article {Pham65,
    AUTHOR = {Pham, Fr\'{e}d\'{e}ric},
     TITLE = {Formules de {P}icard-{L}efschetz g\'{e}n\'{e}ralis\'{e}es et ramification
              des int\'{e}grales},
   JOURNAL = {Bull. Soc. Math. France},
  FJOURNAL = {Bulletin de la Soci\'{e}t\'{e} Math\'{e}matique de France},
    VOLUME = {93},
      YEAR = {1965},
     PAGES = {333--367},
      ISSN = {0037-9484},
   MRCLASS = {14.55 (32.44)},
  MRNUMBER = {0195868},
MRREVIEWER = {M. F. Atiyah},
       URL = {http://www.numdam.org/item?id=BSMF_1965__93__333_0},
}

@article {Atiyah87,
    AUTHOR = {Atiyah, Michael},
     TITLE = {The logarithm of the {D}edekind {$\eta$}-function},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {278},
      YEAR = {1987},
    NUMBER = {1-4},
     PAGES = {335--380},
      ISSN = {0025-5831},
   MRCLASS = {58G10 (11F20)},
  MRNUMBER = {909232},
MRREVIEWER = {Friedbert Pr\"{u}fer},
       DOI = {10.1007/BF01458075},
       URL = {https://doi.org/10.1007/BF01458075},
}

@article {KirbyMelvin94,
    AUTHOR = {Kirby, Robion and Melvin, Paul},
     TITLE = {Dedekind sums, {$\mu$}-invariants and the signature cocycle},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {299},
      YEAR = {1994},
    NUMBER = {2},
     PAGES = {231--267},
      ISSN = {0025-5831},
   MRCLASS = {11F20 (57M25 57N12 57N13)},
  MRNUMBER = {1275766},
MRREVIEWER = {Terry Lawson},
       DOI = {10.1007/BF01459782},
       URL = {https://doi.org/10.1007/BF01459782},
}

@article {KB93,
    AUTHOR = {Kania-Bartoszynska, Joanna},
     TITLE = {Examples of different {$3$}-manifolds with the same invariants
              of {W}itten and {R}eshetikhin-{T}uraev},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {32},
      YEAR = {1993},
    NUMBER = {1},
     PAGES = {47--54},
      ISSN = {0040-9383},
   MRCLASS = {57N10},
  MRNUMBER = {1204405},
MRREVIEWER = {Bruno P. Zimmermann},
       DOI = {10.1016/0040-9383(93)90036-U},
       URL = {https://doi.org/10.1016/0040-9383(93)90036-U},
}

@article {Lickorish93,
    AUTHOR = {Lickorish, W. B. R.},
     TITLE = {Distinct {$3$}-manifolds with all {${\rm SU}(2)_q$} invariants
              the same},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {117},
      YEAR = {1993},
    NUMBER = {1},
     PAGES = {285--292},
      ISSN = {0002-9939},
   MRCLASS = {57N10 (17B37 57M25)},
  MRNUMBER = {1129882},
MRREVIEWER = {Louis H. Kauffman},
       DOI = {10.2307/2159729},
       URL = {https://doi.org/10.2307/2159729},
}

@book {Newstead78,
    AUTHOR = {Newstead, P. E.},
     TITLE = {Introduction to moduli problems and orbit spaces},
    SERIES = {Tata Institute of Fundamental Research Lectures on Mathematics
              and Physics},
    VOLUME = {51},
 PUBLISHER = {Tata Institute of Fundamental Research, Bombay; by the Narosa
              Publishing House, New Delhi},
      YEAR = {1978},
     PAGES = {vi+183},
      ISBN = {0-387-08851-2},
   MRCLASS = {14-02 (14D20)},
  MRNUMBER = {546290},
MRREVIEWER = {G. Horrocks},
}

@article {BlanchetCostantinoGeer18,
    AUTHOR = {Blanchet, Christian and Costantino, Francesco and Geer, Nathan
              and Patureau-Mirand, Bertrand},
     TITLE = {Non-semi-simple {TQFT}s, {R}eidemeister torsion and
              {K}ashaev's invariants},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {301},
      YEAR = {2016},
     PAGES = {1--78},
      ISSN = {0001-8708},
   MRCLASS = {57R56 (57M27 57Q10)},
  MRNUMBER = {3539369},
MRREVIEWER = {Daniel D. Moskovich},
       DOI = {10.1016/j.aim.2016.06.003},
       URL = {https://doi.org/10.1016/j.aim.2016.06.003},
}

@incollection {Lurie09,
    AUTHOR = {Lurie, Jacob},
     TITLE = {On the classification of topological field theories},
 BOOKTITLE = {Current developments in mathematics, 2008},
     PAGES = {129--280},
 PUBLISHER = {Int. Press, Somerville, MA},
      YEAR = {2009},
   MRCLASS = {57R56 (18D10 18G30 57R15 57R75)},
  MRNUMBER = {2555928},
MRREVIEWER = {Julia Bergner},
}

@article {Freed13,
    AUTHOR = {Freed, Daniel S.},
     TITLE = {The cobordism hypothesis},
   JOURNAL = {Bull. Amer. Math. Soc. (N.S.)},
  FJOURNAL = {American Mathematical Society. Bulletin. New Series},
    VOLUME = {50},
      YEAR = {2013},
    NUMBER = {1},
     PAGES = {57--92},
      ISSN = {0273-0979},
   MRCLASS = {57-02 (57R56)},
  MRNUMBER = {2994995},
       DOI = {10.1090/S0273-0979-2012-01393-9},
       URL = {https://doi.org/10.1090/S0273-0979-2012-01393-9},
}

@article {BaezDolan95,
    AUTHOR = {Baez, John C. and Dolan, James},
     TITLE = {Higher-dimensional algebra and topological quantum field
              theory},
   JOURNAL = {J. Math. Phys.},
  FJOURNAL = {Journal of Mathematical Physics},
    VOLUME = {36},
      YEAR = {1995},
    NUMBER = {11},
     PAGES = {6073--6105},
      ISSN = {0022-2488},
   MRCLASS = {18D05 (55P42 57R57)},
  MRNUMBER = {1355899},
       DOI = {10.1063/1.531236},
       URL = {https://doi.org/10.1063/1.531236},
}

@ARTICLE{BDSV15,
       author = {{Bartlett}, Bruce and {Douglas}, Christopher L. and
         {Schommer-Pries}, Christopher J. and {Vicary}, Jamie},
        title = "{Modular categories as representations of the 3-dimensional bordism 2-category}",
      journal = {arXiv e-prints},
     keywords = {Mathematics - Algebraic Topology, Mathematics - Category Theory, Mathematics - Geometric Topology, Mathematics - Quantum Algebra, Mathematics - Representation Theory},
         year = "2015",
        month = "Sep",
          eid = {arXiv:1509.06811},
        pages = {arXiv:1509.06811},
archivePrefix = {arXiv},
       eprint = {1509.06811},
 primaryClass = {math.AT},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015arXiv150906811B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article {Bar-NatanGaroufalidis,
    AUTHOR = {Bar-Natan, Dror and Garoufalidis, Stavros},
     TITLE = {On the {M}elvin-{M}orton-{R}ozansky conjecture},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {125},
      YEAR = {1996},
    NUMBER = {1},
     PAGES = {103--133},
      ISSN = {0020-9910},
   MRCLASS = {57M25 (17B99)},
  MRNUMBER = {1389962},
MRREVIEWER = {Zhenghan Wang},
       DOI = {10.1007/s002220050070},
       URL = {https://doi.org/10.1007/s002220050070},
}

@article {GaroufalidisLe05,
    AUTHOR = {Garoufalidis, Stavros and L\^{e}, Thang T. Q.},
     TITLE = {The colored {J}ones function is {$q$}-holonomic},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry and Topology},
    VOLUME = {9},
      YEAR = {2005},
     PAGES = {1253--1293},
      ISSN = {1465-3060},
   MRCLASS = {57M27 (33D15 33F10 57M25 57N10)},
  MRNUMBER = {2174266},
MRREVIEWER = {Vladimir V. Tchernov},
       DOI = {10.2140/gt.2005.9.1253},
       URL = {https://doi.org/10.2140/gt.2005.9.1253},
}

@ARTICLE{Schiappa18,
       author = {{Aniceto}, In{\^e}s and {Ba{\textcommabelow s}ar}, G{\"o}k{\c{c}}e and
         {Schiappa}, Ricardo},
        title = "{A Primer on Resurgent Transseries and Their Asymptotics}",
      journal = {arXiv e-prints},
     keywords = {High Energy Physics - Theory, High Energy Physics - Lattice, High Energy Physics - Phenomenology, Mathematical Physics, Quantum Physics},
         year = "2018",
        month = "Feb",
          eid = {arXiv:1802.10441},
        pages = {arXiv:1802.10441},
archivePrefix = {arXiv},
       eprint = {1802.10441},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018arXiv180210441A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{BethashDunneSchaefterSulejmanpasicUnsal15,
       author = {{Behtash}, Alireza and {Dunne}, Gerald V. and {Schaefer}, Thomas and
         {Sulejmanpasic}, Tin and {Unsal}, Mithat},
        title = "{Toward Picard-Lefschetz Theory of Path Integrals, Complex Saddles and Resurgence}",
      journal = {arXiv e-prints},
     keywords = {High Energy Physics - Theory},
         year = "2015",
        month = "Oct",
          eid = {arXiv:1510.03435},
        pages = {arXiv:1510.03435},
archivePrefix = {arXiv},
       eprint = {1510.03435},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015arXiv151003435B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ioos18,
       author = {{Ioos}, Louis},
        title = "{Quantization of symplectic maps and Witten's asymptotic conjecture}",
      journal = {arXiv e-prints},
     keywords = {Mathematics - Differential Geometry, Mathematical Physics, Mathematics - Geometric Topology, Mathematics - Symplectic Geometry},
         year = "2018",
        month = "Oct",
          eid = {arXiv:1810.03589},
        pages = {arXiv:1810.03589},
archivePrefix = {arXiv},
       eprint = {1810.03589},
 primaryClass = {math.DG},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018arXiv181003589I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GukovCiprian19,
       author = {{Gukov}, Sergei and {Manolescu}, Ciprian},
        title = "{A two-variable series for knot complements}",
      journal = {arXiv e-prints},
     keywords = {Mathematics - Geometric Topology, High Energy Physics - Theory, Mathematical Physics, Mathematics - Quantum Algebra, 57M27, 57M25},
         year = "2019",
        month = "Apr",
          eid = {arXiv:1904.06057},
        pages = {arXiv:1904.06057},
archivePrefix = {arXiv},
       eprint = {1904.06057},
 primaryClass = {math.GT},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190406057G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{HikamiLovejoy14,
       author = {{Hikami}, Kazuhiro and {Lovejoy}, Jeremy},
        title = "{Torus knots and quantum modular forms}",
      journal = {arXiv e-prints},
     keywords = {Mathematics - Number Theory, Mathematics - Quantum Algebra},
         year = "2014",
        month = "Sep",
          eid = {arXiv:1409.6243},
        pages = {arXiv:1409.6243},
archivePrefix = {arXiv},
       eprint = {1409.6243},
 primaryClass = {math.NT},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014arXiv1409.6243H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hikami05c,
       author = {{Hikami}, K.},
        title = "{Mock (False) Theta Functions as Quantum Invariants}",
      journal = {Regular and Chaotic Dynamics},
     keywords = {Mathematical Physics},
         year = "2005",
        month = "Jan",
       volume = {10},
       number = {4},
        pages = {509},
          doi = {10.1070/RD2005v010n04ABEH000328},
archivePrefix = {arXiv},
       eprint = {math-ph/0506073},
 primaryClass = {math-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005RCD....10..509H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hikami06q,
       author = {{Hikami}, Kazuhiro},
        title = "{Quantum invariants, modular forms, and lattice points II}",
      journal = {Journal of Mathematical Physics},
     keywords = {11.15.-q, 02.30.Rz, 11.30.Ly, Gauge field theories, Integral equations, Other internal and higher symmetries, Mathematics - Quantum Algebra, Mathematics - Geometric Topology},
         year = "2006",
        month = "Oct",
       volume = {47},
       number = {10},
        pages = {102301-102301},
          doi = {10.1063/1.2349484},
archivePrefix = {arXiv},
       eprint = {math/0604091},
 primaryClass = {math.QA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006JMP....47j2301H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article {Hikami05b,
    AUTHOR = {Hikami, Kazuhiro},
     TITLE = {Quantum invariant, modular form, and lattice points},
   JOURNAL = {Int. Math. Res. Not.},
  FJOURNAL = {International Mathematics Research Notices},
      YEAR = {2005},
    NUMBER = {3},
     PAGES = {121--154},
      ISSN = {1073-7928},
   MRCLASS = {11F23 (11F37 11P21 57M27 58J28)},
  MRNUMBER = {2130240},
MRREVIEWER = {Ruth Lawrence},
       DOI = {10.1155/IMRN.2005.121},
       URL = {https://doi.org/10.1155/IMRN.2005.121},
}

@incollection {Kapranov95,
    AUTHOR = {Kapranov, M. M.},
     TITLE = {Analogies between the {L}anglands correspondence and
              topological quantum field theory},
 BOOKTITLE = {Functional analysis on the eve of the 21st century, {V}ol. 1
              ({N}ew {B}runswick, {NJ}, 1993)},
    SERIES = {Progr. Math.},
    VOLUME = {131},
     PAGES = {119--151},
 PUBLISHER = {Birkh\"{a}user Boston, Boston, MA},
      YEAR = {1995},
   MRCLASS = {11G45 (11R39 14A20 19F05 58D29)},
  MRNUMBER = {1373001},
MRREVIEWER = {I. Dolgachev},
}

@article {FreedGompf91,
    AUTHOR = {Freed, Daniel S. and Gompf, Robert E.},
     TITLE = {Computer calculation of {W}itten's {$3$}-manifold invariant},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {141},
      YEAR = {1991},
    NUMBER = {1},
     PAGES = {79--117},
      ISSN = {0010-3616},
   MRCLASS = {57N10 (11L03 57M25 58D30 58G26 81T13 81T40)},
  MRNUMBER = {1133261},
MRREVIEWER = {Ronald J. Stern},
       URL = {http://projecteuclid.org/euclid.cmp/1104248195},
}

@ARTICLE{Bruno16,
       author = {{Martelli}, Bruno},
        title = "{An Introduction to Geometric Topology}",
      journal = {arXiv e-prints},
     keywords = {Mathematics - Geometric Topology, Mathematics - Differential Geometry},
         year = "2016",
        month = "Oct",
          eid = {arXiv:1610.02592},
        pages = {arXiv:1610.02592},
archivePrefix = {arXiv},
       eprint = {1610.02592},
 primaryClass = {math.GT},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016arXiv161002592M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article {FennRourke79,
    AUTHOR = {Fenn, Roger and Rourke, Colin},
     TITLE = {On {K}irby's calculus of links},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {18},
      YEAR = {1979},
    NUMBER = {1},
     PAGES = {1--15},
      ISSN = {0040-9383},
   MRCLASS = {57M25},
  MRNUMBER = {528232},
MRREVIEWER = {Wilbur Whitten},
       DOI = {10.1016/0040-9383(79)90010-7},
       URL = {https://doi.org/10.1016/0040-9383(79)90010-7},
}

@article {KirkKlassen93,
    AUTHOR = {Kirk, Paul and Klassen, Eric},
     TITLE = {Chern-{S}imons invariants of {$3$}-manifolds decomposed along
              tori and the circle bundle over the representation space of
              {$T^2$}},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {153},
      YEAR = {1993},
    NUMBER = {3},
     PAGES = {521--557},
      ISSN = {0010-3616},
   MRCLASS = {57N10 (57R19)},
  MRNUMBER = {1218931},
MRREVIEWER = {Dave Auckly},
       URL = {http://projecteuclid.org/euclid.cmp/1104252787},
}

@article {Kirby78,
    AUTHOR = {Kirby, Robion},
     TITLE = {A calculus for framed links in {$S^{3}$}},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {45},
      YEAR = {1978},
    NUMBER = {1},
     PAGES = {35--56},
      ISSN = {0020-9910},
   MRCLASS = {57A10 (55A25)},
  MRNUMBER = {0467753},
MRREVIEWER = {Roger Fenn},
       DOI = {10.1007/BF01406222},
       URL = {https://doi.org/10.1007/BF01406222},
}

@book {Lee13,
    AUTHOR = {Lee, John M.},
     TITLE = {Introduction to smooth manifolds},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {218},
   EDITION = {Second},
 PUBLISHER = {Springer, New York},
      YEAR = {2013},
     PAGES = {xvi+708},
      ISBN = {978-1-4419-9981-8},
   MRCLASS = {58-01 (53-01 57-01)},
  MRNUMBER = {2954043},
}

@incollection {Morton92,
    AUTHOR = {Morton, H. R.},
     TITLE = {Invariants of links and {$3$}-manifolds from skein theory and
              from quantum groups},
 BOOKTITLE = {Topics in knot theory ({E}rzurum, 1992)},
    SERIES = {NATO Adv. Sci. Inst. Ser. C Math. Phys. Sci.},
    VOLUME = {399},
     PAGES = {107--155},
 PUBLISHER = {Kluwer Acad. Publ., Dordrecht},
      YEAR = {1993},
   MRCLASS = {57M25 (57N10)},
  MRNUMBER = {1257908},
}

@article{KoldHansen01,
       author = {Kold Hansen, Soren},
        title = {Reshetikhin-Turaev invariants of Seifert 3-manifolds and a rational surgery formula},
      journal = {arXiv Mathematics e-prints},
     keywords = {Mathematics - Geometric Topology, Mathematics - Quantum Algebra, 57M27, 17B37, 18D10, 57M25},
         year = {2001},
        month = {Nov},
          eid = {math/0111057},
        pages = {math/0111057},
archivePrefix = {arXiv},
       eprint = {math/0111057},
 primaryClass = {math.GT},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001math.....11057K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article {Mostow68,
    AUTHOR = {Mostow, G. D.},
     TITLE = {Quasi-conformal mappings in {$n$}-space and the rigidity of
              hyperbolic space forms},
   JOURNAL = {Inst. Hautes \'{E}tudes Sci. Publ. Math.},
  FJOURNAL = {Institut des Hautes \'{E}tudes Scientifiques. Publications
              Math\'{e}matiques},
    NUMBER = {34},
      YEAR = {1968},
     PAGES = {53--104},
      ISSN = {0073-8301},
   MRCLASS = {30.47},
  MRNUMBER = {0236383},
MRREVIEWER = {R. J. Cannon},
       URL = {http://www.numdam.org/item?id=PMIHES_1968__34__53_0},
}
	

@book {Chavel06,
    AUTHOR = {Chavel, Isaac},
     TITLE = {Riemannian geometry},
    SERIES = {Cambridge Studies in Advanced Mathematics},
    VOLUME = {98},
   EDITION = {Second},
      NOTE = {A modern introduction},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {2006},
     PAGES = {xvi+471},
      ISBN = {978-0-521-61954-7; 0-521-61954-8},
   MRCLASS = {53-02 (53Cxx)},
  MRNUMBER = {2229062},
       DOI = {10.1017/CBO9780511616822},
       URL = {https://doi.org/10.1017/CBO9780511616822},
}

@book {Hirsch94,
    AUTHOR = {Hirsch, Morris W.},
     TITLE = {Differential topology},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {33},
      NOTE = {Corrected reprint of the 1976 original},
 PUBLISHER = {Springer-Verlag, New York},
      YEAR = {1994},
     PAGES = {x+222},
      ISBN = {0-387-90148-5},
   MRCLASS = {57-01 (58-01)},
  MRNUMBER = {1336822},
}

@book {Nicolaescu11,
    AUTHOR = {Nicolaescu, Liviu},
     TITLE = {An invitation to {M}orse theory},
    SERIES = {Universitext},
   EDITION = {Second},
 PUBLISHER = {Springer, New York},
      YEAR = {2011},
     PAGES = {xvi+353},
      ISBN = {978-1-4614-1104-8},
   MRCLASS = {58E05 (37D15 37J15 57R45 57R70 58K05)},
  MRNUMBER = {2883440},
       DOI = {10.1007/978-1-4614-1105-5},
       URL = {https://doi.org/10.1007/978-1-4614-1105-5},
}

@book {PrasolovSossinsky97,
    AUTHOR = {Prasolov, V. V. and Sossinsky, A. B.},
     TITLE = {Knots, links, braids and 3-manifolds},
    SERIES = {Translations of Mathematical Monographs},
    VOLUME = {154},
      NOTE = {An introduction to the new invariants in low-dimensional
              topology,
              Translated from the Russian manuscript by Sossinsky
              [Sosinski\u{\i}]},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {1997},
     PAGES = {viii+239},
      ISBN = {0-8218-0588-6},
   MRCLASS = {57M25 (57M12 57N10)},
  MRNUMBER = {1414898},
MRREVIEWER = {Joanna Kania-Bartoszynska},
}

@article {Yoshida85,
    AUTHOR = {Yoshida, Tomoyoshi},
     TITLE = {The {$\eta$}-invariant of hyperbolic {$3$}-manifolds},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {81},
      YEAR = {1985},
    NUMBER = {3},
     PAGES = {473--514},
      ISSN = {0020-9910},
   MRCLASS = {58G10 (53C20 57R20)},
  MRNUMBER = {807069},
MRREVIEWER = {Th. Friedrich},
       DOI = {10.1007/BF01388583},
       URL = {https://doi.org/10.1007/BF01388583},
}

@book {Ohtsuki02,
    AUTHOR = {Ohtsuki, Tomotada},
     TITLE = {Quantum invariants},
    SERIES = {Series on Knots and Everything},
    VOLUME = {29},
      NOTE = {A study of knots, 3-manifolds, and their sets},
 PUBLISHER = {World Scientific Publishing Co., Inc., River Edge, NJ},
      YEAR = {2002},
     PAGES = {xiv+489},
      ISBN = {981-02-4675-7},
   MRCLASS = {57M27},
  MRNUMBER = {1881401},
MRREVIEWER = {Justin D. Roberts},
}

@book {Yetter01,
    AUTHOR = {Yetter, David N.},
     TITLE = {Functorial knot theory},
    SERIES = {Series on Knots and Everything},
    VOLUME = {26},
      NOTE = {Categories of tangles, coherence, categorical deformations,
              and topological invariants},
 PUBLISHER = {World Scientific Publishing Co., Inc., River Edge, NJ},
      YEAR = {2001},
     PAGES = {iv+230},
      ISBN = {981-02-4443-6},
   MRCLASS = {18D10 (57M25 57M27)},
  MRNUMBER = {1834675},
MRREVIEWER = {Nikolai N. Saveliev},
       DOI = {10.1142/9789812810465},
       URL = {https://doi.org/10.1142/9789812810465},
}

@article {Neumann04,
    AUTHOR = {Neumann, Walter D.},
     TITLE = {Extended {B}loch group and the {C}heeger-{C}hern-{S}imons
              class},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry and Topology},
    VOLUME = {8},
      YEAR = {2004},
     PAGES = {413--474},
      ISSN = {1465-3060},
   MRCLASS = {57M27 (11G55 19E99 57R20 57T99)},
  MRNUMBER = {2033484},
MRREVIEWER = {Kerry N. Jones},
       DOI = {10.2140/gt.2004.8.413},
       URL = {https://doi.org/10.2140/gt.2004.8.413},
}

@incollection {CheegerSimons85,
    AUTHOR = {Cheeger, Jeff and Simons, James},
     TITLE = {Differential characters and geometric invariants},
 BOOKTITLE = {Geometry and topology ({C}ollege {P}ark, {M}d., 1983/84)},
    SERIES = {Lecture Notes in Math.},
    VOLUME = {1167},
     PAGES = {50--80},
 PUBLISHER = {Springer, Berlin},
      YEAR = {1985},
   MRCLASS = {53C20 (57R20 58G10)},
  MRNUMBER = {827262},
MRREVIEWER = {P. Molino},
       DOI = {10.1007/BFb0075216},
       URL = {https://doi.org/10.1007/BFb0075216},
}

@article {Thurston82,
    AUTHOR = {Thurston, William P.},
     TITLE = {Three-dimensional manifolds, {K}leinian groups and hyperbolic
              geometry},
   JOURNAL = {Bull. Amer. Math. Soc. (N.S.)},
  FJOURNAL = {American Mathematical Society. Bulletin. New Series},
    VOLUME = {6},
      YEAR = {1982},
    NUMBER = {3},
     PAGES = {357--381},
      ISSN = {0273-0979},
   MRCLASS = {57N10 (20H15 30F40 57M35 57M40 57S17)},
  MRNUMBER = {648524},
MRREVIEWER = {Klaus Johannson},
       DOI = {10.1090/S0273-0979-1982-15003-0},
       URL = {https://doi.org/10.1090/S0273-0979-1982-15003-0},
}

@article {NeumannZagier85,
    AUTHOR = {Neumann, Walter D. and Zagier, Don},
     TITLE = {Volumes of hyperbolic three-manifolds},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {24},
      YEAR = {1985},
    NUMBER = {3},
     PAGES = {307--332},
      ISSN = {0040-9383},
   MRCLASS = {57N10 (22E40 53C20)},
  MRNUMBER = {815482},
MRREVIEWER = {Troels J\o rgensen},
       DOI = {10.1016/0040-9383(85)90004-7},
       URL = {https://doi.org/10.1016/0040-9383(85)90004-7},
}

@article {SergeiSuikowski12,
    AUTHOR = {Gukov, Sergei and Su\l kowski, Piotr},
     TITLE = {A-polynomial, {B}-model, and quantization},
   JOURNAL = {J. High Energy Phys.},
  FJOURNAL = {Journal of High Energy Physics},
      YEAR = {2012},
    NUMBER = {2},
     PAGES = {070, front matter+56},
      ISSN = {1126-6708},
   MRCLASS = {81T70 (57M25)},
  MRNUMBER = {2996110},
MRREVIEWER = {Vida Milani},
       DOI = {10.1007/JHEP02(2012)070},
       URL = {https://doi.org/10.1007/JHEP02(2012)070},
}

@article {TudorGukovLenellsZagier09,
    AUTHOR = {Dimofte, Tudor and Gukov, Sergei and Lenells, Jonatan and
              Zagier, Don},
     TITLE = {Exact results for perturbative {C}hern-{S}imons theory with
              complex gauge group},
   JOURNAL = {Commun. Number Theory Phys.},
  FJOURNAL = {Communications in Number Theory and Physics},
    VOLUME = {3},
      YEAR = {2009},
    NUMBER = {2},
     PAGES = {363--443},
      ISSN = {1931-4523},
   MRCLASS = {58J28 (33B30 57M27 81Q30 81T45)},
  MRNUMBER = {2551896},
MRREVIEWER = {Hitoshi Murakami},
       DOI = {10.4310/CNTP.2009.v3.n2.a4},
       URL = {https://doi.org/10.4310/CNTP.2009.v3.n2.a4},
}

@article {Gukov05,
    AUTHOR = {Gukov, Sergei},
     TITLE = {Three-dimensional quantum gravity, {C}hern-{S}imons theory,
              and the {A}-polynomial},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {255},
      YEAR = {2005},
    NUMBER = {3},
     PAGES = {577--627},
      ISSN = {0010-3616},
   MRCLASS = {58J28 (57M27 57M50 81T13 83C45 83C80)},
  MRNUMBER = {2134725},
MRREVIEWER = {Marcel L. Vonk},
       DOI = {10.1007/s00220-005-1312-y},
       URL = {https://doi.org/10.1007/s00220-005-1312-y},
}

@article {GaroufalidisThurstonZickert15,
    AUTHOR = {Garoufalidis, Stavros and Thurston, Dylan P. and Zickert,
              Christian K.},
     TITLE = {The complex volume of SL(n,C)-representations
              of 3-manifolds},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {164},
      YEAR = {2015},
    NUMBER = {11},
     PAGES = {2099--2160},
      ISSN = {0012-7094},
   MRCLASS = {57N10 (11G55 11R70 19F27 57M27 57M50 58J28)},
  MRNUMBER = {3385130},
MRREVIEWER = {Mattia Mecchia},
       DOI = {10.1215/00127094-3121185},
       URL = {https://doi.org/10.1215/00127094-3121185},
}

@book {Sontz15,
    AUTHOR = {Sontz, Stephen Bruce},
     TITLE = {Principal bundles},
    SERIES = {Universitext},
      NOTE = {The classical case},
 PUBLISHER = {Springer, Cham},
      YEAR = {2015},
     PAGES = {xvi+280},
      ISBN = {978-3-319-14764-2; 978-3-319-14765-9},
   MRCLASS = {53C05 (53-01 53C80 53Z05 78A25 81T13)},
  MRNUMBER = {3309256},
MRREVIEWER = {Fernando Etayo Gordejuela},
       DOI = {10.1007/978-3-319-15829-7},
       URL = {https://doi.org/10.1007/978-3-319-15829-7},
}

@book {KobayashiNomizu96b,
    AUTHOR = {Kobayashi, Shoshichi and Nomizu, Katsumi},
     TITLE = {Foundations of differential geometry. {V}ol. {II}},
    SERIES = {Wiley Classics Library},
      NOTE = {Reprint of the 1969 original,
              A Wiley-Interscience Publication},
 PUBLISHER = {John Wiley \& Sons, Inc., New York},
      YEAR = {1996},
     PAGES = {xvi+468},
      ISBN = {0-471-15732-5},
   MRCLASS = {53-01},
  MRNUMBER = {1393941},
}
    
@book {KobayashiNomizu96a,
    AUTHOR = {Kobayashi, Shoshichi and Nomizu, Katsumi},
     TITLE = {Foundations of differential geometry. {V}ol. {I}},
    SERIES = {Wiley Classics Library},
      NOTE = {Reprint of the 1963 original,
              A Wiley-Interscience Publication},
 PUBLISHER = {John Wiley \& Sons, Inc., New York},
      YEAR = {1996},
     PAGES = {xii+329},
      ISBN = {0-471-15733-3},
   MRCLASS = {53-01},
  MRNUMBER = {1393940},
}

@book {Joyce07,
    AUTHOR = {Joyce, Dominic D.},
     TITLE = {Riemannian holonomy groups and calibrated geometry},
    SERIES = {Oxford Graduate Texts in Mathematics},
    VOLUME = {12},
 PUBLISHER = {Oxford University Press, Oxford},
      YEAR = {2007},
     PAGES = {x+303},
      ISBN = {978-0-19-921559-1},
   MRCLASS = {53C38 (53C29)},
  MRNUMBER = {2292510},
MRREVIEWER = {Spiro Karigiannis},
}

@incollection {Thaddeus97,
    AUTHOR = {Thaddeus, Michael},
     TITLE = {An introduction to the topology of the moduli space of stable
              bundles on a {R}iemann surface},
 BOOKTITLE = {Geometry and physics ({A}arhus, 1995)},
    SERIES = {Lecture Notes in Pure and Appl. Math.},
    VOLUME = {184},
     PAGES = {71--99},
 PUBLISHER = {Dekker, New York},
      YEAR = {1997},
   MRCLASS = {14D20 (14F25 14H60)},
  MRNUMBER = {1423157},
MRREVIEWER = {Werner Kleinert},
}

@article {CataldoHauselMigliorini12,
    AUTHOR = {de Cataldo, Mark Andrea A. and Hausel, Tam\'{a}s and Migliorini,
              Luca},
     TITLE = {Topology of {H}itchin systems and {H}odge theory of character
              varieties: the case {$A_1$}},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {175},
      YEAR = {2012},
    NUMBER = {3},
     PAGES = {1329--1407},
      ISSN = {0003-486X},
   MRCLASS = {14D20 (53D30)},
  MRNUMBER = {2912707},
MRREVIEWER = {Sean Lawton},
       DOI = {10.4007/annals.2012.175.3.7},
       URL = {https://doi.org/10.4007/annals.2012.175.3.7},
}

@article {HauselRodriguez,
    AUTHOR = {Hausel, Tam\'{a}s and Rodriguez-Villegas, Fernando},
     TITLE = {Mixed {H}odge polynomials of character varieties},
      NOTE = {With an appendix by Nicholas M. Katz},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {174},
      YEAR = {2008},
    NUMBER = {3},
     PAGES = {555--624},
      ISSN = {0020-9910},
   MRCLASS = {14L30 (14D20 14F43)},
  MRNUMBER = {2453601},
MRREVIEWER = {Sean Lawton},
       DOI = {10.1007/s00222-008-0142-x},
       URL = {https://doi.org/10.1007/s00222-008-0142-x},
}

@article {HauselThaddeus03,
    AUTHOR = {Hausel, Tam\'{a}s and Thaddeus, Michael},
     TITLE = {Mirror symmetry, {L}anglands duality, and the {H}itchin
              system},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {153},
      YEAR = {2003},
    NUMBER = {1},
     PAGES = {197--229},
      ISSN = {0020-9910},
   MRCLASS = {14J32 (14D20 32J25 32Q25)},
  MRNUMBER = {1990670},
MRREVIEWER = {Anatoly Libgober},
       DOI = {10.1007/s00222-003-0286-7},
       URL = {https://doi.org/10.1007/s00222-003-0286-7},
}

@ARTICLE{ChengChunFerrariGukovHarrison18,
       author = {{Cheng}, Miranda C.~N. and {Chun}, Sungbong and {Ferrari}, Francesca and
         {Gukov}, Sergei and {Harrison}, Sarah M.},
        title = "{3d Modularity}",
      journal = {arXiv e-prints},
     keywords = {High Energy Physics - Theory, Mathematics - Geometric Topology, Mathematics - Number Theory, Mathematics - Quantum Algebra, Mathematics - Representation Theory},
         year = "2018",
        month = "Sep",
          eid = {arXiv:1809.10148},
        pages = {arXiv:1809.10148},
archivePrefix = {arXiv},
       eprint = {1809.10148},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018arXiv180910148C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GukovPeiPutrovVada18,
       author = {{Gukov}, Sergei and {Pei}, Du and {Putrov}, Pavel and {Vafa}, Cumrun},
        title = "{4-manifolds and topological modular forms}",
      journal = {arXiv e-prints},
     keywords = {High Energy Physics - Theory, Mathematical Physics, Mathematics - Algebraic Topology, Mathematics - Geometric Topology},
         year = "2018",
        month = "Nov",
          eid = {arXiv:1811.07884},
        pages = {arXiv:1811.07884},
archivePrefix = {arXiv},
       eprint = {1811.07884},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018arXiv181107884G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article {ACampo73,
    AUTHOR = {A'Campo, Norbert},
     TITLE = {Le nombre de Lefschetz d'une monodromie},
   JOURNAL = {Nederl. Akad. Wetensch. Proc. Ser. A 76 = Indag. Math.},
    VOLUME = {35},
      YEAR = {1973},
     PAGES = {113--118},
   MRCLASS = {32C40 (14D05 14B05)},
  MRNUMBER = {0320364},
MRREVIEWER = {J. P. Levine},
}

@article {ACampo75,
    AUTHOR = {A'Campo, Norbert},
     TITLE = {La fonction z\^{e}ta d'une monodromie},
   JOURNAL = {Comment. Math. Helv.},
  FJOURNAL = {Commentarii Mathematici Helvetici},
    VOLUME = {50},
      YEAR = {1975},
     PAGES = {233--248},
      ISSN = {0010-2571},
   MRCLASS = {14B05 (32C40 14D05)},
  MRNUMBER = {0371889},
MRREVIEWER = {R. C. Randell},
       DOI = {10.1007/BF02565748},
       URL = {https://doi.org/10.1007/BF02565748},
}

@book {Forster91,
    AUTHOR = {Forster, Otto},
     TITLE = {Lectures on {R}iemann surfaces},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {81},
      NOTE = {Translated from the 1977 German original by Bruce Gilligan,
              Reprint of the 1981 English translation},
 PUBLISHER = {Springer-Verlag, New York},
      YEAR = {1991},
     PAGES = {viii+254},
      ISBN = {0-387-90617-7},
   MRCLASS = {30Fxx (14H55 32-01)},
  MRNUMBER = {1185074},
}

@article {Manin58,
    AUTHOR = {Manin, Ju. I.},
     TITLE = {Algebraic curves over fields with differentiation},
   JOURNAL = {Izv. Akad. Nauk SSSR. Ser. Mat.},
  FJOURNAL = {Izvestiya Akademii Nauk SSSR. Seriya Matematicheskaya},
    VOLUME = {22},
      YEAR = {1958},
     PAGES = {737--756},
      ISSN = {0373-2436},
   MRCLASS = {14.00},
  MRNUMBER = {0103889},
MRREVIEWER = {E. Lluis},
}

@article {Varchenko81,
    AUTHOR = {Var\v{c}enko, A. N.},
     TITLE = {Asymptotic {H}odge structure on vanishing cohomology},
   JOURNAL = {Izv. Akad. Nauk SSSR Ser. Mat.},
  FJOURNAL = {Izvestiya Akademii Nauk SSSR. Seriya Matematicheskaya},
    VOLUME = {45},
      YEAR = {1981},
    NUMBER = {3},
     PAGES = {540--591, 688},
      ISSN = {0373-2436},
   MRCLASS = {32B30 (14F40 32G20 57R45)},
  MRNUMBER = {623350},
MRREVIEWER = {I. Dolgachev},
}

@article {Brieskorn70,
    AUTHOR = {Brieskorn, Egbert},
     TITLE = {Die {M}onodromie der isolierten {S}ingularit\"{a}ten von
              {H}yperfl\"{a}chen},
   JOURNAL = {Manuscripta Math.},
  FJOURNAL = {Manuscripta Mathematica},
    VOLUME = {2},
      YEAR = {1970},
     PAGES = {103--161},
      ISSN = {0025-2611},
   MRCLASS = {57.60},
  MRNUMBER = {0267607},
MRREVIEWER = {J. P. Levine},
       DOI = {10.1007/BF01155695},
       URL = {https://doi.org/10.1007/BF01155695},
}

@article {Leray59,
    AUTHOR = {Leray, Jean},
     TITLE = {Le calcul diff\'{e}rentiel et int\'{e}gral sur une vari\'{e}t\'{e} analytique
              complexe. ({P}robl\`eme de {C}auchy. {III})},
   JOURNAL = {Bull. Soc. Math. France},
  FJOURNAL = {Bulletin de la Soci\'{e}t\'{e} Math\'{e}matique de France},
    VOLUME = {87},
      YEAR = {1959},
     PAGES = {81--180},
      ISSN = {0037-9484},
   MRCLASS = {32.15 (32.40)},
  MRNUMBER = {0125984},
MRREVIEWER = {F. Norguet},
       URL = {http://www.numdam.org/item?id=BSMF_1959__87__81_0},
}

@article {LeDT77,
    AUTHOR = {L\^{e} D\~{u}ng Tr\'{a}ng},
     TITLE = {Some remarks on relative monodromy},
 BOOKTITLE = {Real and complex singularities ({P}roc. {N}inth {N}ordic
              {S}ummer {S}chool/{NAVF} {S}ympos. {M}ath., {O}slo, 1976)},
     PAGES = {397--403},
 PUBLISHER = {Sijthoff and Noordhoff, Alphen aan den Rijn},
      YEAR = {1977},
   MRCLASS = {14D05},
  MRNUMBER = {0476739},
MRREVIEWER = {I. N. Iomdin},
}

@book {Milnor68,
    AUTHOR = {Milnor, John},
     TITLE = {Singular points of complex hypersurfaces},
    SERIES = {Annals of Mathematics Studies, No. 61},
 PUBLISHER = {Princeton University Press, Princeton, N.J.; University of
              Tokyo Press, Tokyo},
      YEAR = {1968},
     PAGES = {iii+122},
   MRCLASS = {57.20 (14.00)},
  MRNUMBER = {0239612},
MRREVIEWER = {J. P. Levine},
}

@article {Kontsevich03,
    AUTHOR = {Kontsevich, Maxim},
     TITLE = {Deformation quantization of {P}oisson manifolds},
   JOURNAL = {Lett. Math. Phys.},
  FJOURNAL = {Letters in Mathematical Physics},
    VOLUME = {66},
      YEAR = {2003},
    NUMBER = {3},
     PAGES = {157--216},
      ISSN = {0377-9017},
   MRCLASS = {53D55 (16E40 53D17 81S10)},
  MRNUMBER = {2062626},
MRREVIEWER = {David Chataur},
       DOI = {10.1023/B:MATH.0000027508.00421.bf},
       URL = {https://doi.org/10.1023/B:MATH.0000027508.00421.bf},
}

@article {Tuynman87,
    AUTHOR = {Tuynman, G. M.},
     TITLE = {Generalized {B}ergman kernels and geometric quantization},
   JOURNAL = {J. Math. Phys.},
  FJOURNAL = {Journal of Mathematical Physics},
    VOLUME = {28},
      YEAR = {1987},
    NUMBER = {3},
     PAGES = {573--583},
      ISSN = {0022-2488},
   MRCLASS = {58F06 (81D07)},
  MRNUMBER = {877229},
MRREVIEWER = {J. H. Rawnsley},
       DOI = {10.1063/1.527642},
       URL = {https://doi.org/10.1063/1.527642},
}

@book {BoutetdeMonvelGuillemin81,
    AUTHOR = {Boutet de Monvel, L. and Guillemin, V.},
     TITLE = {The spectral theory of {T}oeplitz operators},
    SERIES = {Annals of Mathematics Studies},
    VOLUME = {99},
 PUBLISHER = {Princeton University Press, Princeton, NJ; University of Tokyo
              Press, Tokyo},
      YEAR = {1981},
     PAGES = {v+161},
      ISBN = {0-691-08284-7; 0-691-08279-0},
   MRCLASS = {58G15 (32F20 35Pxx 35S05 47B35)},
  MRNUMBER = {620794},
MRREVIEWER = {V. Peller},
       DOI = {10.1515/9781400881444},
       URL = {https://doi.org/10.1515/9781400881444},
}

@book {Milnor63,
    AUTHOR = {Milnor, J.},
     TITLE = {Morse theory},
    SERIES = {Based on lecture notes by M. Spivak and R. Wells. Annals of
              Mathematics Studies, No. 51},
 PUBLISHER = {Princeton University Press, Princeton, N.J.},
      YEAR = {1963},
     PAGES = {vi+153},
   MRCLASS = {57.50 (53.72)},
  MRNUMBER = {0163331},
MRREVIEWER = {H. I. Levine},
}

@book {Wong01,
    AUTHOR = {Wong, R.},
     TITLE = {Asymptotic approximations of integrals},
    SERIES = {Classics in Applied Mathematics},
    VOLUME = {34},
      NOTE = {Corrected reprint of the 1989 original},
 PUBLISHER = {Society for Industrial and Applied Mathematics (SIAM),
              Philadelphia, PA},
      YEAR = {2001},
     PAGES = {xviii+543},
      ISBN = {0-89871-497-4},
   MRCLASS = {41A60 (44A15 46F10)},
  MRNUMBER = {1851050},
       DOI = {10.1137/1.9780898719260},
       URL = {https://doi.org/10.1137/1.9780898719260},
}

@book {Hormander03,
    AUTHOR = {H\"{o}rmander, Lars},
     TITLE = {The analysis of linear partial differential operators. {I}},
    SERIES = {Classics in Mathematics},
      NOTE = {Distribution theory and Fourier analysis,
              Reprint of the second (1990) edition [Springer, Berlin;
              MR1065993 (91m:35001a)]},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {2003},
     PAGES = {x+440},
      ISBN = {3-540-00662-1},
   MRCLASS = {35-02},
  MRNUMBER = {1996773},
       DOI = {10.1007/978-3-642-61497-2},
       URL = {https://doi.org/10.1007/978-3-642-61497-2},
}

@book {Neretin11,
    AUTHOR = {Neretin, Yurii A.},
     TITLE = {Lectures on {G}aussian integral operators and classical
              groups},
    SERIES = {EMS Series of Lectures in Mathematics},
 PUBLISHER = {European Mathematical Society (EMS), Z\"{u}rich},
      YEAR = {2011},
     PAGES = {xii+559},
      ISBN = {978-3-03719-080-7},
   MRCLASS = {22E30 (22E46 32A70 46E20 47A48 47G10)},
  MRNUMBER = {2790054},
MRREVIEWER = {Philip J. Feinsilver},
       DOI = {10.4171/080},
       URL = {https://doi.org/10.4171/080},
}

@article {Hansen2001,
    AUTHOR = {Hansen, S\o ren Kold},
     TITLE = {Reshetikhin-{T}uraev invariants of {S}eifert 3-manifolds and a
              rational surgery formula},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {1},
      YEAR = {2001},
     PAGES = {627--686},
      ISSN = {1472-2747},
   MRCLASS = {57M27 (18D10)},
  MRNUMBER = {1875611},
MRREVIEWER = {Nikolai N. Saveliev},
       DOI = {10.2140/agt.2001.1.627},
       URL = {https://doi.org/10.2140/agt.2001.1.627},
}

@article {GaroufalidisLaudaLe18,
    AUTHOR = {Garoufalidis, Stavros and Lauda, Aaron D. and L\^{e}, Thang T. Q.},
     TITLE = {The colored {HOMFLYPT} function is {$q$}-holonomic},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {167},
      YEAR = {2018},
    NUMBER = {3},
     PAGES = {397--447},
      ISSN = {0012-7094},
   MRCLASS = {57M27 (57M25)},
  MRNUMBER = {3761103},
MRREVIEWER = {Benjamin Cooper},
       DOI = {10.1215/00127094-2017-0030},
       URL = {https://doi.org/10.1215/00127094-2017-0030},
}

@article {Turaev88,
    AUTHOR = {Turaev, V. G.},
     TITLE = {The {Y}ang-{B}axter equation and invariants of links},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {92},
      YEAR = {1988},
    NUMBER = {3},
     PAGES = {527--553},
      ISSN = {0020-9910},
   MRCLASS = {57M25 (20F36 82A68)},
  MRNUMBER = {939474},
MRREVIEWER = {Toshitake Kohno},
       DOI = {10.1007/BF01393746},
       URL = {https://doi.org/10.1007/BF01393746},
}

@article {InesSchiappaVonk12,
    AUTHOR = {Aniceto, In\^{e}s and Schiappa, Ricardo and Vonk, Marcel},
     TITLE = {The resurgence of instantons in string theory},
   JOURNAL = {Commun. Number Theory Phys.},
  FJOURNAL = {Communications in Number Theory and Physics},
    VOLUME = {6},
      YEAR = {2012},
    NUMBER = {2},
     PAGES = {339--496},
      ISSN = {1931-4523},
   MRCLASS = {81T30 (15B52)},
  MRNUMBER = {2993121},
MRREVIEWER = {Gernot Akemann},
       DOI = {10.4310/CNTP.2012.v6.n2.a3},
       URL = {https://doi.org/10.4310/CNTP.2012.v6.n2.a3},
}

@article {CousoSantamariaEdelsteinSchiappaVonk15,
    AUTHOR = {Couso-Santamar\'{i}a, Ricardo and Edelstein, Jos\'{e} D. and Schiappa,
              Ricardo and Vonk, Marcel},
     TITLE = {Resurgent transseries and the holomorphic anomaly:
              nonperturbative closed strings in local {$\Bbb{C}\Bbb{P}^2$}},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {338},
      YEAR = {2015},
    NUMBER = {1},
     PAGES = {285--346},
      ISSN = {0010-3616},
   MRCLASS = {32L81 (81T30)},
  MRNUMBER = {3345378},
MRREVIEWER = {Adam Gregory Harris},
       DOI = {10.1007/s00220-015-2358-0},
       URL = {https://doi.org/10.1007/s00220-015-2358-0},
}

@article {CousoSantamariaEdelsteinSchiappaVonk16,
    AUTHOR = {Couso-Santamar\'{i}a, Ricardo and Edelstein, Jos\'{e} D. and Schiappa,
              Ricardo and Vonk, Marcel},
     TITLE = {Resurgent transseries and the holomorphic anomaly},
   JOURNAL = {Ann. Henri Poincar\'{e}},
  FJOURNAL = {Annales Henri Poincar\'{e}. A Journal of Theoretical and
              Mathematical Physics},
    VOLUME = {17},
      YEAR = {2016},
    NUMBER = {2},
     PAGES = {331--399},
      ISSN = {1424-0637},
   MRCLASS = {81T13},
  MRNUMBER = {3447848},
       DOI = {10.1007/s00023-015-0407-z},
       URL = {https://doi.org/10.1007/s00023-015-0407-z},
}

@incollection {KapustinSaulinab11,
    AUTHOR = {Kapustin, Anton and Saulina, Natalia},
     TITLE = {Surface operators in 3d topological field theory and 2d
              rational conformal field theory},
 BOOKTITLE = {Mathematical foundations of quantum field theory and
              perturbative string theory},
    SERIES = {Proc. Sympos. Pure Math.},
    VOLUME = {83},
     PAGES = {175--198},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2011},
   MRCLASS = {81T45 (18D05 81T40)},
  MRNUMBER = {2742429},
MRREVIEWER = {Christoph Schweigert},
       DOI = {10.1090/pspum/083/2742429},
       URL = {https://doi.org/10.1090/pspum/083/2742429},
}

@article {KapustinSaulina11a,
    AUTHOR = {Kapustin, Anton and Saulina, Natalia},
     TITLE = {Topological boundary conditions in abelian {C}hern-{S}imons
              theory},
   JOURNAL = {Nuclear Phys. B},
  FJOURNAL = {Nuclear Physics. B. Theoretical, Phenomenological, and
              Experimental High Energy Physics. Quantum Field Theory and
              Statistical Systems},
    VOLUME = {845},
      YEAR = {2011},
    NUMBER = {3},
     PAGES = {393--435},
      ISSN = {0550-3213},
   MRCLASS = {57R56 (18D05 81T45)},
  MRNUMBER = {2755172},
MRREVIEWER = {Johannes Walcher},
       DOI = {10.1016/j.nuclphysb.2010.12.017},
       URL = {https://doi.org/10.1016/j.nuclphysb.2010.12.017},
}

@article {CappelliItzyksonZuber87,
    AUTHOR = {Cappelli, A. and Itzykson, C. and Zuber, J.-B.},
     TITLE = {The {${\rm A}$}-{${\rm D}$}-{${\rm E}$} classification of
              minimal and {$A^{(1)}_1$} conformal invariant theories},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {113},
      YEAR = {1987},
    NUMBER = {1},
     PAGES = {1--26},
      ISSN = {0010-3616},
   MRCLASS = {81E99 (11F22 17B67 81E40 82A68)},
  MRNUMBER = {918402},
MRREVIEWER = {Andrew A. Bytsenko},
       URL = {http://projecteuclid.org/euclid.cmp/1104160138},
}

@article {Gurarie93,
    AUTHOR = {Gurarie, V.},
     TITLE = {Logarithmic operators in conformal field theory},
   JOURNAL = {Nuclear Phys. B},
  FJOURNAL = {Nuclear Physics. B. Theoretical, Phenomenological, and
              Experimental High Energy Physics. Quantum Field Theory and
              Statistical Systems},
    VOLUME = {410},
      YEAR = {1993},
    NUMBER = {3},
     PAGES = {535--549},
      ISSN = {0550-3213},
   MRCLASS = {81T40 (17B68 81R10 82B43 82D60)},
  MRNUMBER = {1256422},
MRREVIEWER = {Stanislav Z. Pakuliak},
       DOI = {10.1016/0550-3213(93)90528-W},
       URL = {https://doi.org/10.1016/0550-3213(93)90528-W},
}

@article {Gawedzki05,
    AUTHOR = {Gaw\c{e}dzki, Krzysztof},
     TITLE = {Abelian and non-abelian branes in {WZW} models and gerbes},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {258},
      YEAR = {2005},
    NUMBER = {1},
     PAGES = {23--73},
      ISSN = {0010-3616},
   MRCLASS = {81T40 (53C80)},
  MRNUMBER = {2166839},
MRREVIEWER = {Hisham Sati},
       DOI = {10.1007/s00220-005-1301-1},
       URL = {https://doi.org/10.1007/s00220-005-1301-1},
}

@incollection {Gawedzki89b,
    AUTHOR = {Gaw\polhk edzki, K.},
     TITLE = {Constructive conformal field theory},
 BOOKTITLE = {Functional integration, geometry and strings ({K}arpacz,
              1989)},
    SERIES = {Progr. Phys.},
    VOLUME = {13},
     PAGES = {277--302},
 PUBLISHER = {Birkh\"{a}user, Basel},
      YEAR = {1989},
   MRCLASS = {81T40 (81T08)},
  MRNUMBER = {1056302},
MRREVIEWER = {Siddhartha Sen},
}

@article {GawedzkiKupiainen89a,
    AUTHOR = {Gaw\polhk edzki, K. and Kupiainen, A.},
     TITLE = {Coset construction from functional integrals},
   JOURNAL = {Nuclear Phys. B},
  FJOURNAL = {Nuclear Physics. B. Theoretical, Phenomenological, and
              Experimental High Energy Physics. Quantum Field Theory and
              Statistical Systems},
    VOLUME = {320},
      YEAR = {1989},
    NUMBER = {3},
     PAGES = {625--668},
      ISSN = {0550-3213},
   MRCLASS = {81T40 (22E70 81T13)},
  MRNUMBER = {1004371},
MRREVIEWER = {Omar Foda},
       DOI = {10.1016/0550-3213(89)90015-1},
       URL = {https://doi.org/10.1016/0550-3213(89)90015-1},
}

@incollection {Gawedzki91,
    AUTHOR = {Gaw\polhk edzki, Krzysztof},
     TITLE = {Noncompact {WZW} conformal field theories},
 BOOKTITLE = {New symmetry principles in quantum field theory ({C}arg\`ese,
              1991)},
    SERIES = {NATO Adv. Sci. Inst. Ser. B Phys.},
    VOLUME = {295},
     PAGES = {247--274},
 PUBLISHER = {Plenum, New York},
      YEAR = {1992},
   MRCLASS = {81T40 (81-02)},
  MRNUMBER = {1204457},
}
@article {DupontZickert06,
    AUTHOR = {Dupont, Johan L. and Zickert, Christian K.},
     TITLE = {A dilogarithmic formula for the {C}heeger-{C}hern-{S}imons
              class},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry and Topology},
    VOLUME = {10},
      YEAR = {2006},
     PAGES = {1347--1372},
      ISSN = {1465-3060},
   MRCLASS = {58J28 (11G55 57M27 57T10 57T30)},
  MRNUMBER = {2255500},
MRREVIEWER = {Jerzy Browkin},
       DOI = {10.2140/gt.2006.10.1347},
       URL = {https://doi.org/10.2140/gt.2006.10.1347},
}


@article {FuchsSchweigertValentin013,
    AUTHOR = {Fuchs, J\"{u}rgen and Schweigert, Christoph and Valentino,
              Alessandro},
     TITLE = {Bicategories for boundary conditions and for surface defects
              in 3-d {TFT}},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {321},
      YEAR = {2013},
    NUMBER = {2},
     PAGES = {543--575},
      ISSN = {0010-3616},
   MRCLASS = {81T45 (18B99 57R56)},
  MRNUMBER = {3063919},
MRREVIEWER = {Theo Johnson-Freyd},
       DOI = {10.1007/s00220-013-1723-0},
       URL = {https://doi.org/10.1007/s00220-013-1723-0},
}

@ARTICLE{CarquevilleRunkelSchaumann17,
       author = {{Carqueville}, Nils and {Runkel}, Ingo and {Schaumann}, Gregor},
        title = "{Line and surface defects in Reshetikhin-Turaev TQFT}",
      journal = {arXiv e-prints},
     keywords = {Mathematics - Quantum Algebra, High Energy Physics - Theory, Mathematical Physics, Mathematics - Geometric Topology},
         year = "2017",
        month = "Oct",
          eid = {arXiv:1710.10214},
        pages = {arXiv:1710.10214},
archivePrefix = {arXiv},
       eprint = {1710.10214},
 primaryClass = {math.QA},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2017arXiv171010214C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article {FuchsRunkelSchweigert02,
    AUTHOR = {Fuchs, J\"{u}rgen and Runkel, Ingo and Schweigert, Christoph},
     TITLE = {T{FT} construction of {RCFT} correlators. {I}. {P}artition
              functions},
   JOURNAL = {Nuclear Phys. B},
  FJOURNAL = {Nuclear Physics. B. Theoretical, Phenomenological, and
              Experimental High Energy Physics. Quantum Field Theory and
              Statistical Systems},
    VOLUME = {646},
      YEAR = {2002},
    NUMBER = {3},
     PAGES = {353--497},
      ISSN = {0550-3213},
   MRCLASS = {81T40 (18D10 57R56 81R10 81T45)},
  MRNUMBER = {1940282},
MRREVIEWER = {Stephen F. Sawin},
       DOI = {10.1016/S0550-3213(02)00744-7},
       URL = {https://doi.org/10.1016/S0550-3213(02)00744-7},
}

@article {FuchsRunkelSchweigert05,
    AUTHOR = {Fuchs, J\"{u}rgen and Runkel, Ingo and Schweigert, Christoph},
     TITLE = {T{FT} construction of {RCFT} correlators. {IV}. {S}tructure
              constants and correlation functions},
   JOURNAL = {Nuclear Phys. B},
  FJOURNAL = {Nuclear Physics. B. Theoretical, Phenomenological, and
              Experimental High Energy Physics. Quantum Field Theory and
              Statistical Systems},
    VOLUME = {715},
      YEAR = {2005},
    NUMBER = {3},
     PAGES = {539--638},
      ISSN = {0550-3213},
   MRCLASS = {81T40 (18D10 57R56 81R10 81T45)},
  MRNUMBER = {2137114},
MRREVIEWER = {Bogus\l aw Broda},
       DOI = {10.1016/j.nuclphysb.2005.03.018},
       URL = {https://doi.org/10.1016/j.nuclphysb.2005.03.018},
}

@article {FuchsRunkelSchweigert05,
    AUTHOR = {Fuchs, J\"{u}rgen and Runkel, Ingo and Schweigert, Christoph},
     TITLE = {T{FT} construction of {RCFT} correlators. {IV}. {S}tructure
              constants and correlation functions},
   JOURNAL = {Nuclear Phys. B},
  FJOURNAL = {Nuclear Physics. B. Theoretical, Phenomenological, and
              Experimental High Energy Physics. Quantum Field Theory and
              Statistical Systems},
    VOLUME = {715},
      YEAR = {2005},
    NUMBER = {3},
     PAGES = {539--638},
      ISSN = {0550-3213},
   MRCLASS = {81T40 (18D10 57R56 81R10 81T45)},
  MRNUMBER = {2137114},
MRREVIEWER = {Bogus\l aw Broda},
       DOI = {10.1016/j.nuclphysb.2005.03.018},
       URL = {https://doi.org/10.1016/j.nuclphysb.2005.03.018},
}

@inproceedings {Teschner04,
    AUTHOR = {Teschner, J.},
     TITLE = {On the relation between quantum {L}iouville theory and the
              quantized {T}eichm\"{u}ller spaces},
 BOOKTITLE = {Proceedings of 6th {I}nternational {W}orkshop on {C}onformal
              {F}ield {T}heory and {I}ntegrable {M}odels},
   JOURNAL = {Internat. J. Modern Phys. A},
  FJOURNAL = {International Journal of Modern Physics A. Particles and
              Fields. Gravitation. Cosmology},
    VOLUME = {19},
      YEAR = {2004},
    NUMBER = {May, suppl.},
     PAGES = {459--477},
      ISSN = {0217-751X},
   MRCLASS = {81T40 (32G15 32G81)},
  MRNUMBER = {2087126},
MRREVIEWER = {Rinat M. Kashaev},
       DOI = {10.1142/S0217751X04020579},
       URL = {https://doi.org/10.1142/S0217751X04020579},
}

@article {BeliakovaBlanchetLe08,
    AUTHOR = {Beliakova, Anna and Blanchet, Christian and L\^{e}, Thang T. Q.},
     TITLE = {Unified quantum invariants and their refinements for homology
              3-spheres with 2-torsion},
   JOURNAL = {Fund. Math.},
  FJOURNAL = {Fundamenta Mathematicae},
    VOLUME = {201},
      YEAR = {2008},
    NUMBER = {3},
     PAGES = {217--239},
      ISSN = {0016-2736},
   MRCLASS = {57M27 (57M25 57N10)},
  MRNUMBER = {2457479},
MRREVIEWER = {Gw\'{e}na\"{e}l Massuyeau},
       DOI = {10.4064/fm201-3-2},
       URL = {https://doi.org/10.4064/fm201-3-2},
}

@incollection {CieliebakLatschev09,
    AUTHOR = {Cieliebak, Kai and Latschev, Janko},
     TITLE = {The role of string topology in symplectic field theory},
 BOOKTITLE = {New perspectives and challenges in symplectic field theory},
    SERIES = {CRM Proc. Lecture Notes},
    VOLUME = {49},
     PAGES = {113--146},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2009},
   MRCLASS = {53D42 (55P50)},
  MRNUMBER = {2555935},
MRREVIEWER = {Tobias Ekholm},
}

@incollection {CieliiebakHoferLatschev07,
    AUTHOR = {Cieliebak, Kai and Hofer, Helmut and Latschev, Janko and
              Schlenk, Felix},
     TITLE = {Quantitative symplectic geometry},
 BOOKTITLE = {Dynamics, ergodic theory, and geometry},
    SERIES = {Math. Sci. Res. Inst. Publ.},
    VOLUME = {54},
     PAGES = {1--44},
 PUBLISHER = {Cambridge Univ. Press, Cambridge},
      YEAR = {2007},
   MRCLASS = {53D35 (37J05 57R17)},
  MRNUMBER = {2369441},
MRREVIEWER = {Michael J. Usher},
       DOI = {10.1017/CBO9780511755187.002},
       URL = {https://doi.org/10.1017/CBO9780511755187.002},
}

@article {AlekseevskyCortesDevchand02,
    AUTHOR = {Alekseevsky, D. V. and Cort\'{e}s, V. and Devchand, C.},
     TITLE = {Special complex manifolds},
   JOURNAL = {J. Geom. Phys.},
  FJOURNAL = {Journal of Geometry and Physics},
    VOLUME = {42},
      YEAR = {2002},
    NUMBER = {1-2},
     PAGES = {85--105},
      ISSN = {0393-0440},
   MRCLASS = {53C26 (53C56)},
  MRNUMBER = {1894078},
MRREVIEWER = {Andrew Swann},
       DOI = {10.1016/S0393-0440(01)00078-X},
       URL = {https://doi.org/10.1016/S0393-0440(01)00078-X},
}

@article {CortesMS04,
    AUTHOR = {Cort\'{e}s, Vicente and Mayer, Christoph and Mohaupt, Thomas and
              Saueressig, Frank},
     TITLE = {Special geometry of {E}uclidean supersymmetry. {I}. {V}ector
              multiplets},
   JOURNAL = {J. High Energy Phys.},
  FJOURNAL = {Journal of High Energy Physics. A SISSA Journal},
      YEAR = {2004},
    NUMBER = {3},
     PAGES = {028, 73},
      ISSN = {1126-6708},
   MRCLASS = {53C26 (53C80 81T60)},
  MRNUMBER = {2061551},
MRREVIEWER = {Krzysztof Galicki},
       DOI = {10.1088/1126-6708/2004/03/028},
       URL = {https://doi.org/10.1088/1126-6708/2004/03/028},
}

@article {Teschner11,
    AUTHOR = {Teschner, J.},
     TITLE = {Quantization of the {H}itchin moduli spaces, {L}iouville
              theory and the geometric {L}anglands correspondence {I}},
   JOURNAL = {Adv. Theor. Math. Phys.},
  FJOURNAL = {Advances in Theoretical and Mathematical Physics},
    VOLUME = {15},
      YEAR = {2011},
    NUMBER = {2},
     PAGES = {471--564},
      ISSN = {1095-0761},
   MRCLASS = {81T40 (14D24 32G81 34M56 53C26 53D50 81T60)},
  MRNUMBER = {2924236},
MRREVIEWER = {Lee-Peng Teo},
       URL = {http://projecteuclid.org/euclid.atmp/1337951929},
}

@article {BytskoTeschner13,
    AUTHOR = {Bytsko, A. and Teschner, J.},
     TITLE = {The integrable structure of nonrational conformal field
              theory},
   JOURNAL = {Adv. Theor. Math. Phys.},
  FJOURNAL = {Advances in Theoretical and Mathematical Physics},
    VOLUME = {17},
      YEAR = {2013},
    NUMBER = {4},
     PAGES = {701--740},
      ISSN = {1095-0761},
   MRCLASS = {81T40 (81R12)},
  MRNUMBER = {3250766},
MRREVIEWER = {Lee-Peng Teo},
       URL = {http://projecteuclid.org/euclid.atmp/1408626423},
}

@article {TeschnerVartanov15,
    AUTHOR = {Teschner, J. and Vartanov, G. S.},
     TITLE = {Supersymmetric gauge theories, quantization of {$\mathcal{M}_{\text{flat}}$}, and conformal field theory},
   JOURNAL = {Adv. Theor. Math. Phys.},
  FJOURNAL = {Advances in Theoretical and Mathematical Physics},
    VOLUME = {19},
      YEAR = {2015},
    NUMBER = {1},
     PAGES = {1--135},
      ISSN = {1095-0761},
   MRCLASS = {81T13 (81T40 81T60)},
  MRNUMBER = {3418499},
MRREVIEWER = {Lewis H. Ryder},
       DOI = {10.4310/ATMP.2015.v19.n1.a1},
       URL = {https://doi.org/10.4310/ATMP.2015.v19.n1.a1},
}

@article {GrossSiebert13,
    AUTHOR = {Gross, Mark and Siebert, Bernd},
     TITLE = {Logarithmic {G}romov-{W}itten invariants},
   JOURNAL = {J. Amer. Math. Soc.},
  FJOURNAL = {Journal of the American Mathematical Society},
    VOLUME = {26},
      YEAR = {2013},
    NUMBER = {2},
     PAGES = {451--510},
      ISSN = {0894-0347},
   MRCLASS = {14N35 (14D23)},
  MRNUMBER = {3011419},
MRREVIEWER = {Hsian-Hua Tseng},
       DOI = {10.1090/S0894-0347-2012-00757-7},
       URL = {https://doi.org/10.1090/S0894-0347-2012-00757-7},
}

@article {NishinouSiebert06,
    AUTHOR = {Nishinou, Takeo and Siebert, Bernd},
     TITLE = {Toric degenerations of toric varieties and tropical curves},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {135},
      YEAR = {2006},
    NUMBER = {1},
     PAGES = {1--51},
      ISSN = {0012-7094},
   MRCLASS = {14N10 (14M25 14N35)},
  MRNUMBER = {2259922},
MRREVIEWER = {Diego Matessi},
       DOI = {10.1215/S0012-7094-06-13511-1},
       URL = {https://doi.org/10.1215/S0012-7094-06-13511-1},
}

@article {GrossPandharipandeSiebert10,
    AUTHOR = {Gross, Mark and Pandharipande, Rahul and Siebert, Bernd},
     TITLE = {The tropical vertex},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {153},
      YEAR = {2010},
    NUMBER = {2},
     PAGES = {297--362},
      ISSN = {0012-7094},
   MRCLASS = {14N35 (14T05 53D45)},
  MRNUMBER = {2667135},
MRREVIEWER = {Hsian-Hua Tseng},
       DOI = {10.1215/00127094-2010-025},
       URL = {https://doi.org/10.1215/00127094-2010-025},
}

@article {SiebertTian05,
    AUTHOR = {Siebert, Bernd and Tian, Gang},
     TITLE = {On the holomorphicity of genus two {L}efschetz fibrations},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {161},
      YEAR = {2005},
    NUMBER = {2},
     PAGES = {959--1020},
      ISSN = {0003-486X},
   MRCLASS = {53D35 (53D45 57R17)},
  MRNUMBER = {2153404},
MRREVIEWER = {Ivan Smith},
       DOI = {10.4007/annals.2005.161.959},
       URL = {https://doi.org/10.4007/annals.2005.161.959},
}

@article {Richter00,
    AUTHOR = {Richter, Birgit},
     TITLE = {{$E_\infty$}-structure for {$Q_*(R)$}},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {316},
      YEAR = {2000},
    NUMBER = {3},
     PAGES = {547--564},
      ISSN = {0025-5831},
   MRCLASS = {16E40 (19D55 55P47)},
  MRNUMBER = {1752784},
MRREVIEWER = {Teimuraz Pirashvili},
       DOI = {10.1007/s002080050343},
       URL = {https://doi.org/10.1007/s002080050343},
}

@article {GrossSiebert11,
    AUTHOR = {Gross, Mark and Siebert, Bernd},
     TITLE = {From real affine geometry to complex geometry},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {174},
      YEAR = {2011},
    NUMBER = {3},
     PAGES = {1301--1428},
      ISSN = {0003-486X},
   MRCLASS = {53D37 (14J33 14T05)},
  MRNUMBER = {2846484},
MRREVIEWER = {Siu-Cheong Lau},
       DOI = {10.4007/annals.2011.174.3.1},
       URL = {https://doi.org/10.4007/annals.2011.174.3.1},
}

@article {CarquevilleRunkel,
    AUTHOR = {Carqueville, Nils and Runkel, Ingo},
     TITLE = {Orbifold completion of defect bicategories},
   JOURNAL = {Quantum Topol.},
  FJOURNAL = {Quantum Topology},
    VOLUME = {7},
      YEAR = {2016},
    NUMBER = {2},
     PAGES = {203--279},
      ISSN = {1663-487X},
   MRCLASS = {18D05 (57R56)},
  MRNUMBER = {3459961},
MRREVIEWER = {Volodymyr V. Lyubashenko},
       DOI = {10.4171/QT/76},
       URL = {https://doi.org/10.4171/QT/76},
}

@article {DavydovKongRunkel15,
    AUTHOR = {Davydov, Alexei and Kong, Liang and Runkel, Ingo},
     TITLE = {Functoriality of the center of an algebra},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {285},
      YEAR = {2015},
     PAGES = {811--876},
      ISSN = {0001-8708},
   MRCLASS = {18D10 (18D05)},
  MRNUMBER = {3406516},
MRREVIEWER = {Carlos Soneira Calvo},
       DOI = {10.1016/j.aim.2015.06.023},
       URL = {https://doi.org/10.1016/j.aim.2015.06.023},
}

@article {KongQuinRunkel14,
    AUTHOR = {Kong, Liang and Li, Qin and Runkel, Ingo},
     TITLE = {Cardy algebras and sewing constraints, {II}},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {262},
      YEAR = {2014},
     PAGES = {604--681},
      ISSN = {0001-8708},
   MRCLASS = {81T40 (16D90 17B69 18D10)},
  MRNUMBER = {3228439},
MRREVIEWER = {Andreas Arvanitoyeorgos},
       DOI = {10.1016/j.aim.2014.05.020},
       URL = {https://doi.org/10.1016/j.aim.2014.05.020},
}

@article {KongRunkel08,
    AUTHOR = {Kong, Liang and Runkel, Ingo},
     TITLE = {Morita classes of algebras in modular tensor categories},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {219},
      YEAR = {2008},
    NUMBER = {5},
     PAGES = {1548--1576},
      ISSN = {0001-8708},
   MRCLASS = {18D10 (81T40)},
  MRNUMBER = {2458146},
MRREVIEWER = {Julien Bichon},
       DOI = {10.1016/j.aim.2008.07.004},
       URL = {https://doi.org/10.1016/j.aim.2008.07.004},
}

@article {FuchsSchaumannSchweigert17,
    AUTHOR = {Fuchs, J\"{u}rgen and Schaumann, Gregor and Schweigert, Christoph},
     TITLE = {A trace for bimodule categories},
   JOURNAL = {Appl. Categ. Structures},
  FJOURNAL = {Applied Categorical Structures. A Journal Devoted to
              Applications of Categorical Methods in Algebra, Analysis,
              Order, Topology and Computer Science},
    VOLUME = {25},
      YEAR = {2017},
    NUMBER = {2},
     PAGES = {227--268},
      ISSN = {0927-2852},
   MRCLASS = {18D05 (18D10 81T45)},
  MRNUMBER = {3638361},
MRREVIEWER = {Jos\'{e} N. Alonso \'{A}lvarez},
       DOI = {10.1007/s10485-016-9425-3},
       URL = {https://doi.org/10.1007/s10485-016-9425-3},
}

@article {FuchsRunkelSchweigert08,
    AUTHOR = {Fuchs, J\"{u}rgen and Runkel, Ingo and Schweigert, Christoph},
     TITLE = {The fusion algebra of bimodule categories},
   JOURNAL = {Appl. Categ. Structures},
  FJOURNAL = {Applied Categorical Structures. A Journal Devoted to
              Applications of Categorical Methods in Algebra, Analysis,
              Order, Topology and Computer Science},
    VOLUME = {16},
      YEAR = {2008},
    NUMBER = {1-2},
     PAGES = {123--140},
      ISSN = {0927-2852},
   MRCLASS = {18D10 (18D35 81T40)},
  MRNUMBER = {2383281},
       DOI = {10.1007/s10485-007-9102-7},
       URL = {https://doi.org/10.1007/s10485-007-9102-7},
}

@article {QuellaRunkelSchweigert02,
    AUTHOR = {Quella, Thomas and Runkel, Ingo and Schweigert, Christoph},
     TITLE = {An algorithm for twisted fusion rules},
   JOURNAL = {Adv. Theor. Math. Phys.},
  FJOURNAL = {Advances in Theoretical and Mathematical Physics},
    VOLUME = {6},
      YEAR = {2002},
    NUMBER = {2},
     PAGES = {197--205},
      ISSN = {1095-0761},
   MRCLASS = {17B81 (81R10)},
  MRNUMBER = {1937855},
MRREVIEWER = {Alberto Medina},
       DOI = {10.4310/ATMP.2002.v6.n2.a1},
       URL = {https://doi.org/10.4310/ATMP.2002.v6.n2.a1},
}

@article {FjelstadFuchsRunjkelSchweigert08,
    AUTHOR = {Fjelstad, Jens and Fuchs, J\"{u}rgen and Runkel, Ingo and
              Schweigert, Christoph},
     TITLE = {Uniqueness of open/closed rational {CFT} with given algebra of
              open states},
   JOURNAL = {Adv. Theor. Math. Phys.},
  FJOURNAL = {Advances in Theoretical and Mathematical Physics},
    VOLUME = {12},
      YEAR = {2008},
    NUMBER = {6},
     PAGES = {1283--1375},
      ISSN = {1095-0761},
   MRCLASS = {81T40 (18D10 57M27 81T45)},
  MRNUMBER = {2443266},
MRREVIEWER = {Stephen F. Sawin},
       URL = {http://projecteuclid.org/euclid.atmp/1221834534},
}

@article {MaierNikolausSchweigert12,
    AUTHOR = {Maier, Jennifer and Nikolaus, Thomas and Schweigert,
              Christoph},
     TITLE = {Equivariant modular categories via {D}ijkgraaf-{W}itten
              theory},
   JOURNAL = {Adv. Theor. Math. Phys.},
  FJOURNAL = {Advances in Theoretical and Mathematical Physics},
    VOLUME = {16},
      YEAR = {2012},
    NUMBER = {1},
     PAGES = {289--358},
      ISSN = {1095-0761},
   MRCLASS = {18D05 (57R56 81R05)},
  MRNUMBER = {3019407},
MRREVIEWER = {Olga Kravchenko},
       URL = {http://projecteuclid.org/euclid.atmp/1358950855},
}

@article {FuchsSchweigert14,
    AUTHOR = {Fuchs, J\"{u}rgen and Schweigert, Christoph and Stigner, Carl},
     TITLE = {Higher genus mapping class group invariants from factorizable
              {H}opf algebras},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {250},
      YEAR = {2014},
     PAGES = {285--319},
      ISSN = {0001-8708},
   MRCLASS = {57N05 (16T05)},
  MRNUMBER = {3122169},
MRREVIEWER = {Mohamed Elhamdadi},
       DOI = {10.1016/j.aim.2013.09.019},
       URL = {https://doi.org/10.1016/j.aim.2013.09.019},
}

@article {FuchSchweigerts17,
    AUTHOR = {Fuchs, J\"{u}rgen and Schweigert, Christoph},
     TITLE = {Consistent systems of correlators in non-semisimple conformal
              field theory},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {307},
      YEAR = {2017},
     PAGES = {598--639},
      ISSN = {0001-8708},
   MRCLASS = {81P40 (57R56)},
  MRNUMBER = {3590526},
MRREVIEWER = {Theo Johnson-Freyd},
       DOI = {10.1016/j.aim.2016.11.020},
       URL = {https://doi.org/10.1016/j.aim.2016.11.020},
}

@article {FFRS06,
    AUTHOR = {Fr\"{o}hlich, J\"{u}rg and Fuchs, J\"{u}rgen and Runkel, Ingo and
              Schweigert, Christoph},
     TITLE = {Correspondences of ribbon categories},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {199},
      YEAR = {2006},
    NUMBER = {1},
     PAGES = {192--329},
      ISSN = {0001-8708},
   MRCLASS = {18D10 (81R10 81R50 81T40)},
  MRNUMBER = {2187404},
MRREVIEWER = {Jos\'{e} M. Fern\'{a}ndez Vilaboa},
       DOI = {10.1016/j.aim.2005.04.007},
       URL = {https://doi.org/10.1016/j.aim.2005.04.007},
}

@book {Pham11,
    AUTHOR = {Pham, Fr\'{e}d\'{e}ric},
     TITLE = {Singularities of integrals},
    SERIES = {Universitext},
      NOTE = {Homology, hyperfunctions and microlocal analysis,
              With a foreword by Jacques Bros,
              Translated from the 2005 French original,
              With supplementary references by Claude Sabbah},
 PUBLISHER = {Springer, London; EDP Sciences, Les Ulis},
      YEAR = {2011},
     PAGES = {xxii+217},
      ISBN = {978-0-85729-602-3; 978-2-7598-0363-7},
   MRCLASS = {58J15 (32A27 32A45 32S30 46F15)},
  MRNUMBER = {2798679},
       DOI = {10.1007/978-0-85729-603-0},
       URL = {https://doi.org/10.1007/978-0-85729-603-0},
}

@book {GoreskyMacPherson88,
    AUTHOR = {Goresky, Mark and MacPherson, Robert},
     TITLE = {Stratified {M}orse theory},
    SERIES = {Ergebnisse der Mathematik und ihrer Grenzgebiete (3) [Results
              in Mathematics and Related Areas (3)]},
    VOLUME = {14},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {1988},
     PAGES = {xiv+272},
      ISBN = {3-540-17300-5},
   MRCLASS = {57R70 (14F45 32C10 32C42 57N80 58A35 58C27)},
  MRNUMBER = {932724},
MRREVIEWER = {K. Lamotke},
       DOI = {10.1007/978-3-642-71714-7},
       URL = {https://doi.org/10.1007/978-3-642-71714-7},
}

@article {FreedmanLarsenWang02b,
    AUTHOR = {Freedman, Michael H. and Larsen, Michael J. and Wang,
              Zhenghan},
     TITLE = {The two-eigenvalue problem and density of {J}ones
              representation of braid groups},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {228},
      YEAR = {2002},
    NUMBER = {1},
     PAGES = {177--199},
      ISSN = {0010-3616},
   MRCLASS = {20F36 (57M25 81P68)},
  MRNUMBER = {1911253},
       DOI = {10.1007/s002200200636},
       URL = {https://doi.org/10.1007/s002200200636},
}

@article {FreedmanLarsenWang02a,
    AUTHOR = {Freedman, Michael H. and Larsen, Michael and Wang, Zhenghan},
     TITLE = {A modular functor which is universal for quantum computation},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {227},
      YEAR = {2002},
    NUMBER = {3},
     PAGES = {605--622},
      ISSN = {0010-3616},
   MRCLASS = {57R56 (68P05 81P68)},
  MRNUMBER = {1910833},
MRREVIEWER = {R\u{a}zvan Gelca},
       DOI = {10.1007/s002200200645},
       URL = {https://doi.org/10.1007/s002200200645},
}

@article {FreedmanKitaecLarsenWang03,
    AUTHOR = {Freedman, Michael H. and Kitaev, Alexei and Larsen, Michael J.
              and Wang, Zhenghan},
     TITLE = {Topological quantum computation},
      NOTE = {Mathematical challenges of the 21st century (Los Angeles, CA,
              2000)},
   JOURNAL = {Bull. Amer. Math. Soc. (N.S.)},
  FJOURNAL = {American Mathematical Society. Bulletin. New Series},
    VOLUME = {40},
      YEAR = {2003},
    NUMBER = {1},
     PAGES = {31--38},
      ISSN = {0273-0979},
   MRCLASS = {57R56 (68Q05 81P68)},
  MRNUMBER = {1943131},
       DOI = {10.1090/S0273-0979-02-00964-3},
       URL = {https://doi.org/10.1090/S0273-0979-02-00964-3},
}

@article {FreedmanKitaecWang02,
    AUTHOR = {Freedman, Michael H. and Kitaev, Alexei and Wang, Zhenghan},
     TITLE = {Simulation of topological field theories by quantum computers},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {227},
      YEAR = {2002},
    NUMBER = {3},
     PAGES = {587--603},
      ISSN = {0010-3616},
   MRCLASS = {57R56 (68P05 81P68 81T45)},
  MRNUMBER = {1910832},
MRREVIEWER = {R\u{a}zvan Gelca},
       DOI = {10.1007/s002200200635},
       URL = {https://doi.org/10.1007/s002200200635},
}


@book {McDuffSalamon,
    AUTHOR = {McDuff, Dusa and Salamon, Dietmar},
     TITLE = {Introduction to symplectic topology},
    SERIES = {Oxford Graduate Texts in Mathematics},
   EDITION = {Third},
 PUBLISHER = {Oxford University Press, Oxford},
      YEAR = {2017},
     PAGES = {xi+623},
      ISBN = {978-0-19-879490-5; 978-0-19-879489-9},
   MRCLASS = {53D35 (53D40 57R17 57R57 57R58)},
  MRNUMBER = {3674984},
MRREVIEWER = {Hansj\"{o}rg Geiges},
       DOI = {10.1093/oso/9780198794899.001.0001},
       URL = {https://doi.org/10.1093/oso/9780198794899.001.0001},
}

@article {WongMcLure84,
    AUTHOR = {Wong, R. and McClure, J. P.},
     TITLE = {Generalized {M}ellin convolutions and their asymptotic
              expansions},
   JOURNAL = {Canad. J. Math.},
  FJOURNAL = {Canadian Journal of Mathematics. Journal Canadien de
              Math\'{e}matiques},
    VOLUME = {36},
      YEAR = {1984},
    NUMBER = {5},
     PAGES = {924--960},
      ISSN = {0008-414X},
   MRCLASS = {41A60 (44A15)},
  MRNUMBER = {762749},
MRREVIEWER = {John S. Lew},
       DOI = {10.4153/CJM-1984-053-x},
       URL = {https://doi.org/10.4153/CJM-1984-053-x},
}

@article {FGD95,
    AUTHOR = {Flajolet, Philippe and Gourdon, Xavier and Dumas, Philippe},
     TITLE = {Mellin transforms and asymptotics: harmonic sums},
      NOTE = {Special volume on mathematical analysis of algorithms},
   JOURNAL = {Theoret. Comput. Sci.},
  FJOURNAL = {Theoretical Computer Science},
    VOLUME = {144},
      YEAR = {1995},
    NUMBER = {1-2},
     PAGES = {3--58},
      ISSN = {0304-3975},
   MRCLASS = {68Q25 (44A15 68P05)},
  MRNUMBER = {1337752},
MRREVIEWER = {Peter Kirschenhofer},
       DOI = {10.1016/0304-3975(95)00002-E},
       URL = {https://doi.org/10.1016/0304-3975(95)00002-E},
}

@incollection {Schlichenmaier12,
    AUTHOR = {Schlichenmaier, Martin},
     TITLE = {Berezin-{T}oeplitz quantization and star products for compact
              {K}\"{a}hler manifolds},
 BOOKTITLE = {Mathematical aspects of quantization},
    SERIES = {Contemp. Math.},
    VOLUME = {583},
     PAGES = {257--294},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2012},
   MRCLASS = {53D55 (47B35)},
  MRNUMBER = {3013098},
MRREVIEWER = {Stefan Waldmann},
       DOI = {10.1090/conm/583/11573},
       URL = {https://doi.org/10.1090/conm/583/11573},
}

@article {Braam88,
    AUTHOR = {Braam, Peter J.},
     TITLE = {Floer homology groups for homology three-spheres},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {88},
      YEAR = {1991},
    NUMBER = {2},
     PAGES = {131--144},
      ISSN = {0001-8708},
   MRCLASS = {57N10 (57R57 58G10 58G25)},
  MRNUMBER = {1120610},
MRREVIEWER = {Ronald J. Stern},
       DOI = {10.1016/0001-8708(91)90005-R},
       URL = {https://doi.org/10.1016/0001-8708(91)90005-R},
}

@article {Floer88,
    AUTHOR = {Floer, Andreas},
     TITLE = {An instanton-invariant for {$3$}-manifolds},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {118},
      YEAR = {1988},
    NUMBER = {2},
     PAGES = {215--240},
      ISSN = {0010-3616},
   MRCLASS = {57N10 (58G05 58G10 58G25)},
  MRNUMBER = {956166},
MRREVIEWER = {Ronald J. Stern},
       URL = {http://projecteuclid.org/euclid.cmp/1104161987},
}

@book {BoutetdeMonvelGuillemin99,
    AUTHOR = {Boutet de Monvel, L. and Guillemin, V.},
     TITLE = {The spectral theory of {T}oeplitz operators},
    SERIES = {Annals of Mathematics Studies},
    VOLUME = {99},
 PUBLISHER = {Princeton University Press, Princeton, NJ; University of Tokyo
              Press, Tokyo},
      YEAR = {1981},
     PAGES = {v+161},
      ISBN = {0-691-08284-7; 0-691-08279-0},
   MRCLASS = {58G15 (32F20 35Pxx 35S05 47B35)},
  MRNUMBER = {620794},
MRREVIEWER = {V. Peller},
       DOI = {10.1515/9781400881444},
       URL = {https://doi.org/10.1515/9781400881444},
}

@article {Berezin74,
    AUTHOR = {Berezin, F. A.},
     TITLE = {Quantization},
   JOURNAL = {Izv. Akad. Nauk SSSR Ser. Mat.},
  FJOURNAL = {Izvestiya Akademii Nauk SSSR. Seriya Matematicheskaya},
    VOLUME = {38},
      YEAR = {1974},
     PAGES = {1116--1175},
      ISSN = {0373-2436},
   MRCLASS = {81.58 (81.46)},
  MRNUMBER = {0395610},
MRREVIEWER = {A. S. Wightman},
}

@book {Souriau70,
    AUTHOR = {Souriau, J.-M.},
     TITLE = {Structure des syst\`emes dynamiques},
    SERIES = {Ma\^{i}trises de math\'{e}matiques},
 PUBLISHER = {Dunod, Paris},
      YEAR = {1970},
     PAGES = {xxxii+414},
   MRCLASS = {69.00 (70.00)},
  MRNUMBER = {0260238},
MRREVIEWER = {J. R. Vanstone},
}

@article {Kostant70,
    AUTHOR = {Kostant, Bertram},
     TITLE = {Quantization and unitary representations. {I}.
              {P}requantization},
 BOOKTITLE = {Lectures in modern analysis and applications, {III}},
     PAGES = {87--208. Lecture Notes in Math., Vol. 170},
 PUBLISHER = {Springer, Berlin},
      YEAR = {1970},
   MRCLASS = {22E70},
  MRNUMBER = {0294568},
MRREVIEWER = {S. Sankaran},
}

@ARTICLE{IoosLuMa17,
       author = {{Ioos}, Louis and {Lu}, Wen and {Ma}, Xiaonan and {Marinescu}, George},
        title = "{Berezin-Toeplitz quantization for eigenstates of the Bochner-Laplacian on symplectic manifolds}",
      journal = {arXiv e-prints},
     keywords = {Mathematics - Differential Geometry},
         year = 2017,
        month = Mar,
          eid = {arXiv:1703.06420},
        pages = {arXiv:1703.06420},
archivePrefix = {arXiv},
       eprint = {1703.06420},
 primaryClass = {math.DG},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2017arXiv170306420I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book {GuilleminSternberg77,
    AUTHOR = {Guillemin, Victor and Sternberg, Shlomo},
     TITLE = {Geometric asymptotics},
      NOTE = {Mathematical Surveys, No. 14},
 PUBLISHER = {American Mathematical Society, Providence, R.I.},
      YEAR = {1977},
     PAGES = {xviii+474 pp. (one plate)},
   MRCLASS = {58G15 (35C99 41A60 47G05 58F05 78.58)},
  MRNUMBER = {0516965},
MRREVIEWER = {Ju. V. Egorov},
}

@article {Hormander71,
    AUTHOR = {H\"{o}rmander, Lars},
     TITLE = {Fourier integral operators. {I}},
   JOURNAL = {Acta Math.},
  FJOURNAL = {Acta Mathematica},
    VOLUME = {127},
      YEAR = {1971},
    NUMBER = {1-2},
     PAGES = {79--183},
      ISSN = {0001-5962},
   MRCLASS = {58G15 (35S05 47G05)},
  MRNUMBER = {0388463},
MRREVIEWER = {Ju. V. Egorov},
       DOI = {10.1007/BF02392052},
       URL = {https://doi.org/10.1007/BF02392052},
}

@article {DuistermaatHormander72,
    AUTHOR = {Duistermaat, J. J. and H\"{o}rmander, L.},
     TITLE = {Fourier integral operators. {II}},
   JOURNAL = {Acta Math.},
  FJOURNAL = {Acta Mathematica},
    VOLUME = {128},
      YEAR = {1972},
    NUMBER = {3-4},
     PAGES = {183--269},
      ISSN = {0001-5962},
   MRCLASS = {58G15 (35S05 47G05)},
  MRNUMBER = {0388464},
MRREVIEWER = {Ju. V. Egorov},
       DOI = {10.1007/BF02392165},
       URL = {https://doi.org/10.1007/BF02392165},
}

@incollection {DU17,
    AUTHOR = {Dunne, Gerald V. and \"{U}nsal, Mithat},
     TITLE = {W{KB} and resurgence in the {M}athieu equation},
 BOOKTITLE = {Resurgence, physics and numbers},
    SERIES = {CRM Series},
    VOLUME = {20},
     PAGES = {249--298},
 PUBLISHER = {Ed. Norm., Pisa},
      YEAR = {2017},
   MRCLASS = {34M60 (35J10 81R12)},
  MRNUMBER = {3728779},
MRREVIEWER = {Gabriel Alvarez},
}

@incollection {Witten11a,
    AUTHOR = {Witten, Edward},
     TITLE = {A new look at the path integral of quantum mechanics},
 BOOKTITLE = {Surveys in differential geometry. {V}olume {XV}.
              {P}erspectives in mathematics and physics},
    SERIES = {Surv. Differ. Geom.},
    VOLUME = {15},
     PAGES = {345--419},
 PUBLISHER = {Int. Press, Somerville, MA},
      YEAR = {2011},
   MRCLASS = {81T45 (58D30 81S40 81T60)},
  MRNUMBER = {2817248},
MRREVIEWER = {Johannes Walcher},
       DOI = {10.4310/SDG.2010.v15.n1.a11},
       URL = {https://doi.org/10.4310/SDG.2010.v15.n1.a11},
}

@article {BDSSU,
    AUTHOR = {Behtash, Alireza and Dunne, Gerald V. and Sch\"{a}fer, Thomas and
              Sulejmanpasic, Tin and \"{U}nsal, Mithat},
     TITLE = {Toward {P}icard-{L}efschetz theory of path integrals, complex
              saddles and resurgence},
   JOURNAL = {Ann. Math. Sci. Appl.},
  FJOURNAL = {Annals of Mathematical Sciences and Applications},
    VOLUME = {2},
      YEAR = {2017},
    NUMBER = {1},
     PAGES = {95--212},
      ISSN = {2380-288X},
   MRCLASS = {81Q30},
  MRNUMBER = {3682433},
MRREVIEWER = {W\l adys\l aw Adam Majewski},
       DOI = {10.4310/AMSA.2017.v2.n1.a3},
       URL = {https://doi.org/10.4310/AMSA.2017.v2.n1.a3},
}

@article {Guralnik,
    AUTHOR = {Guralnik, G. and Guralnik, Z.},
     TITLE = {Complexified path integrals and the phases of quantum field
              theory},
   JOURNAL = {Ann. Physics},
  FJOURNAL = {Annals of Physics},
    VOLUME = {325},
      YEAR = {2010},
    NUMBER = {11},
     PAGES = {2486--2498},
      ISSN = {0003-4916},
   MRCLASS = {81S40 (34M40 58D30 81R40)},
  MRNUMBER = {2718556},
MRREVIEWER = {Vitor R. Vieira},
       DOI = {10.1016/j.aop.2010.06.001},
       URL = {https://doi.org/10.1016/j.aop.2010.06.001},
}

@article {Wallace60,
    AUTHOR = {Wallace, Andrew H.},
     TITLE = {Modifications and cobounding manifolds},
   JOURNAL = {Canad. J. Math.},
  FJOURNAL = {Canadian Journal of Mathematics. Journal Canadien de
              Math\'{e}matiques},
    VOLUME = {12},
      YEAR = {1960},
     PAGES = {503--528},
      ISSN = {0008-414X},
   MRCLASS = {57.10},
  MRNUMBER = {0125588},
MRREVIEWER = {M. W. Hirsch},
       DOI = {10.4153/CJM-1960-045-7},
       URL = {https://doi.org/10.4153/CJM-1960-045-7},
}

@article {Lickorish62,
    AUTHOR = {Lickorish, W. B. R.},
     TITLE = {A representation of orientable combinatorial {$3$}-manifolds},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {76},
      YEAR = {1962},
     PAGES = {531--540},
      ISSN = {0003-486X},
   MRCLASS = {54.78},
  MRNUMBER = {0151948},
MRREVIEWER = {A. D. Wallace},
       DOI = {10.2307/1970373},
       URL = {https://doi.org/10.2307/1970373},
}

@book {Lefschetz75,
    AUTHOR = {Lefschetz, S.},
     TITLE = {Applications of algebraic topology},
      NOTE = {Graphs and networks, the Picard-Lefschetz theory and Feynman
              integrals,
              Applied Mathematical Sciences, Vol. 16},
 PUBLISHER = {Springer-Verlag, New York-Heidelberg},
      YEAR = {1975},
     PAGES = {viii+189},
   MRCLASS = {57C05 (14D05 81.32 94A20)},
  MRNUMBER = {0494126},
MRREVIEWER = {P. Orlik},
}

@book {Lefschetz,
    AUTHOR = {Lefschetz, S.},
     TITLE = {L'analysis situs et la g\'{e}om\'{e}trie alg\'{e}brique},
 PUBLISHER = {Gauthier-Villars, Paris},
      YEAR = {1950},
     PAGES = {vi+154},
   MRCLASS = {14.0X},
  MRNUMBER = {0033557},
}

@book {PicardSimart,
    AUTHOR = {Picard, \'{E}mile and Simart, Georges},
     TITLE = {Th\'{e}orie des fonctions alg\'{e}briques de deux variables
              ind\'{e}pendantes. {T}ome {I}, {II}},
      NOTE = {R\'{e}impression corrig\'{e}e (en un volume) de l'\'{e}dition en deux
              volumes de 1897 et 1906},
 PUBLISHER = {Chelsea Publishing Co., Bronx, N.Y.},
      YEAR = {1971},
     PAGES = {Tome I: xiv+244 pp.; Tome II: ii+52 pp. (bound as one)},
   MRCLASS = {01A75},
  MRNUMBER = {0392468},
}

@ARTICLE{Chung18,
       author = {{Chung}, Hee-Joong},
        title = "{BPS Invariants for Seifert Manifolds}",
      journal = {arXiv e-prints},
     keywords = {High Energy Physics - Theory, Mathematics - Geometric Topology,
        Mathematics - Number Theory},
         year = 2018,
        month = Nov,
          eid = {arXiv:1811.08863},
        pages = {arXiv:1811.08863},
archivePrefix = {arXiv},
       eprint = {1811.08863},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2018arXiv181108863C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{ChengChunFerrariGukovHarrison,
       author = {{Cheng}, Miranda C.~N. and {Chun}, Sungbong and {Ferrari}, Francesca and
        {Gukov}, Sergei and {Harrison}, Sarah M.},
        title = "{3d Modularity}",
      journal = {arXiv e-prints},
     keywords = {High Energy Physics - Theory, Mathematics - Geometric Topology,
        Mathematics - Number Theory, Mathematics - Quantum Algebra,
        Mathematics - Representation Theory},
         year = 2018,
        month = Sep,
          eid = {arXiv:1809.10148},
        pages = {arXiv:1809.10148},
archivePrefix = {arXiv},
       eprint = {1809.10148},
 primaryClass = {hep-th},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2018arXiv180910148C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Yoon18,
   author = {{Yoon}, S.},
    title = "{On the potential functions for a link diagram}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1810.09080},
 primaryClass = "math.GT",
 keywords = {Mathematics - Geometric Topology, 57M25, 57M27},
     year = 2018,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv181009080Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book {HowlsKawaiTakei00,
     TITLE = {Toward the exact {WKB} analysis of differential equations,
              linear or non-linear},
    EDITOR = {Howls, Christopher J. and Kawai, Takahiro and Takei,
              Yoshitsugu},
      NOTE = {Papers from the Symposium on Algebraic Analysis of Singular
              Perturbations held at Kyoto University, Kyoto, November
              30--December 5, 1998},
 PUBLISHER = {Kyoto University Press, Kyoto},
      YEAR = {2000},
     PAGES = {x+298},
      ISBN = {4-87698-089-6},
   MRCLASS = {34-06 (32-06 34E20 34M30 34M55 34M60 81-06)},
  MRNUMBER = {1770278},
}

@book {Costin09,
    AUTHOR = {Costin, Ovidiu},
     TITLE = {Asymptotics and {B}orel summability},
    SERIES = {Chapman \& Hall/CRC Monographs and Surveys in Pure and Applied
              Mathematics},
    VOLUME = {141},
 PUBLISHER = {CRC Press, Boca Raton, FL},
      YEAR = {2009},
     PAGES = {xiv+250},
      ISBN = {978-1-4200-7031-6},
   MRCLASS = {34-02 (34M30 34M37 34M40 34M55 39A11 40G10)},
  MRNUMBER = {2474083},
MRREVIEWER = {B. L. J. Braaksma},
}

@book {Vassiliev02,
    AUTHOR = {Vassiliev, V. A.},
     TITLE = {Applied {P}icard-{L}efschetz theory},
    SERIES = {Mathematical Surveys and Monographs},
    VOLUME = {97},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {2002},
     PAGES = {xii+324},
      ISBN = {0-8218-2948-3},
   MRCLASS = {32S40 (14B05 14D05)},
  MRNUMBER = {1930577},
MRREVIEWER = {Jan Stevens},
       DOI = {10.1090/surv/097},
       URL = {https://doi.org/10.1090/surv/097},
}

@book {Loday-Richaud16,
    AUTHOR = {Loday-Richaud, Mich\`ele},
     TITLE = {Divergent series, summability and resurgence. {II}},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {2154},
      NOTE = {Simple and multiple summability,
              With prefaces by Jean-Pierre Ramis, \'{E}ric Delabaere, Claude
              Mitschi and David Sauzin},
 PUBLISHER = {Springer, [Cham]},
      YEAR = {2016},
     PAGES = {xxiii+272},
      ISBN = {978-3-319-29074-4; 978-3-319-29075-1},
   MRCLASS = {40-02 (34-02 34M30 40A05 40A30 40Cxx)},
  MRNUMBER = {3495546},
MRREVIEWER = {Francisco Marcell\'{a}n},
       DOI = {10.1007/978-3-319-29075-1},
       URL = {https://doi.org/10.1007/978-3-319-29075-1},
}

@article {BorotEynardOrantin15,
    AUTHOR = {Borot, G. and Eynard, B. and Orantin, N.},
     TITLE = {Abstract loop equations, topological recursion and new
              applications},
   JOURNAL = {Commun. Number Theory Phys.},
  FJOURNAL = {Communications in Number Theory and Physics},
    VOLUME = {9},
      YEAR = {2015},
    NUMBER = {1},
     PAGES = {51--187},
      ISSN = {1931-4523},
   MRCLASS = {81T45},
  MRNUMBER = {3339853},
       DOI = {10.4310/CNTP.2015.v9.n1.a2},
       URL = {https://doi.org/10.4310/CNTP.2015.v9.n1.a2},
}

@article {EynardOrantin09,
    AUTHOR = {Eynard, B. and Orantin, N.},
     TITLE = {Topological recursion in enumerative geometry and random
              matrices},
   JOURNAL = {J. Phys. A},
  FJOURNAL = {Journal of Physics. A. Mathematical and Theoretical},
    VOLUME = {42},
      YEAR = {2009},
    NUMBER = {29},
     PAGES = {293001, 117},
      ISSN = {1751-8113},
   MRCLASS = {14N10 (14H10 14N35 37K20)},
  MRNUMBER = {2519749},
MRREVIEWER = {Hsian-Hua Tseng},
       DOI = {10.1088/1751-8113/42/29/293001},
       URL = {https://doi.org/10.1088/1751-8113/42/29/293001},
}

@incollection {KontsevichSoibelman14,
    AUTHOR = {Kontsevich, M. and Soibelman, Y.},
     TITLE = {Wall-crossing structures in {D}onaldson-{T}homas invariants,
              integrable systems and mirror symmetry},
 BOOKTITLE = {Homological mirror symmetry and tropical geometry},
    SERIES = {Lect. Notes Unione Mat. Ital.},
    VOLUME = {15},
     PAGES = {197--308},
 PUBLISHER = {Springer, Cham},
      YEAR = {2014},
   MRCLASS = {14N35 (14J33 53D37)},
  MRNUMBER = {3330788},
MRREVIEWER = {Victor Przyjalkowski},
       DOI = {10.1007/978-3-319-06514-4_6},
       URL = {https://doi.org/10.1007/978-3-319-06514-4_6},
}

@incollection {Le16,
    AUTHOR = {L\^{e}, T. T. Q.},
     TITLE = {The colored {J}ones polynomial and the {AJ} conjecture},
 BOOKTITLE = {Lectures on quantum topology in dimension three},
    SERIES = {Panor. Synth\`eses},
    VOLUME = {48},
     PAGES = {33--90},
 PUBLISHER = {Soc. Math. France, Paris},
      YEAR = {2016},
   MRCLASS = {57M27 (57M25 57N10)},
  MRNUMBER = {3617632},
MRREVIEWER = {Christine Lescop},
}

@article {KirbyMelvin,
    AUTHOR = {Kirby, Robion and Melvin, Paul},
     TITLE = {The {$3$}-manifold invariants of {W}itten and
              {R}eshetikhin-{T}uraev for sl($2$,C)},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {105},
      YEAR = {1991},
    NUMBER = {3},
     PAGES = {473--545},
      ISSN = {0020-9910},
   MRCLASS = {57M25 (17B37 57N10)},
  MRNUMBER = {1117149},
MRREVIEWER = {Louis H. Kauffman},
       DOI = {10.1007/BF01232277},
       URL = {https://doi.org/10.1007/BF01232277},
}

@article {AndersenHimpel12,
    AUTHOR = {Andersen, J. E. and Himpel, Benjamin},
     TITLE = {The {W}itten-{R}eshetikhin-{T}uraev invariants of finite order
              mapping tori {II}},
   JOURNAL = {Quantum Topol.},
  FJOURNAL = {Quantum Topology},
    VOLUME = {3},
      YEAR = {2012},
    NUMBER = {3-4},
     PAGES = {377--421},
      ISSN = {1663-487X},
   MRCLASS = {57M27 (53D50 57R56 58J28 58J30)},
  MRNUMBER = {2928090},
MRREVIEWER = {Daniel D. Moskovich},
       DOI = {10.4171/qt/33},
       URL = {https://doi.org/10.4171/qt/33},
}

@incollection {AndersenKashaev15,
    AUTHOR = {Andersen, J. E. and Kashaev, R.},
     TITLE = {Faddeev's quantum dilogarithm and state-integrals on shaped
              triangulations},
 BOOKTITLE = {Mathematical aspects of quantum field theories},
    SERIES = {Math. Phys. Stud.},
     PAGES = {133--152},
 PUBLISHER = {Springer, Cham},
      YEAR = {2015},
   MRCLASS = {81T45 (57R56 81T30)},
  MRNUMBER = {3330241},
MRREVIEWER = {Giuseppe Nardelli},
}

@article {AndersenKashaev14b,
    AUTHOR = {Andersen, J. E. and Kashaev, R.},
     TITLE = {A {TQFT} from {Q}uantum {T}eichm\"{u}ller theory},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {330},
      YEAR = {2014},
    NUMBER = {3},
     PAGES = {887--934},
      ISSN = {0010-3616},
   MRCLASS = {81T45 (30F60 32G15 37F30 57R56 81Q20)},
  MRNUMBER = {3227503},
MRREVIEWER = {Daniel D. Moskovich},
       DOI = {10.1007/s00220-014-2073-2},
       URL = {https://doi.org/10.1007/s00220-014-2073-2},
}

@ARTICLE{AndersenKashaev18,
   author = {Andersen, J.E. and Kashaev, R.},
    title = "{{T}he {T}eichmüller {TQFT}}",
  journal = {Proceedings of ICM, Rio de Janeiro},
     year = 2018,
  
}

@ARTICLE{Sauzin07,
   author = {{Sauzin}, D.},
    title = "{Resurgent functions and splitting problems}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {0706.0137},
 primaryClass = "math.DS",
 keywords = {Mathematics - Dynamical Systems},
     year = 2007,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2007arXiv0706.0137S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book {C.09,
    AUTHOR = {Costin, Ovidiu},
     TITLE = {Asymptotics and {B}orel summability},
    SERIES = {Chapman \& Hall/CRC Monographs and Surveys in Pure and Applied
              Mathematics},
    VOLUME = {141},
 PUBLISHER = {CRC Press, Boca Raton, FL},
      YEAR = {2009},
     PAGES = {xiv+250},
      ISBN = {978-1-4200-7031-6},
   MRCLASS = {34-02 (34M30 34M37 34M40 34M55 39A11 40G10)},
  MRNUMBER = {2474083},
MRREVIEWER = {B. L. J. Braaksma},
}

@ARTICLE{Dorigoni14,
   author = {{Dorigoni}, D.},
    title = "{An Introduction to Resurgence, Trans-Series and Alien Calculus}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1411.3585},
 primaryClass = "hep-th",
 keywords = {High Energy Physics - Theory},
     year = 2014,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1411.3585D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{AndersenBorotOrantin17,
   author = {{Andersen}, J. E. and {Borot}, G. and {Orantin}, N.},
    title = "{Geometric recursion}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1711.04729},
 primaryClass = "math.GT",
 keywords = {Mathematics - Geometric Topology, Mathematical Physics, 51P05, 81Q30},
     year = 2017,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv171104729E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book {MitschiSauzin16,
    AUTHOR = {Mitschi, C. and Sauzin, D.},
     TITLE = {Divergent series, summability and resurgence. {I}},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {2153},
      NOTE = {Monodromy and resurgence,
              With a foreword by Jean-Pierre Ramis and a preface by \'{E}ric
              Delabaere, Mich\`ele Loday-Richaud, Claude Mitschi and David
              Sauzin},
 PUBLISHER = {Springer, [Cham]},
      YEAR = {2016},
     PAGES = {xxi+298},
      ISBN = {978-3-319-28735-5; 978-3-319-28736-2},
   MRCLASS = {40-02 (30B40 34M35 37F10 40A05)},
  MRNUMBER = {3526111},
MRREVIEWER = {Francisco Marcell\'{a}n},
       DOI = {10.1007/978-3-319-28736-2},
       URL = {https://doi.org/10.1007/978-3-319-28736-2},
}

@article {Curtis03,
    AUTHOR = {Curtis, C. L.},
     TITLE = {Erratum to: ``{A}n intersection theory count of the {$\text{
              SL}_2({\Bbb C})$}-representations of the fundamental group
              of a 3-manifold'' [{T}opology { 40} (2001), no. 4,
              773--787; {MR}1851563 (2002k:57022)]},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {42},
      YEAR = {2003},
    NUMBER = {4},
     PAGES = {929},
      ISSN = {0040-9383},
   MRCLASS = {57M27 (57M25 57N10)},
  MRNUMBER = {1958534},
       DOI = {10.1016/S0040-9383(02)00101-5},
       URL = {https://doi.org/10.1016/S0040-9383(02)00101-5},
}

@article {Curtis01,
    AUTHOR = {Curtis, C. L.},
     TITLE = {An intersection theory count of the {$\text{SL}_2({\Bbb
              C})$}-representations of the fundamental group of a
              {$3$}-manifold},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {40},
      YEAR = {2001},
    NUMBER = {4},
     PAGES = {773--787},
      ISSN = {0040-9383},
   MRCLASS = {57M27 (57M25 57N10)},
  MRNUMBER = {1851563},
MRREVIEWER = {Hans U. Boden},
       DOI = {10.1016/S0040-9383(99)00083-X},
       URL = {https://doi.org/10.1016/S0040-9383(99)00083-X},
}

@book {Thurston97,
    AUTHOR = {Thurston, W P.},
     TITLE = {Three-dimensional geometry and topology. {V}ol. 1},
    SERIES = {Princeton Mathematical Series},
    VOLUME = {35},
      NOTE = {Edited by Silvio Levy},
 PUBLISHER = {Princeton University Press, Princeton, NJ},
      YEAR = {1997},
     PAGES = {x+311},
      ISBN = {0-691-08304-5},
   MRCLASS = {57M50 (53A35 57M25 57M60 57N10)},
  MRNUMBER = {1435975},
MRREVIEWER = {Athanase Papadopoulos},
}

@book {Ratcliffe,
    AUTHOR = {Ratcliffe, John G.},
     TITLE = {Foundations of hyperbolic manifolds},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {149},
 PUBLISHER = {Springer-Verlag, New York},
      YEAR = {1994},
     PAGES = {xii+747},
      ISBN = {0-387-94348-X},
   MRCLASS = {57M50 (20H10 30F40 51M10)},
  MRNUMBER = {1299730},
MRREVIEWER = {Colin C. Adams},
       DOI = {10.1007/978-1-4757-4013-4},
       URL = {https://doi.org/10.1007/978-1-4757-4013-4},
}

@article {Klassen91,
    AUTHOR = {Klassen, E. P.},
     TITLE = {Representations of knot groups in {$\text{SU}(2)$}},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {326},
      YEAR = {1991},
    NUMBER = {2},
     PAGES = {795--828},
      ISSN = {0002-9947},
   MRCLASS = {57M05 (57M25)},
  MRNUMBER = {1008696},
MRREVIEWER = {Paul A. Kirk},
       DOI = {10.2307/2001784},
       URL = {https://doi.org/10.2307/2001784},
}

@article {KirkKlassen91,
    AUTHOR = {Kirk, P. A. and Klassen, E. P.},
     TITLE = {Representation spaces of {S}eifert fibered homology spheres},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {30},
      YEAR = {1991},
    NUMBER = {1},
     PAGES = {77--95},
      ISSN = {0040-9383},
   MRCLASS = {57N10 (55N99)},
  MRNUMBER = {1081935},
MRREVIEWER = {Dave Auckly},
       DOI = {10.1016/0040-9383(91)90035-3},
       URL = {https://doi.org/10.1016/0040-9383(91)90035-3},
}

@article {Riley85,
    AUTHOR = {Riley, R.},
     TITLE = {Holomorphically parameterized families of subgroups of {$\text{
              SL}(2,{ C})$}},
   JOURNAL = {Mathematika},
  FJOURNAL = {Mathematika. A Journal of Pure and Applied Mathematics},
    VOLUME = {32},
      YEAR = {1985},
    NUMBER = {2},
     PAGES = {248--264 (1986)},
      ISSN = {0025-5793},
   MRCLASS = {32G15 (11F06 20H20 30F40)},
  MRNUMBER = {834494},
MRREVIEWER = {C. Maclachlan},
       DOI = {10.1112/S0025579300011037},
       URL = {https://doi.org/10.1112/S0025579300011037},
}

@article {Robert84,
    AUTHOR = {Riley, Robert},
     TITLE = {Nonabelian representations of {$2$}-bridge knot groups},
   JOURNAL = {Quart. J. Math. Oxford Ser. (2)},
  FJOURNAL = {The Quarterly Journal of Mathematics. Oxford. Second Series},
    VOLUME = {35},
      YEAR = {1984},
    NUMBER = {138},
     PAGES = {191--208},
      ISSN = {0033-5606},
   MRCLASS = {20F38 (57M25)},
  MRNUMBER = {745421},
MRREVIEWER = {Norbert Wielenberg},
       DOI = {10.1093/qmath/35.2.191},
       URL = {https://doi.org/10.1093/qmath/35.2.191},
}

@ARTICLE{GalassoPaolette18,
   author = {{Galasso}, A. and {Paoletti}, R.},
    title = "{Equivariant Asymptotics of Szeg$\backslash$``$\{$o$\}$ kernels under Hamiltonian $SU(2)$-action}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1805.00637},
 primaryClass = "math.SG",
 keywords = {Mathematics - Symplectic Geometry, Mathematics - Classical Analysis and ODEs, Mathematics - Complex Variables},
     year = 2018,
    month = may,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv180500637G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zeldith03,
   author = {{Zelditch}, S.},
    title = "{Quantum maps and automorphisms}",
  journal = {ArXiv Mathematics e-prints},
   eprint = {math/0307175},
 keywords = {Mathematics - Quantum Algebra, Mathematical Physics},
     year = 2003,
    month = jul,
   adsurl = {http://adsabs.harvard.edu/abs/2003math......7175Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article {Zeldith97,
    AUTHOR = {Zelditch, S.},
     TITLE = {Index and dynamics of quantized contact transformations},
   JOURNAL = {Ann. Inst. Fourier (Grenoble)},
  FJOURNAL = {Universit\'{e} de Grenoble. Annales de l'Institut Fourier},
    VOLUME = {47},
      YEAR = {1997},
    NUMBER = {1},
     PAGES = {305--363},
      ISSN = {0373-0956},
   MRCLASS = {58F06 (35P99 46N50 47G30 58G15 58G25)},
  MRNUMBER = {1437187},
MRREVIEWER = {Alejandro Uribe},
       URL = {http://www.numdam.org/item?id=AIF_1997__47_1_305_0},
}

@article {Bolte98,
    AUTHOR = {Bolte, Jens and Keppeler, Stefan},
     TITLE = {Semiclassical time evolution and trace formula for
              relativistic spin-{$1/2$} particles},
   JOURNAL = {Phys. Rev. Lett.},
  FJOURNAL = {Physical Review Letters},
    VOLUME = {81},
      YEAR = {1998},
    NUMBER = {10},
     PAGES = {1987--1991},
      ISSN = {0031-9007},
   MRCLASS = {81Q20},
  MRNUMBER = {1644088},
       DOI = {10.1103/PhysRevLett.81.1987},
       URL = {https://doi.org/10.1103/PhysRevLett.81.1987},
}

@article {Faddeev94,
    AUTHOR = {Faddeev, L. D.},
     TITLE = {Discrete {H}eisenberg-{W}eyl group and modular group},
   JOURNAL = {Lett. Math. Phys.},
  FJOURNAL = {Letters in Mathematical Physics},
    VOLUME = {34},
      YEAR = {1995},
    NUMBER = {3},
     PAGES = {249--254},
      ISSN = {0377-9017},
   MRCLASS = {46L10 (22D25 22E27 46L60 47D45 47N50 81S05)},
  MRNUMBER = {1345554},
MRREVIEWER = {Alain Valette},
       DOI = {10.1007/BF01872779},
       URL = {https://doi.org/10.1007/BF01872779},
}

@article {FaddeevKashaev94,
    AUTHOR = {Faddeev, L. D. and Kashaev, R. M.},
     TITLE = {Quantum dilogarithm},
   JOURNAL = {Modern Phys. Lett. A},
  FJOURNAL = {Modern Physics Letters A. Particles and Fields, Gravitation,
              Cosmology, Nuclear Physics},
    VOLUME = {9},
      YEAR = {1994},
    NUMBER = {5},
     PAGES = {427--434},
      ISSN = {0217-7323},
   MRCLASS = {11Z05 (33B99 81R10 81S05 81T40 82B20 82B23)},
  MRNUMBER = {1264393},
MRREVIEWER = {Yas-Hiro Quano},
       DOI = {10.1142/S0217732394000447},
       URL = {https://doi.org/10.1142/S0217732394000447},
}

@article {AndersenKoldHansen,
    AUTHOR = {Andersen, J. E. and Hansen, S. K.},
     TITLE = {Asymptotics of the quantum invariants for surgeries on the
              figure 8 knot},
   JOURNAL = {J. Knot Theory Ramifications},
  FJOURNAL = {Journal of Knot Theory and its Ramifications},
    VOLUME = {15},
      YEAR = {2006},
    NUMBER = {4},
     PAGES = {479--548},
      ISSN = {0218-2165},
   MRCLASS = {58J28 (57M25 57M27 58J37)},
  MRNUMBER = {2221531},
MRREVIEWER = {Hitoshi Murakami},
       DOI = {10.1142/S0218216506004555},
       URL = {https://doi.org/10.1142/S0218216506004555},
}

@article {ChernSimons,
    AUTHOR = {Chern, S. S. and Simons, J.},
     TITLE = {Characteristic forms and geometric invariants},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {99},
      YEAR = {1974},
     PAGES = {48--69},
      ISSN = {0003-486X},
   MRCLASS = {57D20},
  MRNUMBER = {0353327},
MRREVIEWER = {R. L. Bishop},
       DOI = {10.2307/1971013},
       URL = {https://doi.org/10.2307/1971013},
}

@incollection {Lawrence95,
    AUTHOR = {Lawrence, R. J.},
     TITLE = {Asymptotic expansions of {W}itten-{R}eshetikhin-{T}uraev
              invariants for some simple {$3$}-manifolds [ {MR}1355900
              (97a:57015)]},
 BOOKTITLE = {R.{C}.{P}. 25, {V}ol. 47 ({S}trasbourg, 1993--1995)},
    SERIES = {Pr\'{e}publ. Inst. Rech. Math. Av.},
    VOLUME = {1995/24},
     PAGES = {151--182},
 PUBLISHER = {Univ. Louis Pasteur, Strasbourg},
      YEAR = {1995},
   MRCLASS = {57N10 (11B68 57M25 58G18)},
  MRNUMBER = {1461311},
}

@book {Walker92,
    AUTHOR = {Walker, Kevin},
     TITLE = {An extension of {C}asson's invariant},
    SERIES = {Annals of Mathematics Studies},
    VOLUME = {126},
 PUBLISHER = {Princeton University Press, Princeton, NJ},
      YEAR = {1992},
     PAGES = {vi+131},
      ISBN = {0-691-08766-0; 0-691-02532-0},
   MRCLASS = {57N10 (11F20 57M25 57R99)},
  MRNUMBER = {1154798},
MRREVIEWER = {Christine Lescop},
       DOI = {10.1515/9781400882465},
       URL = {https://doi.org/10.1515/9781400882465},
}

@article {LMO95,
    AUTHOR = {Le, T. T. Q. and Murakami, H. and Murakami, J. and
              Ohtsuki, T.},
     TITLE = {A three-manifold invariant derived from the universal
              {V}assiliev-{K}ontsevich invariant},
   JOURNAL = {Proc. Japan Acad. Ser. A Math. Sci.},
  FJOURNAL = {Japan Academy. Proceedings. Series A. Mathematical Sciences},
    VOLUME = {71},
      YEAR = {1995},
    NUMBER = {6},
     PAGES = {125--127},
      ISSN = {0386-2194},
   MRCLASS = {57M25},
  MRNUMBER = {1344664},
MRREVIEWER = {Mark R. Woodard},
       URL = {http://projecteuclid.org/euclid.pja/1195510655},
}

@article {LMO99,
    AUTHOR = {Le, T. T. Q. and Murakami, H. and Murakami, J. and
              Ohtsuki, T.},
     TITLE = {A three-manifold invariant via the {K}ontsevich integral},
   JOURNAL = {Osaka J. Math.},
  FJOURNAL = {Osaka Journal of Mathematics},
    VOLUME = {36},
      YEAR = {1999},
    NUMBER = {2},
     PAGES = {365--395},
      ISSN = {0030-6126},
   MRCLASS = {57M27 (57M25 57N10)},
  MRNUMBER = {1736483},
MRREVIEWER = {Christine Lescop},
       URL = {http://projecteuclid.org/euclid.ojm/1200788570},
}

@article {Ohtsuki96b,
    AUTHOR = {Ohtsuki, T.},
     TITLE = {A polynomial invariant of rational homology {$3$}-spheres},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {123},
      YEAR = {1996},
    NUMBER = {2},
     PAGES = {241--257},
      ISSN = {0020-9910},
   MRCLASS = {57N10 (57M25)},
  MRNUMBER = {1374199},
MRREVIEWER = {Zhenghan Wang},
       DOI = {10.1007/s002220050025},
       URL = {https://doi.org/10.1007/s002220050025},
}

@article {Ohtsuki96a,
    AUTHOR = {Ohtsuki, T.},
     TITLE = {Finite type invariants of integral homology {$3$}-spheres},
   JOURNAL = {J. Knot Theory Ramifications},
  FJOURNAL = {Journal of Knot Theory and its Ramifications},
    VOLUME = {5},
      YEAR = {1996},
    NUMBER = {1},
     PAGES = {101--115},
      ISSN = {0218-2165},
   MRCLASS = {57N10 (57M25)},
  MRNUMBER = {1373813},
MRREVIEWER = {Zhenghan Wang},
       DOI = {10.1142/S0218216596000084},
       URL = {https://doi.org/10.1142/S0218216596000084},
}

@article {Ohtsuki95,
    AUTHOR = {Ohtsuki, T.},
     TITLE = {A polynomial invariant of integral homology {$3$}-spheres},
   JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
  FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical
              Society},
    VOLUME = {117},
      YEAR = {1995},
    NUMBER = {1},
     PAGES = {83--112},
      ISSN = {0305-0041},
   MRCLASS = {57N10 (17B37)},
  MRNUMBER = {1297897},
MRREVIEWER = {S. V. Duzhin},
       DOI = {10.1017/S0305004100072935},
       URL = {https://doi.org/10.1017/S0305004100072935},
}

@article {BoileauZieschang,
    AUTHOR = {Boileau, M. and Zieschang, H.},
     TITLE = {Heegaard genus of closed orientable {S}eifert {$3$}-manifolds},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {76},
      YEAR = {1984},
    NUMBER = {3},
     PAGES = {455--468},
      ISSN = {0020-9910},
   MRCLASS = {57N10},
  MRNUMBER = {746538},
MRREVIEWER = {Klaus Johannson},
       DOI = {10.1007/BF01388469},
       URL = {https://doi.org/10.1007/BF01388469},
}


@article {JeffreyWeitsman93,
    AUTHOR = {Jeffrey, Lisa C. and Weitsman, Jonathan},
     TITLE = {Half density quantization of the moduli space of flat
              connections and {W}itten's semiclassical manifold invariants},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {32},
      YEAR = {1993},
    NUMBER = {3},
     PAGES = {509--529},
      ISSN = {0040-9383},
   MRCLASS = {58F06 (57R57 58D27)},
  MRNUMBER = {1231958},
MRREVIEWER = {Daniel S. Freed},
       DOI = {10.1016/0040-9383(93)90003-E},
       URL = {https://doi.org/10.1016/0040-9383(93)90003-E},
}
@article {JeffreyWeitsman92,
    AUTHOR = {Jeffrey, Lisa C. and Weitsman, Jonathan},
     TITLE = {Bohr-{S}ommerfeld orbits in the moduli space of flat
              connections and the {V}erlinde dimension formula},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {150},
      YEAR = {1992},
    NUMBER = {3},
     PAGES = {593--630},
      ISSN = {0010-3616},
   MRCLASS = {58F06 (53C07 58D27 81S10 81T40)},
  MRNUMBER = {1204322},
MRREVIEWER = {Matthias Blau},
       URL = {http://projecteuclid.org/euclid.cmp/1104251961},
}

@article {Lickorish88,
    AUTHOR = {Lickorish, W. B. R.},
     TITLE = {Polynomials for links},
   JOURNAL = {Bull. London Math. Soc.},
  FJOURNAL = {The Bulletin of the London Mathematical Society},
    VOLUME = {20},
      YEAR = {1988},
    NUMBER = {6},
     PAGES = {558--588},
      ISSN = {0024-6093},
   MRCLASS = {57M25},
  MRNUMBER = {980759},
MRREVIEWER = {J\'{o}zef H. Przytycki},
       DOI = {10.1112/blms/20.6.558},
       URL = {https://doi.org/10.1112/blms/20.6.558},
}

@incollection {KirillovReshetikhin,
    AUTHOR = {Kirillov, A. N. and Reshetikhin, N. Yu.},
     TITLE = {Representations of the algebra {${U}_q(\text{
              sl}(2)),\;q$}-orthogonal polynomials and invariants of links},
 BOOKTITLE = {Infinite-dimensional {L}ie algebras and groups
              ({L}uminy-{M}arseille, 1988)},
    SERIES = {Adv. Ser. Math. Phys.},
    VOLUME = {7},
     PAGES = {285--339},
 PUBLISHER = {World Sci. Publ., Teaneck, NJ},
      YEAR = {1989},
   MRCLASS = {17B35 (05A30 16A24 33A65 57M25 81C40)},
  MRNUMBER = {1026957},
MRREVIEWER = {Bruce W. Westbury},
}

@book {Olver,
    AUTHOR = {Olver, F. W. J.},
     TITLE = {Asymptotics and special functions},
      NOTE = {Computer Science and Applied Mathematics},
 PUBLISHER = {Academic Press [A subsidiary of Harcourt Brace Jovanovich,
              Publishers], New York-London},
      YEAR = {1974},
     PAGES = {xvi+572},
   MRCLASS = {41A60},
  MRNUMBER = {0435697},
MRREVIEWER = {Norman Bleistein},
}

@incollection {Hikami11,
    AUTHOR = {Hikami, Kazuhiro},
     TITLE = {Decomposition of {W}itten-{R}eshetikhin-{T}uraev invariant:
              linking pairing and modular forms},
 BOOKTITLE = {Chern-{S}imons gauge theory: 20 years after},
    SERIES = {AMS/IP Stud. Adv. Math.},
    VOLUME = {50},
     PAGES = {131--151},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2011},
   MRCLASS = {58J28 (11F23 11F37 11F67 57M27)},
  MRNUMBER = {2809450},
MRREVIEWER = {Kazuo Habiro},
}

@article {KirkKlassen91,
    AUTHOR = {Kirk, P. A. and Klassen, E. P.},
     TITLE = {Representation spaces of {S}eifert fibered homology spheres},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {30},
      YEAR = {1991},
    NUMBER = {1},
     PAGES = {77--95},
      ISSN = {0040-9383},
   MRCLASS = {57N10 (55N99)},
  MRNUMBER = {1081935},
MRREVIEWER = {Dave Auckly},
       DOI = {10.1016/0040-9383(91)90035-3},
       URL = {https://doi.org/10.1016/0040-9383(91)90035-3},
}

@book {Dingle73,
    AUTHOR = {Dingle, R. B.},
     TITLE = {Asymptotic expansions: their derivation and interpretation},
 PUBLISHER = {Academic Press [A subsidiary of Harcourt Brace Jovanovich,
              Publishers], London-New York},
      YEAR = {1973},
     PAGES = {xv+521},
   MRCLASS = {41A60},
  MRNUMBER = {0499926},
}

@article {Kashaev97,
    AUTHOR = {Kashaev, R. M.},
     TITLE = {The hyperbolic volume of knots from the quantum dilogarithm},
   JOURNAL = {Lett. Math. Phys.},
  FJOURNAL = {Letters in Mathematical Physics},
    VOLUME = {39},
      YEAR = {1997},
    NUMBER = {3},
     PAGES = {269--275},
      ISSN = {0377-9017},
   MRCLASS = {57M25 (33E20 57N10)},
  MRNUMBER = {1434238},
MRREVIEWER = {Colin C. Adams},
       DOI = {10.1023/A:1007364912784},
       URL = {https://doi.org/10.1023/A:1007364912784},
}

@article {FintushelStern90,
    AUTHOR = {Fintushel, R. and Stern, R. J.},
     TITLE = {Instanton homology of {S}eifert fibred homology three spheres},
   JOURNAL = {Proc. London Math. Soc. (3)},
  FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
    VOLUME = {61},
      YEAR = {1990},
    NUMBER = {1},
     PAGES = {109--137},
      ISSN = {0024-6115},
   MRCLASS = {57R19 (55N35 57N10 57R20 58E05)},
  MRNUMBER = {1051101},
MRREVIEWER = {Dave Auckly},
       DOI = {10.1112/plms/s3-61.1.109},
       URL = {https://doi.org/10.1112/plms/s3-61.1.109},
}

@article {Hikami05,
    AUTHOR = {Hikami, Kazuhiro},
     TITLE = {On the quantum invariant for the {B}rieskorn homology spheres},
   JOURNAL = {Internat. J. Math.},
  FJOURNAL = {International Journal of Mathematics},
    VOLUME = {16},
      YEAR = {2005},
    NUMBER = {6},
     PAGES = {661--685},
      ISSN = {0129-167X},
   MRCLASS = {57M27 (11F23 11F67 57N10 58J28)},
  MRNUMBER = {2153489},
MRREVIEWER = {Ruth Lawrence},
       DOI = {10.1142/S0129167X05003004},
       URL = {https://doi.org/10.1142/S0129167X05003004},
}

@ARTICLE{Chun17,
   author = {{Chun}, S.},
    title = "{A resurgence analysis of the $SU(2)$ Chern-Simons partition functions on a Brieskorn homology sphere $\Sigma(2,5,7)$}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1701.03528},
 primaryClass = "hep-th",
 keywords = {High Energy Physics - Theory, Mathematical Physics, Mathematics - Geometric Topology},
     year = 2017,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170103528C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{AndersenKashaev14,
   author = {{Andersen}, J. E. and {Kashaev}, R.},
    title = "{Complex Quantum Chern-Simons}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1409.1208},
 primaryClass = "math.QA",
 keywords = {Mathematics - Quantum Algebra},
     year = 2014,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1409.1208E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kontsevich12,
  author = {Kontsevich, M.},
  title = {Resurgence from the path integral perspective},
  journal = {Perimeter Institute},
  year = {2015}
}

@ARTICLE{DunneUnsal15,
   author = {{Dunne}, G.~V. and {Unsal}, M.},
    title = "{What is QFT? Resurgent trans-series, Lefschetz thimbles, and new exact saddles}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1511.05977},
 primaryClass = "hep-lat",
 keywords = {High Energy Physics - Lattice, High Energy Physics - Theory},
     year = 2015,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2015arXiv151105977D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book {Ecalle81b,
    AUTHOR = {\'{E}calle, J.},
     TITLE = {Les fonctions r\'{e}surgentes. {T}ome {II}},
    SERIES = {Publications Math\'{e}matiques d'Orsay 81 [Mathematical
              Publications of Orsay 81]},
    VOLUME = {6},
      NOTE = {Les fonctions r\'{e}surgentes appliqu\'{e}es \`a l'it\'{e}ration. [Resurgent
              functions applied to iteration]},
 PUBLISHER = {Universit\'{e} de Paris-Sud, D\'{e}partement de Math\'{e}matique, Orsay},
      YEAR = {1981},
     PAGES = {248--531},
   MRCLASS = {30F99 (22E65 39B99)},
  MRNUMBER = {670418},
MRREVIEWER = {Carlos A. Berenstein},
}

@book {Ecalle81a,
    AUTHOR = {\'{E}calle, J.},
     TITLE = {Les fonctions r\'{e}surgentes. {T}ome {I}},
    SERIES = {Publications Math\'{e}matiques d'Orsay 81 [Mathematical
              Publications of Orsay 81]},
    VOLUME = {5},
      NOTE = {Les alg\`ebres de fonctions r\'{e}surgentes. [The algebras of
              resurgent functions],
              With an English foreword},
 PUBLISHER = {Universit\'{e} de Paris-Sud, D\'{e}partement de Math\'{e}matique, Orsay},
      YEAR = {1981},
     PAGES = {247},
   MRCLASS = {30F99 (39B99)},
  MRNUMBER = {670417},
MRREVIEWER = {Carlos A. Berenstein},
}

@incollection {Witten11,
    AUTHOR = {Witten, E.},
     TITLE = {Analytic continuation of {C}hern-{S}imons theory},
 BOOKTITLE = {Chern-{S}imons gauge theory: 20 years after},
    SERIES = {AMS/IP Stud. Adv. Math.},
    VOLUME = {50},
     PAGES = {347--446},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2011},
   MRCLASS = {81T45 (58J28)},
  MRNUMBER = {2809462},
MRREVIEWER = {Piotr Su\l kowski},
}

@article {BodenCurtis06,
    AUTHOR = {Boden, H. U. and Curtis, C. L.},
     TITLE = {The {$\text{SL}_2(\Bbb C)$} {C}asson invariant for {S}eifert
              fibered homology spheres and surgeries on twist knots},
   JOURNAL = {J. Knot Theory Ramifications},
  FJOURNAL = {Journal of Knot Theory and its Ramifications},
    VOLUME = {15},
      YEAR = {2006},
    NUMBER = {7},
     PAGES = {813--837},
      ISSN = {0218-2165},
   MRCLASS = {57M27 (57M25)},
  MRNUMBER = {2264157},
MRREVIEWER = {Ryan D. Budney},
       DOI = {10.1142/S0218216506004762},
       URL = {https://doi.org/10.1142/S0218216506004762},
}

@article {Auckly94,
    AUTHOR = {Auckly, David R.},
     TITLE = {Topological methods to compute {C}hern-{S}imons invariants},
   JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
  FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical
              Society},
    VOLUME = {115},
      YEAR = {1994},
    NUMBER = {2},
     PAGES = {229--251},
      ISSN = {0305-0041},
   MRCLASS = {57N10 (57M99 57R57)},
  MRNUMBER = {1277058},
MRREVIEWER = {Yongwu Rong},
       DOI = {10.1017/S0305004100072066},
       URL = {https://doi.org/10.1017/S0305004100072066},
}

@article {KirkKlassen91,
    AUTHOR = {Kirk, P. A. and Klassen, E. P.},
     TITLE = {Representation spaces of {S}eifert fibered homology spheres},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {30},
      YEAR = {1991},
    NUMBER = {1},
     PAGES = {77--95},
      ISSN = {0040-9383},
   MRCLASS = {57N10 (55N99)},
  MRNUMBER = {1081935},
MRREVIEWER = {Dave Auckly},
       DOI = {10.1016/0040-9383(91)90035-3},
       URL = {https://doi.org/10.1016/0040-9383(91)90035-3},
}

@article {KirkKlassen90,
    AUTHOR = {Kirk, P. A. and Klassen, E. P.},
     TITLE = {Chern-{S}imons invariants of {$3$}-manifolds and
              representation spaces of knot groups},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {287},
      YEAR = {1990},
    NUMBER = {2},
     PAGES = {343--367},
      ISSN = {0025-5831},
   MRCLASS = {57M99 (53C05)},
  MRNUMBER = {1054574},
MRREVIEWER = {Michael Kapovich},
       DOI = {10.1007/BF01446898},
       URL = {https://doi.org/10.1007/BF01446898},
}

@article {Killingback92,
    AUTHOR = {Killingback, T. P.},
     TITLE = {Quantization of {$\text{SL}(2,{ R})$} {C}hern-{S}imons
              theory},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {145},
      YEAR = {1992},
    NUMBER = {1},
     PAGES = {1--16},
      ISSN = {0010-3616},
   MRCLASS = {58F06 (22E70 32G81 81S10 81T13)},
  MRNUMBER = {1155281},
MRREVIEWER = {Michael Thaddeus},
       URL = {http://projecteuclid.org/euclid.cmp/1104249532},
}

@ARTICLE{KitanoYamaguchi16,
   author = {{Kitano}, T. and {Yamaguchi}, Y.},
    title = "{SL(2;R)-representations of a Brieskorn homology 3-sphere}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1602.07503},
 primaryClass = "math.GT",
 keywords = {Mathematics - Geometric Topology, Mathematics - General Topology},
     year = 2016,
    month = feb,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160207503K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@incollection {Hikami11,
    AUTHOR = {Hikami, Kazuhiro},
     TITLE = {Decomposition of {W}itten-{R}eshetikhin-{T}uraev invariant:
              linking pairing and modular forms},
 BOOKTITLE = {Chern-{S}imons gauge theory: 20 years after},
    SERIES = {AMS/IP Stud. Adv. Math.},
    VOLUME = {50},
     PAGES = {131--151},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2011},
   MRCLASS = {58J28 (11F23 11F37 11F67 57M27)},
  MRNUMBER = {2809450},
MRREVIEWER = {Kazuo Habiro},
}

@article {BerryHowls90,
    AUTHOR = {Berry, M. V. and Howls, C. J.},
     TITLE = {Hyperasymptotics},
   JOURNAL = {Proc. Roy. Soc. London Ser. A},
  FJOURNAL = {Proceedings of the Royal Society. London. Series A.
              Mathematical, Physical and Engineering Sciences},
    VOLUME = {430},
      YEAR = {1990},
    NUMBER = {1880},
     PAGES = {653--668},
      ISSN = {0962-8444},
   MRCLASS = {34E20 (41A60 65D99 65L99)},
  MRNUMBER = {1070081},
MRREVIEWER = {F. W. J. Olver},
       DOI = {10.1098/rspa.1990.0111},
       URL = {https://doi.org/10.1098/rspa.1990.0111},
}

@article {BerryHowls91,
    AUTHOR = {Berry, M. V. and Howls, C. J.},
     TITLE = {Hyperasymptotics for integrals with saddles},
   JOURNAL = {Proc. Roy. Soc. London Ser. A},
  FJOURNAL = {Proceedings of the Royal Society. London. Series A.
              Mathematical, Physical and Engineering Sciences},
    VOLUME = {434},
      YEAR = {1991},
    NUMBER = {1892},
     PAGES = {657--675},
      ISSN = {0962-8444},
   MRCLASS = {41A60 (30E15 65D32)},
  MRNUMBER = {1126872},
MRREVIEWER = {Andreas Guthmann},
       DOI = {10.1098/rspa.1991.0119},
       URL = {https://doi.org/10.1098/rspa.1991.0119},
}

@article {Howls97,
    AUTHOR = {Howls, C. J.},
     TITLE = {Hyperasymptotics for multidimensional integrals, exact
              remainder terms and the global connection problem},
   JOURNAL = {Proc. Roy. Soc. London Ser. A},
  FJOURNAL = {Proceedings of the Royal Society. London. Series A.
              Mathematical, Physical and Engineering Sciences},
    VOLUME = {453},
      YEAR = {1997},
    NUMBER = {1966},
     PAGES = {2271--2294},
      ISSN = {0962-8444},
   MRCLASS = {58G18 (44A10)},
  MRNUMBER = {1480118},
MRREVIEWER = {F. Ursell},
       DOI = {10.1098/rspa.1997.0122},
       URL = {https://doi.org/10.1098/rspa.1997.0122},
}

@article {BennetHowlsNemesDaalhuis,
    AUTHOR = {Bennett, T. and Howls, C. J. and Nemes, G. and Olde Daalhuis,
              A. B.},
     TITLE = {Globally exact asymptotics for integrals with arbitrary order
              saddles},
   JOURNAL = {SIAM J. Math. Anal.},
  FJOURNAL = {SIAM Journal on Mathematical Analysis},
    VOLUME = {50},
      YEAR = {2018},
    NUMBER = {2},
     PAGES = {2144--2177},
      ISSN = {0036-1410},
   MRCLASS = {41A60 (41A80 58K05)},
  MRNUMBER = {3787779},
MRREVIEWER = {Jos\'e Luis L\'opez},
       DOI = {10.1137/17M1154217},
       URL = {https://doi.org/10.1137/17M1154217},
}

@article {DelabaereHowls02,
    AUTHOR = {Delabaere, E. and Howls, C. J.},
     TITLE = {Global asymptotics for multiple integrals with boundaries},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {112},
      YEAR = {2002},
    NUMBER = {2},
     PAGES = {199--264},
      ISSN = {0012-7094},
   MRCLASS = {32C30 (41A60)},
  MRNUMBER = {1894360},
MRREVIEWER = {P. Lappan},
       DOI = {10.1215/S0012-9074-02-11221-6},
       URL = {https://doi.org/10.1215/S0012-9074-02-11221-6},
}

@article {LawrenceRon06,
    AUTHOR = {Lawrence, R. and Ron, O.},
     TITLE = {On {H}abiro's cyclotomic expansions of the {O}htsuki
              invariant},
   JOURNAL = {J. Knot Theory Ramifications},
  FJOURNAL = {Journal of Knot Theory and its Ramifications},
    VOLUME = {15},
      YEAR = {2006},
    NUMBER = {6},
     PAGES = {661--680},
      ISSN = {0218-2165},
   MRCLASS = {57M27 (11Z05)},
  MRNUMBER = {2253829},
MRREVIEWER = {Hitoshi Murakami},
       DOI = {10.1142/S0218216506004737},
       URL = {https://doi.org/10.1142/S0218216506004737},
}

@article {Garoufalidis98,
    AUTHOR = {Garoufalidis, S.},
     TITLE = {Applications of quantum invariants in low-dimensional
              topology},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {37},
      YEAR = {1998},
    NUMBER = {1},
     PAGES = {219--224},
      ISSN = {0040-9383},
   MRCLASS = {57N10},
  MRNUMBER = {1480887},
MRREVIEWER = {Gretchen Wright},
       DOI = {10.1016/S0040-9383(97)00009-8},
       URL = {https://doi.org/10.1016/S0040-9383(97)00009-8},
}

@article {LawrenceRozansky,
    AUTHOR = {Lawrence, R. and Rozansky, L.},
     TITLE = {Witten-{R}eshetikhin-{T}uraev invariants of {S}eifert
              manifolds},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {205},
      YEAR = {1999},
    NUMBER = {2},
     PAGES = {287--314},
      ISSN = {0010-3616},
   MRCLASS = {58J28 (57M27 57R57 58J37)},
  MRNUMBER = {1712599},
       DOI = {10.1007/s002200050678},
       URL = {https://doi.org/10.1007/s002200050678},
}

@article {DelabaereHowls02,
    AUTHOR = {Delabaere, E. and Howls, C. J.},
     TITLE = {Global asymptotics for multiple integrals with boundaries},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {112},
      YEAR = {2002},
    NUMBER = {2},
     PAGES = {199--264},
      ISSN = {0012-7094},
   MRCLASS = {32C30 (41A60)},
  MRNUMBER = {1894360},
MRREVIEWER = {P. Lappan},
       DOI = {10.1215/S0012-9074-02-11221-6},
       URL = {https://doi.org/10.1215/S0012-9074-02-11221-6},
}

@article {BerryHowls90,
    AUTHOR = {Berry, M. V. and Howls, C. J.},
     TITLE = {Hyperasymptotics},
   JOURNAL = {Proc. Roy. Soc. London Ser. A},
  FJOURNAL = {Proceedings of the Royal Society. London. Series A.
              Mathematical, Physical and Engineering Sciences},
    VOLUME = {430},
      YEAR = {1990},
    NUMBER = {1880},
     PAGES = {653--668},
      ISSN = {0962-8444},
   MRCLASS = {34E20 (41A60 65D99 65L99)},
  MRNUMBER = {1070081},
MRREVIEWER = {F. W. J. Olver},
       DOI = {10.1098/rspa.1990.0111},
       URL = {https://doi.org/10.1098/rspa.1990.0111},
}

@article {BerryHowls91,
    AUTHOR = {Berry, M. V. and Howls, C. J.},
     TITLE = {Hyperasymptotics for integrals with saddles},
   JOURNAL = {Proc. Roy. Soc. London Ser. A},
  FJOURNAL = {Proceedings of the Royal Society. London. Series A.
              Mathematical, Physical and Engineering Sciences},
    VOLUME = {434},
      YEAR = {1991},
    NUMBER = {1892},
     PAGES = {657--675},
      ISSN = {0962-8444},
   MRCLASS = {41A60 (30E15 65D32)},
  MRNUMBER = {1126872},
MRREVIEWER = {Andreas Guthmann},
       DOI = {10.1098/rspa.1991.0119},
       URL = {https://doi.org/10.1098/rspa.1991.0119},
}

@incollection {Pham83,
    AUTHOR = {Pham, F.},
     TITLE = {Vanishing homologies and the {$n$} variable saddlepoint
              method},
 BOOKTITLE = {Singularities, {P}art 2 ({A}rcata, {C}alif., 1981)},
    SERIES = {Proc. Sympos. Pure Math.},
    VOLUME = {40},
     PAGES = {319--333},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {1983},
   MRCLASS = {32C40 (41A60 58G15)},
  MRNUMBER = {713258},
MRREVIEWER = {M. Sebastiani},
}

@ARTICLE{TudorGaroufalidis15,
       author = {{Dimofte}, Tudor and {Garoufalidis}, Stavros},
        title = "{Quantum modularity and complex Chern-Simons theory}",
      journal = {arXiv e-prints},
     keywords = {Mathematics - Geometric Topology, High Energy Physics - Theory},
         year = "2015",
        month = "Nov",
          eid = {arXiv:1511.05628},
        pages = {arXiv:1511.05628},
archivePrefix = {arXiv},
       eprint = {1511.05628},
 primaryClass = {math.GT},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015arXiv151105628D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article {Garoufalidis08,
    AUTHOR = {Garoufalidis, S.},
     TITLE = {Chern-{S}imons theory, analytic continuation and arithmetic},
   JOURNAL = {Acta Math. Vietnam.},
  FJOURNAL = {Acta Mathematica Vietnamica},
    VOLUME = {33},
      YEAR = {2008},
    NUMBER = {3},
     PAGES = {335--362},
      ISSN = {0251-4184},
   MRCLASS = {58J28 (57M27)},
  MRNUMBER = {2501849},
MRREVIEWER = {Hitoshi Murakami},
}

@article {GaroufalidisLe08,
    AUTHOR = {Garoufalidis, S. and L\^e, T. T. Q.},
     TITLE = {Gevrey series in quantum topology},
   JOURNAL = {J. Reine Angew. Math.},
  FJOURNAL = {Journal f\"ur die Reine und Angewandte Mathematik. [Crelle's
              Journal]},
    VOLUME = {618},
      YEAR = {2008},
     PAGES = {169--195},
      ISSN = {0075-4102},
   MRCLASS = {57M27},
  MRNUMBER = {2404749},
MRREVIEWER = {Qingtao Chen},
       DOI = {10.1515/CRELLE.2008.036},
       URL = {https://doi.org/10.1515/CRELLE.2008.036},
}

@article {CostinGaroufalidis09,
    AUTHOR = {Costin, Ovidiu and Garoufalidis, S.},
     TITLE = {Resurgence of the fractional polylogarithms},
   JOURNAL = {Math. Res. Lett.},
  FJOURNAL = {Mathematical Research Letters},
    VOLUME = {16},
      YEAR = {2009},
    NUMBER = {5},
     PAGES = {817--826},
      ISSN = {1073-2780},
   MRCLASS = {33B30 (11G55)},
  MRNUMBER = {2576699},
MRREVIEWER = {Matilde N. Lal\'\i n},
       DOI = {10.4310/MRL.2009.v16.n5.a5},
       URL = {https://doi.org/10.4310/MRL.2009.v16.n5.a5},
}

@article {CostinGaroufalidis08,
    AUTHOR = {Costin, Ovidiu and Garoufalidis, S.},
     TITLE = {Resurgence of the {E}uler-{M}ac{L}aurin summation formula},
   JOURNAL = {Ann. Inst. Fourier (Grenoble)},
  FJOURNAL = {Universit\'e de Grenoble. Annales de l'Institut Fourier},
    VOLUME = {58},
      YEAR = {2008},
    NUMBER = {3},
     PAGES = {893--914},
      ISSN = {0373-0956},
   MRCLASS = {34M30 (34M37 34M40 39A10)},
  MRNUMBER = {2427514},
MRREVIEWER = {Akira Shudo},
       URL = {http://aif.cedram.org/item?id=AIF_2008__58_3_893_0},
}

@article {CostinGaroufalidis11,
    AUTHOR = {Costin, Ovidiu and Garoufalidis, S.},
     TITLE = {Resurgence of the {K}ontsevich-{Z}agier series},
   JOURNAL = {Ann. Inst. Fourier (Grenoble)},
  FJOURNAL = {Universit\'e de Grenoble. Annales de l'Institut Fourier},
    VOLUME = {61},
      YEAR = {2011},
    NUMBER = {3},
     PAGES = {1225--1258},
      ISSN = {0373-0956},
   MRCLASS = {57M27 (11F20 40G10)},
  MRNUMBER = {2918728},
MRREVIEWER = {B. L. J. Braaksma},
       DOI = {10.5802/aif.2639},
       URL = {https://doi.org/10.5802/aif.2639},
}

@ARTICLE{AndersenPetersen18,
   author = {{Andersen}, J. E. and {Petersen}, W. E.},
    title = "{Asymptotic expansions of the Witten-Reshetikhin-Turaev Invariants of Mapping Tori I}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1803.09510},
 primaryClass = "math.DG",
 keywords = {Mathematics - Differential Geometry},
     year = 2018,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv180309510E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{jeffrey1992,
author = "Jeffrey, Lisa C.",
fjournal = "Communications in Mathematical Physics",
journal = "Comm. Math. Phys.",
number = "3",
pages = "563--604",
publisher = "Springer",
title = "Chern-Simons-Witten invariants of lens spaces and torus bundles, and the semiclassical approximation",
url = "https://projecteuclid.org:443/euclid.cmp/1104250751",
volume = "147",
year = "1992"
}

@book {GelfandShilovGeneralizedFunctions,
    AUTHOR = {Gelfand, I. M. and Shilov, G. E.},
     TITLE = {Generalized functions. {V}ol. 2},
      NOTE = {Spaces of fundamental and generalized functions,
              Translated from the Russian by Morris D. Friedman, Amiel
              Feinstein and Christian P. Peltzer},
 PUBLISHER = {Academic Press [Harcourt Brace Jovanovich, Publishers], New
              York-London},
      YEAR = {1968 [1977]},
     PAGES = {x+261},
   MRCLASS = {46FXX},
  MRNUMBER = {0435832},
}

@article {Jones85,
    AUTHOR = {Jones, V. F. R.},
     TITLE = {A polynomial invariant for knots via von {N}eumann algebras},
   JOURNAL = {Bull. Amer. Math. Soc. (N.S.)},
  FJOURNAL = {American Mathematical Society. Bulletin. New Series},
    VOLUME = {12},
      YEAR = {1985},
    NUMBER = {1},
     PAGES = {103--111},
      ISSN = {0273-0979},
   MRCLASS = {57M25 (46L10)},
  MRNUMBER = {766964},
MRREVIEWER = {J. S. Birman},
       DOI = {10.1090/S0273-0979-1985-15304-2},
       URL = {https://doi.org/10.1090/S0273-0979-1985-15304-2},
}

@book {BleisteinHandelsman,
    AUTHOR = {Bleistein, Norman and Handelsman, Richard A.},
     TITLE = {Asymptotic expansions of integrals},
   EDITION = {Second},
 PUBLISHER = {Dover Publications, Inc., New York},
      YEAR = {1986},
     PAGES = {xvi+425},
      ISBN = {0-486-65082-0},
   MRCLASS = {41A60},
  MRNUMBER = {863284},
}

@INPROCEEDINGS{Reshetikhin10,
   author = {{Reshetikhin}, N.},
    title = "{Lectures on Quantization of Gauge Systems}",
 keywords = {Physics},
booktitle = {Lecture Notes in Physics, Berlin Springer Verlag},
     year = 2010,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 807,
archivePrefix = "arXiv",
   eprint = {1008.1411},
 primaryClass = "math-ph",
   editor = {{Boo{\ss}-Bavnbek}, B. and {Esposito}, G. and {Lesch}, M.},
    pages = {125},
      doi = {10.1007/978-3-642-11897-5_3},
   adsurl = {http://adsabs.harvard.edu/abs/2010LNP...807..125R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article {AndersenHansen,
    AUTHOR = {Andersen, J. E. and Hansen, S. K.},
     TITLE = {Asymptotics of the quantum invariants for surgeries on the
              figure 8 knot},
   JOURNAL = {J. Knot Theory Ramifications},
  FJOURNAL = {Journal of Knot Theory and its Ramifications},
    VOLUME = {15},
      YEAR = {2006},
    NUMBER = {4},
     PAGES = {479--548},
      ISSN = {0218-2165},
   MRCLASS = {58J28 (57M25 57M27 58J37)},
  MRNUMBER = {2221531},
MRREVIEWER = {Hitoshi Murakami},
       DOI = {10.1142/S0218216506004555},
       URL = {https://doi.org/10.1142/S0218216506004555},
}

@article {AndersenJoergensen,
    AUTHOR = {Andersen, J. E. and J\o rgensen, S. F.},
     TITLE = {On the {W}itten-{R}eshetikhin-{T}uraev invariants of torus
              bundles},
   JOURNAL = {J. Knot Theory Ramifications},
  FJOURNAL = {Journal of Knot Theory and its Ramifications},
    VOLUME = {24},
      YEAR = {2015},
    NUMBER = {11},
     PAGES = {1550055, 48},
      ISSN = {0218-2165},
   MRCLASS = {57R56 (53D50 57M25 57M27)},
  MRNUMBER = {3413187},
MRREVIEWER = {Haimiao Chen},
       DOI = {10.1142/S0218216515500558},
       URL = {https://doi.org/10.1142/S0218216515500558},
}

@ARTICLE{AndersenBorotOrantin,
   author = {{Andersen}, J. E. and {Borot}, G. and {Orantin}, N.},
    title = "{Geometric recursion}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1711.04729},
 primaryClass = "math.GT",
 keywords = {Mathematics - Geometric Topology, Mathematical Physics, 51P05, 81Q30},
     year = 2017,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv171104729E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article {LawrenceZagier,
    AUTHOR = {Lawrence, Ruth and Zagier, Don},
     TITLE = {Modular forms and quantum invariants of {$3$}-manifolds},
      NOTE = {Sir Michael Atiyah: a great mathematician of the twentieth
              century},
   JOURNAL = {Asian J. Math.},
  FJOURNAL = {Asian Journal of Mathematics},
    VOLUME = {3},
      YEAR = {1999},
    NUMBER = {1},
     PAGES = {93--107},
      ISSN = {1093-6106},
   MRCLASS = {11F23 (11F67 57M27 57N10)},
  MRNUMBER = {1701924},
MRREVIEWER = {Justin D. Roberts},
       DOI = {10.4310/AJM.1999.v3.n1.a5},
       URL = {https://doi.org/10.4310/AJM.1999.v3.n1.a5},
}

@article {BringmannHikamiLovejoy,
    AUTHOR = {Bringmann, Kathrin and Hikami, Kazuhiro and Lovejoy, Jeremy},
     TITLE = {On the modularity of the unified {WRT} invariants of certain
              {S}eifert manifolds},
   JOURNAL = {Adv. in Appl. Math.},
  FJOURNAL = {Advances in Applied Mathematics},
    VOLUME = {46},
      YEAR = {2011},
    NUMBER = {1-4},
     PAGES = {86--93},
      ISSN = {0196-8858},
   MRCLASS = {11F23 (11F27 11F37 57M27)},
  MRNUMBER = {2794015},
MRREVIEWER = {Amanda Folsom},
       DOI = {10.1016/j.aam.2009.12.004},
       URL = {https://doi.org/10.1016/j.aam.2009.12.004},
}

@article {Hikami2005,
    AUTHOR = {Hikami, Kazuhiro},
     TITLE = {Quantum invariant, modular form, and lattice points},
   JOURNAL = {Int. Math. Res. Not.},
  FJOURNAL = {International Mathematics Research Notices},
      YEAR = {2005},
    NUMBER = {3},
     PAGES = {121--154},
      ISSN = {1073-7928},
   MRCLASS = {11F23 (11F37 11P21 57M27 58J28)},
  MRNUMBER = {2130240},
MRREVIEWER = {Ruth Lawrence},
       DOI = {10.1155/IMRN.2005.121},
       URL = {https://doi.org/10.1155/IMRN.2005.121},
}

@article {Hikami2004,
    AUTHOR = {Hikami, Kazuhiro},
     TITLE = {Quantum invariant for torus link and modular forms},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {246},
      YEAR = {2004},
    NUMBER = {2},
     PAGES = {403--426},
      ISSN = {0010-3616},
   MRCLASS = {11F67 (11F23 33D80 57M27)},
  MRNUMBER = {2048564},
MRREVIEWER = {Ruth Lawrence},
       DOI = {10.1007/s00220-004-1046-2},
       URL = {https://doi.org/10.1007/s00220-004-1046-2},
}


@ARTICLE{AP2,
   author = {{Andersen}, J. E. and {Petersen}, W. E.},
    title = "{Asymptotic expansions of the Witten-Reshetikhin-Turaev Invariants of Mapping Tori I}",
  journal = {{T}ransactions of the {A}merican {M}athematical {S}ociety},
  year  = 2018,
}


@ARTICLE{AP3,
   author = {{Andersen}, J. E. and {Petersen}, W. E.},
    title = "{Resurgence Analysis of Quantum Invariants: Seifert Manifolds and Surgeries on The Figure Eight Knot}",
archivePrefix = "arXiv",
   eprint = {1811.05376},
     year = 2018,
    month = November,
}
  journal = {To appear in: ar{X}ive},
   year   =  2018,
   month  =  nov,

}

@ARTICLE{AP4,
   author = {{Andersen}, J. E. and {Petersen}, W. E.},
    title = "{Resurgence Analysis of Quantum Invariants}",
    journal = {To appear on ar{X}ive}
    
}

@ARTICLE{Witten2010,
   author = {{Witten}, E.},
    title = "{Analytic Continuation Of Chern-Simons Theory}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1001.2933},
 primaryClass = "hep-th",
 keywords = {High Energy Physics - Theory},
     year = 2010,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1001.2933W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GukovMarinoPutrov,
   author = {{Gukov}, S. and {Marino}, M. and {Putrov}, P.},
    title = "{Resurgence in complex Chern-Simons theory}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1605.07615},
 primaryClass = "hep-th",
 keywords = {High Energy Physics - Theory, Mathematical Physics, Mathematics - Geometric Topology, Mathematics - Number Theory, Mathematics - Quantum Algebra},
     year = 2016,
    month = may,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160507615G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article {CharlesMarchII,
    AUTHOR = {Charles, L. and March\'e, J.},
     TITLE = {Knot state asymptotics {II}: {W}itten conjecture and
              irreducible representations},
   JOURNAL = {Publ. Math. Inst. Hautes \'Etudes Sci.},
  FJOURNAL = {Publications Math\'ematiques. Institut de Hautes \'Etudes
              Scientifiques},
    VOLUME = {121},
      YEAR = {2015},
     PAGES = {323--361},
      ISSN = {0073-8301},
   MRCLASS = {81T20 (53D50 57M27 57R56)},
  MRNUMBER = {3349835},
MRREVIEWER = {Xin Liu},
       DOI = {10.1007/s10240-015-0069-x},
       URL = {https://doi.org/10.1007/s10240-015-0069-x},
}

@article {CharlesMarhcI,
    AUTHOR = {Charles, L. and March\'e, J.},
     TITLE = {Knot state asymptotics {I}: {AJ} conjecture and {A}belian
              representations},
   JOURNAL = {Publ. Math. Inst. Hautes \'Etudes Sci.},
  FJOURNAL = {Publications Math\'ematiques. Institut de Hautes \'Etudes
              Scientifiques},
    VOLUME = {121},
      YEAR = {2015},
     PAGES = {279--322},
      ISSN = {0073-8301},
   MRCLASS = {81T20 (53D50 57M27 57R56)},
  MRNUMBER = {3349834},
MRREVIEWER = {Xin Liu},
       DOI = {10.1007/s10240-015-0068-y},
       URL = {https://doi.org/10.1007/s10240-015-0068-y},
}

@article {Pauly1,
    AUTHOR = {Pauly, C.},
     TITLE = {Espaces de modules de fibr\'es paraboliques et blocs conformes},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {84},
      YEAR = {1996},
    NUMBER = {1},
     PAGES = {217--235},
      ISSN = {0012-7094},
   MRCLASS = {14D20 (14F05 17B10 81T40)},
  MRNUMBER = {1394754},
MRREVIEWER = {Emma Previato},
       DOI = {10.1215/S0012-7094-96-08408-2},
       URL = {https://doi.org/10.1215/S0012-7094-96-08408-2},
}

@article {MehtaSeshadri,
    AUTHOR = {Mehta, V. B. and Seshadri, C. S.},
     TITLE = {Moduli of vector bundles on curves with parabolic structures},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {248},
      YEAR = {1980},
    NUMBER = {3},
     PAGES = {205--239},
      ISSN = {0025-5831},
   MRCLASS = {14F05 (14D20)},
  MRNUMBER = {575939},
MRREVIEWER = {Klaus Hulek},
       DOI = {10.1007/BF01420526},
       URL = {https://doi.org/10.1007/BF01420526},
}

@incollection {DaskalopoulosWentworth,
    AUTHOR = {Daskalopoulos, Georgios D. and Wentworth, Richard A.},
     TITLE = {Geometric quantization for the moduli space of vector bundles
              with parabolic structure},
 BOOKTITLE = {Geometry, topology and physics ({C}ampinas, 1996)},
     PAGES = {119--155},
 PUBLISHER = {de Gruyter, Berlin},
      YEAR = {1997},
   MRCLASS = {32G13 (14D20 58F06)},
  MRNUMBER = {1605216},
MRREVIEWER = {Nitin Nitsure},
}

@ARTICLE{ASP16,
   author = {Andersen, J.~E. and Poulsen, Niccolo Skovgaard},
    title = "{The Curvature of the Hitchin Connection}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1609.01243},
 primaryClass = "math.DG",
 keywords = {Mathematics - Differential Geometry, 53C05},
     year = 2016,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160901243E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article {ZT88,
    AUTHOR = {Takhtajan, L. A. and Zograf, P. G.},
     TITLE = {The {S}elberg zeta function and a new {K}\"ahler metric on the
              moduli space of punctured {R}iemann surfaces},
   JOURNAL = {J. Geom. Phys.},
  FJOURNAL = {Journal of Geometry and Physics},
    VOLUME = {5},
      YEAR = {1988},
    NUMBER = {4},
     PAGES = {551--570 (1989)},
      ISSN = {0393-0440},
   MRCLASS = {58G26 (30F10 30F30 35G15 58G10)},
  MRNUMBER = {1075722},
MRREVIEWER = {V. V. Chueshev},
       DOI = {10.1016/0393-0440(88)90019-8},
       URL = {https://doi.org/10.1016/0393-0440(88)90019-8},
}

@article {ZT89,
    AUTHOR = {Takhtajan, L. A. and Zograf, P. G.},
     TITLE = {The geometry of moduli spaces of vector bundles over a
              {R}iemann surface},
   JOURNAL = {Izv. Akad. Nauk SSSR Ser. Mat.},
  FJOURNAL = {Izvestiya Akademii Nauk SSSR. Seriya Matematicheskaya},
    VOLUME = {53},
      YEAR = {1989},
    NUMBER = {4},
     PAGES = {753--770, 911},
      ISSN = {0373-2436},
   MRCLASS = {32L05 (14H15 32L15 32N05 53C55 58G05)},
  MRNUMBER = {1018746},
MRREVIEWER = {V. V. Chueshev},
       DOI = {10.1070/IM1990v035n01ABEH000687},
       URL = {https://doi.org/10.1070/IM1990v035n01ABEH000687},
}

@article {ZT91,
    AUTHOR = {Takhtajan, L. A. and Zograf, P. G.},
     TITLE = {A local index theorem for families of
              {$\overline\partial$}-operators on punctured {R}iemann
              surfaces and a new {K}\"ahler metric on their moduli spaces},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {137},
      YEAR = {1991},
    NUMBER = {2},
     PAGES = {399--426},
      ISSN = {0010-3616},
   MRCLASS = {58G10 (14H15 32G15 32L10 58G26)},
  MRNUMBER = {1101693},
MRREVIEWER = {V. V. Chueshev},
       URL = {http://projecteuclid.org/euclid.cmp/1104202624},
}

@article {ZT87,
    AUTHOR = {Takhtajan, L. A. and Zograf, P. G.},
     TITLE = {A local index theorem for families of
              {$\overline\partial$}-operators on {R}iemann surfaces},
   JOURNAL = {Uspekhi Mat. Nauk},
  FJOURNAL = {Akademiya Nauk SSSR i Moskovskoe Matematicheskoe Obshchestvo.
              Uspekhi Matematicheskikh Nauk},
    VOLUME = {42},
      YEAR = {1987},
    NUMBER = {6(258)},
     PAGES = {133--150, 248},
      ISSN = {0042-1316},
   MRCLASS = {58G10 (32G15 32L10 58G05 81E30)},
  MRNUMBER = {933998},
MRREVIEWER = {P. A. Kuchment},
}

@article {BdMS,
    AUTHOR = {Boutet de Monvel, L. and Sj\"ostrand, J.},
     TITLE = {Sur la singularit 'e des noyaux de {B}ergman et de {S}zegö},
 BOOKTITLE = {Journ\'ees: \'Equations aux {D}\'eriv\'ees {P}artielles de {R}ennes
              (1975)},
     PAGES = {123--164. Ast\'erisque, No. 34-35},
 PUBLISHER = {Soc. Math. France, Paris},
      YEAR = {1976},
   MRCLASS = {32H10 (35H05 35N99)},
  MRNUMBER = {0590106},
}

@book {BdMG,
    AUTHOR = {Boutet de Monvel, L. and Guillemin, V.},
     TITLE = {The spectral theory of {T}oeplitz operators},
    SERIES = {Annals of Mathematics Studies},
    VOLUME = {99},
 PUBLISHER = {Princeton University Press, Princeton, NJ; University of Tokyo
              Press, Tokyo},
      YEAR = {1981},
     PAGES = {v+161},
      ISBN = {0-691-08284-7; 0-691-08279-0},
   MRCLASS = {58G15 (32F20 35Pxx 35S05 47B35)},
  MRNUMBER = {620794},
MRREVIEWER = {V. Peller},
       DOI = {10.1515/9781400881444},
       URL = {https://doi.org/10.1515/9781400881444},
}

@article {Loi,
    AUTHOR = {Loi, Andrea},
     TITLE = {A {L}aplace integral on a {K}\"ahler manifold and {C}alabi's
              diastasis function},
   JOURNAL = {Differential Geom. Appl.},
  FJOURNAL = {Differential Geometry and its Applications},
    VOLUME = {23},
      YEAR = {2005},
    NUMBER = {1},
     PAGES = {55--66},
      ISSN = {0926-2245},
   MRCLASS = {53D50 (53C55 58J37)},
  MRNUMBER = {2148910},
MRREVIEWER = {Miroslav Engli\v s},
       DOI = {10.1016/j.difgeo.2005.03.005},
       URL = {https://doi.org/10.1016/j.difgeo.2005.03.005},
}

@article {Laurent10,
    AUTHOR = {Charles, Laurent},
     TITLE = {A {L}efschetz fixed point formula for symplectomorphisms},
   JOURNAL = {J. Geom. Phys.},
  FJOURNAL = {Journal of Geometry and Physics},
    VOLUME = {60},
      YEAR = {2010},
    NUMBER = {12},
     PAGES = {1890--1902},
      ISSN = {0393-0440},
   MRCLASS = {53D50 (53D12 58J20)},
  MRNUMBER = {2735276},
MRREVIEWER = {Miroslav Engli\v s},
       DOI = {10.1016/j.geomphys.2010.07.002},
       URL = {https://doi.org/10.1016/j.geomphys.2010.07.002},
}


@article {Varchenko,
    AUTHOR = {Var\v cenko, A. N.},
     TITLE = {Newton polyhedra and estimates of oscillatory integrals},
   JOURNAL = {Funkcional. Anal. i Prilo\v zen.},
  FJOURNAL = {Akademija Nauk SSSR. Funkcional\cprime nyi Analiz i ego Prilo\v zenija},
    VOLUME = {10},
      YEAR = {1976},
    NUMBER = {3},
     PAGES = {13--38},
      ISSN = {0374-1990},
   MRCLASS = {14B05 (14D05)},
  MRNUMBER = {0422257},
MRREVIEWER = {Helmut Hamm},
}

@article {VaVassiliev,
    AUTHOR = {Vasil'ev, V. A.},
     TITLE = {Asymptotic behavior of exponential integrals in the complex
              domain},
   JOURNAL = {Funktsional. Anal. i Prilozhen.},
  FJOURNAL = {Akademiya Nauk SSSR. Funktsional\cprime ny\u\i \ Analiz i ego
              Prilozheniya},
    VOLUME = {13},
      YEAR = {1979},
    NUMBER = {4},
     PAGES = {1--12, 96},
      ISSN = {0374-1990},
   MRCLASS = {41A60 (32C40 58C27)},
  MRNUMBER = {554406},
MRREVIEWER = {H. Tornehave},
}

@article {Quillen85,
    AUTHOR = {Quillen, D.},
     TITLE = {Determinants of {C}auchy-{R}iemann operators on {R}iemann
              surfaces},
   JOURNAL = {Funktsional. Anal. i Prilozhen.},
  FJOURNAL = {Akademiya Nauk SSSR. Funktsional\cprime ny\u\i \ Analiz i ego
              Prilozheniya},
    VOLUME = {19},
      YEAR = {1985},
    NUMBER = {1},
     PAGES = {37--41, 96},
      ISSN = {0374-1990},
   MRCLASS = {32F99 (58G99)},
  MRNUMBER = {783704},
MRREVIEWER = {Harold P. Boas},
}

\bibitem[AR18]{AR} J\o{}rgen~Ellegaard Andersen and Kenneth Rasmussen.
\newblock A Hitchin connection for a large class of families of K\"{a}hler structures,
\newblock {\em Proceedings of Hitchin70}, Oxford University Press, 2017

@article {AR,
    AUTHOR = {Andersen, J.~E. and Rasmussen, K.},
     TITLE = {A Hitchin connection for a large class of families of K\"{a}hler structures},
   JOURNAL = {Proceedings of Hitchin70},
   PUBLISHER = {Oxford University Press},
   YEAR = {2017}
}

@article {Goldman97,
    AUTHOR = {Goldman, William M.},
     TITLE = {Ergodic theory on moduli spaces},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {146},
      YEAR = {1997},
    NUMBER = {3},
     PAGES = {475--507},
      ISSN = {0003-486X},
   MRCLASS = {58D29 (57M99 58F11)},
  MRNUMBER = {1491446},
MRREVIEWER = {Ambar N. Sengupta},
       URL = {https://doi.org/10.2307/2952454},
}

@article {Penner88,
    AUTHOR = {Penner, Robert C.},
     TITLE = {A construction of pseudo-{A}nosov homeomorphisms},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {310},
      YEAR = {1988},
    NUMBER = {1},
     PAGES = {179--197},
      ISSN = {0002-9947},
   MRCLASS = {57N05 (20F34 58F15)},
  MRNUMBER = {930079},
MRREVIEWER = {William Dunbar},
       URL = {https://doi.org/10.2307/2001116},
}

@article {Brown08,
    AUTHOR = {Brown, Richard J.},
     TITLE = {Anosov mapping class actions on the {$\text{
              SU}(2)$}-representation variety of a punctured torus},
   JOURNAL = {Ergodic Theory Dynam. Systems},
  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {18},
      YEAR = {1998},
    NUMBER = {3},
     PAGES = {539--554},
      ISSN = {0143-3857},
   MRCLASS = {58F15 (57S15 58D29 58F11 58F27)},
  MRNUMBER = {1631712},
MRREVIEWER = {Jonathan A. Poritz},
       URL = {https://doi.org/10.1017/S0143385798108258},
}

@article {BordemannMeinrenken,
    AUTHOR = {Bordemann, M. and Meinrenken, E. and Schlichenmaier,
              M.},
     TITLE = {Toeplitz quantization of {K}\"ahler manifolds and {$\text{gl}(N)$}, {$N\to\infty$} limits},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {165},
      YEAR = {1994},
    NUMBER = {2},
     PAGES = {281--296},
      ISSN = {0010-3616},
   MRCLASS = {58F06 (32C17 32J27 47B35 81S10)},
  MRNUMBER = {1301849},
MRREVIEWER = {Albert Jeu-Liang Sheu},
       URL = {http://projecteuclid.org/euclid.cmp/1104271132},
}

@article {Charles16,
    AUTHOR = {Charles, Laurent},
     TITLE = {Asymptotic properties of the quantum representations of the
              mapping class group},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {368},
      YEAR = {2016},
    NUMBER = {10},
     PAGES = {7507--7531},
      ISSN = {0002-9947},
   MRCLASS = {57N05 (14D21 53D30)},
  MRNUMBER = {3471099},
MRREVIEWER = {Weiyi Zhang},
       DOI = {10.1090/tran6680},
       URL = {http://dx.doi.org/10.1090/tran6680},
}

@incollection {Schlichenmaier2000,
    AUTHOR = {Schlichenmaier, M.},
     TITLE = {Deformation quantization of compact {K}\"ahler manifolds by
              {B}erezin-{T}oeplitz quantization},
 BOOKTITLE = {Conf\'erence {M}osh\'e {F}lato 1999, {V}ol. {II} ({D}ijon)},
    SERIES = {Math. Phys. Stud.},
    VOLUME = {22},
     PAGES = {289--306},
 PUBLISHER = {Kluwer Acad. Publ., Dordrecht},
      YEAR = {2000},
   MRCLASS = {53D55 (32Q15 53C55 53D50)},
  MRNUMBER = {1805922},
MRREVIEWER = {Naoya Miyazaki},
}

@incollection {Schlichenmaier2001,
    AUTHOR = {Schlichenmaier, M.},
     TITLE = {Berezin-{T}oeplitz quantization and {B}erezin transform},
 BOOKTITLE = {Long time behaviour of classical and quantum systems
              ({B}ologna, 1999)},
    SERIES = {Ser. Concr. Appl. Math.},
    VOLUME = {1},
     PAGES = {271--287},
 PUBLISHER = {World Sci. Publ., River Edge, NJ},
      YEAR = {2001},
   MRCLASS = {53D55 (32Q15 53D50)},
  MRNUMBER = {1852228},
MRREVIEWER = {Naoya Miyazaki},
       DOI = {10.1142/9789812794598_0015},
       URL = {http://dx.doi.org/10.1142/9789812794598_0015},
}


@article {Goldman84,
    AUTHOR = {Goldman, William M.},
     TITLE = {The symplectic nature of fundamental groups of surfaces},
   JOURNAL = {Adv. in Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {54},
      YEAR = {1984},
    NUMBER = {2},
     PAGES = {200--225},
      ISSN = {0001-8708},
   MRCLASS = {32G15 (57M05)},
  MRNUMBER = {762512},
MRREVIEWER = {C. Earle},
       DOI = {10.1016/0001-8708(84)90040-9},
       URL = {http://dx.doi.org/10.1016/0001-8708(84)90040-9},
}

@article {AtiyahBott,
    AUTHOR = {Atiyah, M. F. and Bott, R.},
     TITLE = {The {Y}ang-{M}ills equations over {R}iemann surfaces},
   JOURNAL = {Philos. Trans. Roy. Soc. London Ser. A},
  FJOURNAL = {Philosophical Transactions of the Royal Society of London.
              Series A. Mathematical and Physical Sciences},
    VOLUME = {308},
      YEAR = {1983},
    NUMBER = {1505},
     PAGES = {523--615},
      ISSN = {0080-4614},
   MRCLASS = {14F05 (14D22 32G13 32L05 53C05 58E05 58E20 81E13)},
  MRNUMBER = {702806},
MRREVIEWER = {Martin A. Guest},
       DOI = {10.1098/rsta.1983.0017},
       URL = {http://dx.doi.org/10.1098/rsta.1983.0017},
}

@article {Andersen12Crelle,
    AUTHOR = {Andersen, J.~E.},
     TITLE = {The {W}itten-{R}eshetikhin-{T}uraev invariants of finite order
              mapping tori {I}},
   JOURNAL = {J. Reine Angew. Math.},
  FJOURNAL = {Journal f\"ur die Reine und Angewandte Mathematik. [Crelle's
              Journal]},
    VOLUME = {681},
      YEAR = {2013},
     PAGES = {1--38},
      ISSN = {0075-4102},
   MRCLASS = {57M27 (11F23)},
  MRNUMBER = {3181488},
MRREVIEWER = {Kazuhiro Hikami},
       DOI = {10.1515/crelle-2012-0033},
       URL = {http://dx.doi.org/10.1515/crelle-2012-0033},
}

@article {BaumFultonMacPherson,
    AUTHOR = {Baum, Paul and Fulton, William and MacPherson, Robert},
     TITLE = {Riemann-{R}och and topological {$K$}\ theory for singular
              varieties},
   JOURNAL = {Acta Math.},
  FJOURNAL = {Acta Mathematica},
    VOLUME = {143},
      YEAR = {1979},
    NUMBER = {3-4},
     PAGES = {155--192},
      ISSN = {0001-5962},
   MRCLASS = {14F12 (14C40)},
  MRNUMBER = {549773},
MRREVIEWER = {Allen B. Altman},
       DOI = {10.1007/BF02392091},
       URL = {http://dx.doi.org/10.1007/BF02392091},
}

@article {BaumFultonQuartz,
    AUTHOR = {Baum, Paul and Fulton, William and Quart, George},
     TITLE = {Lefschetz-{R}iemann-{R}och for singular varieties},
   JOURNAL = {Acta Math.},
  FJOURNAL = {Acta Mathematica},
    VOLUME = {143},
      YEAR = {1979},
    NUMBER = {3-4},
     PAGES = {193--211},
      ISSN = {0001-5962},
   MRCLASS = {14F12 (14C40)},
  MRNUMBER = {549774},
MRREVIEWER = {Allen B. Altman},
       DOI = {10.1007/BF02392092},
       URL = {http://dx.doi.org/10.1007/BF02392092},
}

@book {JohnsonLapidus,
    AUTHOR = {Johnson, Gerald W. and Lapidus, Michel L.},
     TITLE = {The {F}eynman integral and {F}eynman's operational calculus},
    SERIES = {Oxford Mathematical Monographs},
      NOTE = {Oxford Science Publications},
 PUBLISHER = {The Clarendon Press, Oxford University Press, New York},
      YEAR = {2000},
     PAGES = {xviii+771},
      ISBN = {0-19-853574-0},
   MRCLASS = {58D30 (28C20 46G12 47D08 47N50 81-01 81S40)},
  MRNUMBER = {1771173},
MRREVIEWER = {Brian Jefferies},
}


@article{Andersen06,
    Author = {Andersen, J.~E.},
     Title = {Asymptotic faithfulness of the quantum $\text{SU}({N})$
              representations of the mapping class groups},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {163},
      YEAR = {2006},
    NUMBER = {1},
     PAGES = {347--368},
      ISSN = {0003-486X},
   MRCLASS = {53D50 (14D21 57M99)},
  MRNUMBER = {2195137},
MRREVIEWER = {Hans U. Boden},
       DOI = {10.4007/annals.2006.163.347},
       URL = {http://dx.doi.org/10.4007/annals.2006.163.347},
}


@article{Andersen06,
    Author = {Andersen, J.~E.},
     Title = {Asymptotic faithfulness of the quantum $\text{SU}({N})$
              representations of the mapping class groups},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {163},
      YEAR = {2006},
    NUMBER = {1},
     PAGES = {347--368},
      ISSN = {0003-486X},
   MRCLASS = {53D50 (14D21 57M99)},
  MRNUMBER = {2195137},
MRREVIEWER = {Hans U. Boden},
       DOI = {10.4007/annals.2006.163.347},
       URL = {http://dx.doi.org/10.4007/annals.2006.163.347},
}

@article{Andersen12,
    AUTHOR = {Andersen, J.~E.},
     TITLE = {Hitchin's connection, {T}oeplitz operators, and symmetry
              invariant deformation quantization},
   JOURNAL = {Quantum Topol.},
  FJOURNAL = {Quantum Topology},
    VOLUME = {3},
      YEAR = {2012},
    NUMBER = {3-4},
     PAGES = {293--325},
      ISSN = {1663-487X},
   MRCLASS = {53Dxx (47B35)},
  MRNUMBER = {2928087},

}

@ARTICLE{Andersen12Unitarity,
   author = {Andersen, J. E.},
    title = "{Mapping class group invariant unitarity of the Hitchin connection over Teichm$\backslash$``uller space}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1206.2635},
 primaryClass = "math.DG",
 keywords = {Mathematics - Differential Geometry, Mathematics - Quantum Algebra},
     year = 2012,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2012arXiv1206.2635E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Walker2006,
    AUTHOR = {Walker, Kevin},
     TITLE = {TQFT's version 1h},
   JOURNAL = {http://canyon23.net/math/tc.pdf},
}


@ARTICLE{AndersenGammelgaard14,
   author = {Andersen, J.~E. and {Leth Gammelgaard}, N.},
    title = "{The Hitchin-Witten Connection and Complex Quantum Chern-Simons Theory}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1409.1035},
 primaryClass = "math.DG",
 keywords = {Mathematics - Differential Geometry, Mathematics - Quantum Algebra},
     year = 2014,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1409.1035E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Andersen02,
Author={Andersen, J.~E.},
Title={The asymptotic expansion conjecture},
JOURNAL = {Geom. Topol. Monogr.},
FJOURNAL = {Geom. Topol. Monogr.} ,
    VOLUME = {4},
      YEAR = {2002},
      NUMBER ={1},
    NUMBER = {1},
     PAGES = {474-481},
}



@book {Arnold,
    AUTHOR = {Arnold, V. I. and Gusein-Zade, S. M. and Varchenko, A. N.},
     TITLE = {Singularities of differentiable maps. {V}olume 2},
    SERIES = {Modern Birkh\"auser Classics},
      NOTE = {Monodromy and asymptotics of integrals,
              Translated from the Russian by Hugh Porteous and revised by
              the authors and James Montaldi,
              Reprint of the 1988 translation},
 PUBLISHER = {Birkh\"auser/Springer, New York},
      YEAR = {2012},
     PAGES = {x+492},
      ISBN = {978-0-8176-8342-9},
   MRCLASS = {58K55 (32B15 32C05 32G10 32S40 58K10)},
  MRNUMBER = {2919697},
}

@article {Atiyah88,
    AUTHOR = {Atiyah, M.},
     TITLE = {Topological quantum field theories},
   JOURNAL = {Inst. Hautes \'Etudes Sci. Publ. Math.},
  FJOURNAL = {Institut des Hautes \'Etudes Scientifiques. Publications
              Math\'ematiques},
    NUMBER = {68},
      YEAR = {1988},
     PAGES = {175--186 (1989)},
      ISSN = {0073-8301},
   MRCLASS = {57R55 (58E15 81E13 81E40)},
  MRNUMBER = {1001453},
MRREVIEWER = {Matthias Blau},
       URL = {http://www.numdam.org/item?id=PMIHES_1988__68__175_0},
}

@article {Atiyah70,
    AUTHOR = {Atiyah, M. F.},
     TITLE = {Resolution of singularities and division of distributions},
   JOURNAL = {Comm. Pure Appl. Math.},
  FJOURNAL = {Communications on Pure and Applied Mathematics},
    VOLUME = {23},
      YEAR = {1970},
     PAGES = {145--150},
      ISSN = {0010-3640},
   MRCLASS = {46.40 (32.00)},
  MRNUMBER = {0256156},
MRREVIEWER = {C. P. Gupta},
       DOI = {10.1002/cpa.3160230202},
       URL = {https://doi.org/10.1002/cpa.3160230202},
}
@article {AJHM,
    AUTHOR = {Andersen, J.~E. and Himpel, Benjamin and J\o{}rgensen,
              S. F. and Martens, J: and McLellan, B.},
     TITLE = {The {W}itten-{R}eshetikhin-{T}uraev invariant for links in
              finite order mapping tori {I}},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {304},
      YEAR = {2017},
     PAGES = {131--178},
      ISSN = {0001-8708},
   MRCLASS = {57M27 (53D50 57R56)},
  MRNUMBER = {3558207},
MRREVIEWER = {Sergiy Koshkin},
       DOI = {10.1016/j.aim.2016.08.042},
       URL = {http://dx.doi.org/10.1016/j.aim.2016.08.042},
}

@article {AH,
    AUTHOR = {Andersen, J.~E. and Himpel, B.},
     TITLE = {The {W}itten-{R}eshetikhin-{T}uraev invariants of finite order
              mapping tori {II}},
   JOURNAL = {Quantum Topol.},
  FJOURNAL = {Quantum Topology},
    VOLUME = {3},
      YEAR = {2012},
    NUMBER = {3-4},
     PAGES = {377--421},
      ISSN = {1663-487X},
   MRCLASS = {57M27 (53D50 57R56 58J28 58J30)},
  MRNUMBER = {2928090},
MRREVIEWER = {Daniel D. Moskovich},
}

@article {AndersenGammelgaardRoed,
    AUTHOR = {Andersen, J.~E. and Gammelgaard, Niels Leth and
              Lauridsen, Magnus Roed},
     TITLE = {Hitchin's connection in metaplectic quantization},
   JOURNAL = {Quantum Topol.},
  FJOURNAL = {Quantum Topology},
    VOLUME = {3},
      YEAR = {2012},
    NUMBER = {3-4},
     PAGES = {327--357},
      ISSN = {1663-487X},
   MRCLASS = {53D50 (32Q55 53D18)},
  MRNUMBER = {2928088},
MRREVIEWER = {Martin Schlichenmaier},
}

@article {AU2,
    AUTHOR = {Andersen, J.~E. and Ueno, K.},
     TITLE = {Geometric construction of modular functors from conformal
              field theory},
   JOURNAL = {J. Knot Theory Ramifications},
  FJOURNAL = {Journal of Knot Theory and its Ramifications},
    VOLUME = {16},
      YEAR = {2007},
    NUMBER = {2},
     PAGES = {127--202},
      ISSN = {0218-2165},
   MRCLASS = {81T40 (57R56 81T45)},
  MRNUMBER = {2306213},
MRREVIEWER = {Stephen F. Sawin},
       DOI = {10.1142/S0218216507005233},
       URL = {http://dx.doi.org/10.1142/S0218216507005233},
}


@article {AU3,
    AUTHOR = {Andersen, J.~E. and Ueno, K.},
     TITLE = {Modular functors are determined by their genus zero data},
   JOURNAL = {Quantum Topol.},
  FJOURNAL = {Quantum Topology},
    VOLUME = {3},
      YEAR = {2012},
    NUMBER = {3-4},
     PAGES = {255--291},
      ISSN = {1663-487X},
   MRCLASS = {57R56},
  MRNUMBER = {2928086},
MRREVIEWER = {Jeffrey Giansiracusa},
}

@article {AU1,
    AUTHOR = {Andersen, J.~E. and Ueno, K.},
     TITLE = {Abelian conformal field theory and determinant bundles},
   JOURNAL = {Internat. J. Math.},
  FJOURNAL = {International Journal of Mathematics},
    VOLUME = {18},
      YEAR = {2007},
    NUMBER = {8},
     PAGES = {919--993},
      ISSN = {0129-167X},
   MRCLASS = {81T40 (57R56 81T45)},
  MRNUMBER = {2339577},
MRREVIEWER = {Stephen F. Sawin},
       DOI = {10.1142/S0129167X07004369},
       URL = {http://dx.doi.org/10.1142/S0129167X07004369},
}

@article {AU4,
    AUTHOR = {Andersen, J.~E. and Ueno, K.},
     TITLE = {Construction of the {W}itten-{R}eshetikhin-{T}uraev {TQFT}
              from conformal field theory},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {201},
      YEAR = {2015},
    NUMBER = {2},
     PAGES = {519--559},
      ISSN = {0020-9910},
   MRCLASS = {81T45 (57R56)},
  MRNUMBER = {3370620},
       DOI = {10.1007/s00222-014-0555-7},
       URL = {http://dx.doi.org/10.1007/s00222-014-0555-7},
}

@article {AP,
    AUTHOR = {{Andersen}, J. E. and {Petersen}, W. E.},
     TITLE = {Construction of Modular Functors from Modular Categories},
   JOURNAL = {Travaux mathematiques},
  FJOURNAL = {Travaux mathematiques},
    VOLUME = {25},
      YEAR = {2017},
    NUMBER = {1},
     PAGES = {147--211},
      
}

@article {ASP17,
    AUTHOR = {Andersen, J.~E. and Poulsen, Niccolo Skovgaard},
     TITLE = {Coordinates for the Universal Moduli Space of Holomorphic Vector Bundles},
   JOURNAL = {Travaux mathematiques},
  FJOURNAL = {Travaux mathematiques},
    VOLUME = {25},
      YEAR = {2017},
    NUMBER = {1},
     PAGES = {9--39},
      
}

@article {ASP18,
    AUTHOR = {Andersen, J.~E. and Poulsen, Niccolo Skovgaard},
     TITLE = {An explicit Ricci potential for the Universal Moduli Space of Vector Bundles},
   JOURNAL = {To appear in Asian Journal of Mathematic},
  FJOURNAL = {To appear in Asian Journal of Mathematic},
      YEAR = {2018},
  
      
}




@article {APW,
    AUTHOR = {Axelrod, S. and Della Pietra, S. and Witten, E.},
     TITLE = {Geometric quantization of {C}hern-{S}imons gauge theory},
   JOURNAL = {J. Differential Geom.},
  FJOURNAL = {Journal of Differential Geometry},
    VOLUME = {33},
      YEAR = {1991},
    NUMBER = {3},
     PAGES = {787--902},
      ISSN = {0022-040X},
   MRCLASS = {58F06 (14D20 32G13 58D27 81S10 81T40)},
  MRNUMBER = {1100212},
MRREVIEWER = {N. J. Hitchin},
       URL = {http://projecteuclid.org/euclid.jdg/1214446565},
}

@incollection {Baez,
    AUTHOR = {Baez, J. and Stay, M.},
     TITLE = {Physics, topology, logic and computation: a {R}osetta {S}tone},
 BOOKTITLE = {New structures for physics},
    SERIES = {Lecture Notes in Phys.},
    VOLUME = {813},
     PAGES = {95--172},
 PUBLISHER = {Springer, Heidelberg},
      YEAR = {2011},
   MRCLASS = {18D10 (03B40 03B80 68Q05 81P10 81P68)},
  MRNUMBER = {2767046},
MRREVIEWER = {Eric C. Rowell},
       DOI = {10.1007/978-3-642-12821-9_2},
       URL = {http://dx.doi.org/10.1007/978-3-642-12821-9_2},
}

@article {Blanchet00,
    AUTHOR = {Blanchet, C.},
     TITLE = {Hecke algebras, modular categories and {$3$}-manifolds quantum
              invariants},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {39},
      YEAR = {2000},
    NUMBER = {1},
     PAGES = {193--223},
      ISSN = {0040-9383},
   MRCLASS = {57M27 (17B37 18D10 57N10)},
  MRNUMBER = {1710999},
MRREVIEWER = {Justin D. Roberts},
       DOI = {10.1016/S0040-9383(98)00066-4},
       URL = {http://dx.doi.org/10.1016/S0040-9383(98)00066-4},
}


@article {BHMV95,
    AUTHOR = {Blanchet, C. and Habegger, N. and Masbaum, G. and Vogel, P.},
     TITLE = {Topological quantum field theories derived from the {K}auffman
              bracket},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {34},
      YEAR = {1995},
    NUMBER = {4},
     PAGES = {883--927},
      ISSN = {0040-9383},
   MRCLASS = {57N10 (57M25 81T40)},
  MRNUMBER = {1362791},
MRREVIEWER = {Justin D. Roberts},
       DOI = {10.1016/0040-9383(94)00051-4},
       URL = {http://dx.doi.org/10.1016/0040-9383(94)00051-4},
}

@article {BHMV92,
    AUTHOR = {Blanchet, C. and Habegger, N. and Masbaum, G. and Vogel, P.},
     TITLE = {Three-manifold invariants derived from the {K}auffman bracket},
   JOURNAL = {Topology},
  FJOURNAL = {Topology. An International Journal of Mathematics},
    VOLUME = {31},
      YEAR = {1992},
    NUMBER = {4},
     PAGES = {685--699},
      ISSN = {0040-9383},
   MRCLASS = {57M25 (57N10)},
  MRNUMBER = {1191373},
MRREVIEWER = {Christine Lescop},
       DOI = {10.1016/0040-9383(92)90002-Y},
       URL = {http://dx.doi.org/10.1016/0040-9383(92)90002-Y},
}

@article {Freed,
    AUTHOR = {Freed, D. S.},
     TITLE = {Classical {C}hern-{S}imons theory. {I}},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {113},
      YEAR = {1995},
    NUMBER = {2},
     PAGES = {237--303},
      ISSN = {0001-8708},
   MRCLASS = {58D29 (57R57 58D27 58Z05 81T13)},
  MRNUMBER = {1337109},
MRREVIEWER = {Jonathan A. Poritz},
       DOI = {10.1006/aima.1995.1039},
       URL = {http://dx.doi.org/10.1006/aima.1995.1039},
}



@book {Griffiths94,
    AUTHOR = {Griffiths, Phillip and Harris, Joseph},
     TITLE = {Principles of algebraic geometry},
    SERIES = {Wiley Classics Library},
      NOTE = {Reprint of the 1978 original},
 PUBLISHER = {John Wiley \& Sons, Inc., New York},
      YEAR = {1994},
     PAGES = {xiv+813},
      ISBN = {0-471-05059-8},
   MRCLASS = {14-01},
  MRNUMBER = {1288523},
       DOI = {10.1002/9781118032527},
       URL = {http://dx.doi.org/10.1002/9781118032527},
}
		
@book {ArocaHironakaVicente18,
    AUTHOR = {Aroca, J. M. and Hironaka, H. and Vicente, J.
              L.},
     TITLE = {Complex analytic desingularization},
      NOTE = {With a foreword by Bernard Teissier},
 PUBLISHER = {Springer, Tokyo},
      YEAR = {2018},
     PAGES = {xxix+330},
      ISBN = {978-4-431-70218-4; 978-4-431-49822-3},
   MRCLASS = {32S45 (32C15 32S65)},
  MRNUMBER = {3839324},
       DOI = {10.1007/978-4-431-49822-3},
       URL = {https://doi.org/10.1007/978-4-431-49822-3},
}


@article {Hironaka,
    AUTHOR = {Hironaka, Heisuke},
     TITLE = {Resolution of singularities of an algebraic variety over a
              field of characteristic zero. {I}, {II}},
   JOURNAL = {Ann. of Math. (2) {\textbf{79}} (1964), 109--203; ibid. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {79},
      YEAR = {1964},
     PAGES = {205--326},
      ISSN = {0003-486X},
   MRCLASS = {14.18},
  MRNUMBER = {0199184},
MRREVIEWER = {J. Giraud},
}

@article {Hitchin,
    AUTHOR = {Hitchin, N. J.},
     TITLE = {Flat connections and geometric quantization},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {131},
      YEAR = {1990},
    NUMBER = {2},
     PAGES = {347--380},
      ISSN = {0010-3616},
   MRCLASS = {32G15 (32G08 53C05 58F06)},
  MRNUMBER = {1065677},
MRREVIEWER = {Jan Segert},
       URL = {http://projecteuclid.org/euclid.cmp/1104200841},
}

@article {Hitchin87,
    AUTHOR = {Hitchin, N. J.},
     TITLE = {The self-duality equations on a {R}iemann surface},
   JOURNAL = {Proc. London Math. Soc. (3)},
  FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
    VOLUME = {55},
      YEAR = {1987},
    NUMBER = {1},
     PAGES = {59--126},
      ISSN = {0024-6115},
   MRCLASS = {32G13 (14F05 14H15 32L10 53C05 58E99 81E13)},
  MRNUMBER = {887284},
MRREVIEWER = {Mitsuhiro Itoh},
       DOI = {10.1112/plms/s3-55.1.59},
       URL = {http://dx.doi.org/10.1112/plms/s3-55.1.59},
}

@book {H,
    AUTHOR = {Hormander, L.},
     TITLE = {The analysis of linear partial differential operators. {I}},
    SERIES = {Classics in Mathematics},
      NOTE = {Distribution theory and Fourier analysis,
              Reprint of the second (1990) edition [Springer, Berlin;
              MR1065993 (91m:35001a)]},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {2003},
     PAGES = {x+440},
      ISBN = {3-540-00662-1},
   MRCLASS = {35-02},
  MRNUMBER = {1996773},
       DOI = {10.1007/978-3-642-61497-2},
       URL = {http://dx.doi.org/10.1007/978-3-642-61497-2},
}

@article {Jean-Quartier,
    AUTHOR = {Jeanquartier, P.},
     TITLE = {D\'eveloppement asymptotique de la distribution de {D}irac
              attach\'ee \`a une fonction analytique},
   JOURNAL = {C. R. Acad. Sci. Paris S\'er. A-B},
    VOLUME = {201},
      YEAR = {1970},
     PAGES = {A1159--A1161},
   MRCLASS = {58C99},
  MRNUMBER = {0420695},
}

@article {Jones,
    AUTHOR = {Jones, V. F. R.},
     TITLE = {Hecke algebra representations of braid groups and link
              polynomials},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {126},
      YEAR = {1987},
    NUMBER = {2},
     PAGES = {335--388},
      ISSN = {0003-486X},
   MRCLASS = {46L99 (20F36 22D25 46L35 46L55 57M25)},
  MRNUMBER = {908150},
MRREVIEWER = {Pierre de la Harpe},
       DOI = {10.2307/1971403},
       URL = {http://dx.doi.org/10.2307/1971403},
}

@article {La1,
    AUTHOR = {Laszlo, Y.},
     TITLE = {Hitchin's and {WZW} connections are the same},
   JOURNAL = {J. Differential Geom.},
  FJOURNAL = {Journal of Differential Geometry},
    VOLUME = {49},
      YEAR = {1998},
    NUMBER = {3},
     PAGES = {547--576},
      ISSN = {0022-040X},
   MRCLASS = {14D20 (14D21 14H60)},
  MRNUMBER = {1669720},
MRREVIEWER = {Nitin Nitsure},
       URL = {http://projecteuclid.org/euclid.jdg/1214461110},
}

@book {JL,
    AUTHOR = {Johnson, Gerald W. and Lapidus, Michel L.},
     TITLE = {The {F}eynman integral and {F}eynman's operational calculus},
    SERIES = {Oxford Mathematical Monographs},
      NOTE = {Oxford Science Publications},
 PUBLISHER = {The Clarendon Press, Oxford University Press, New York},
      YEAR = {2000},
     PAGES = {xviii+771},
      ISBN = {0-19-853574-0},
   MRCLASS = {58D30 (28C20 46G12 47D08 47N50 81-01 81S40)},
  MRNUMBER = {1771173},
MRREVIEWER = {Brian Jefferies},
}

@book {Hansen,
    AUTHOR = {Hansen, S. K.},
     TITLE = {Reshetikhin-{T}uraev invariants of {S}eifert {3}-manifolds},
 PUBLISHER = {Aarhus University, Aarhus},
      YEAR = {2013},
}

@book {Joerg,
    AUTHOR = {J\o{}rgensen, S. F.},
     TITLE = {Semiclassical properties of the quantum representations of mapping class groups},
 PUBLISHER = {Aarhus University, Aarhus},
      YEAR = {2013},
}

@book {MacLane,
    AUTHOR = {Mac Lane, Saunders},
     TITLE = {Categories for the working mathematician},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {5},
   EDITION = {Second},
 PUBLISHER = {Springer-Verlag, New York},
      YEAR = {1998},
}

@article {Jeffrey,
    AUTHOR = {Jeffrey, Lisa C.},
     TITLE = {Chern-{S}imons-{W}itten invariants of lens spaces and torus
              bundles, and the semiclassical approximation},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {147},
      YEAR = {1992},
    NUMBER = {3},
     PAGES = {563--604},
      ISSN = {0010-3616},
   MRCLASS = {57R57 (11L03 57N10 58D29 58G10 58G18 58G26)},
  MRNUMBER = {1175494},
MRREVIEWER = {Ronald J. Stern},
       URL = {http://projecteuclid.org/euclid.cmp/1104250751},
}

@article {Malgrange,
    AUTHOR = {Malgrange, B.},
     TITLE = {Int\'egrales asymptotiques et monodromie},
   JOURNAL = {Ann. Sci. \'Ecole Norm. Sup. (4)},
  FJOURNAL = {Annales Scientifiques de l'\'Ecole Normale Sup\'erieure. Quatri\`eme
              S\'erie},
    VOLUME = {7},
      YEAR = {1974},
     PAGES = {405--430 (1975)},
      ISSN = {0012-9593},
   MRCLASS = {32C40},
  MRNUMBER = {0372243},
MRREVIEWER = {M. Sebastiani},
       URL = {http://www.numdam.org/item?id=ASENS_1974_4_7_3_405_0},
}

@article {NS,
    AUTHOR = {Narasimhan, M. S. and Seshadri, C. S.},
     TITLE = {Holomorphic vector bundles on a compact {R}iemann surface},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {155},
      YEAR = {1964},
     PAGES = {69--80},
      ISSN = {0025-5831},
   MRCLASS = {14.55 (32.50)},
  MRNUMBER = {0166799},
MRREVIEWER = {H. R\~A\P hrl},
       DOI = {10.1007/BF01350891},
       URL = {http://dx.doi.org/10.1007/BF01350891},
}


@article {KS01,
    AUTHOR = {Karabegov, A. V. and Schlichenmaier, M.},
     TITLE = {Identification of {B}erezin-{T}oeplitz deformation
              quantization},
   JOURNAL = {J. Reine Angew. Math.},
  FJOURNAL = {Journal f\"ur die Reine und Angewandte Mathematik. [Crelle's
              Journal]},
    VOLUME = {540},
      YEAR = {2001},
     PAGES = {49--76},
      ISSN = {0075-4102},
   MRCLASS = {53D55},
  MRNUMBER = {1868597},
MRREVIEWER = {Stefan Waldmann},
       DOI = {10.1515/crll.2001.086},
       URL = {http://dx.doi.org/10.1515/crll.2001.086},
}
@article {ReshetikhinTuraev90,
    AUTHOR = {Reshetikhin, N. Y. and Turaev, V. G.},
     TITLE = {Ribbon graphs and their invariants derived from quantum
              groups},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {127},
      YEAR = {1990},
    NUMBER = {1},
     PAGES = {1--26},
      ISSN = {0010-3616},
   MRCLASS = {57M25 (16W30 17B35)},
  MRNUMBER = {1036112},
MRREVIEWER = {Louis H. Kauffman},
       URL = {http://projecteuclid.org/euclid.cmp/1104180037},
}


@article {ReshetikhinTuraev91,
    AUTHOR = {Reshetikhin, N. Y. and Turaev, V. G.},
     TITLE = {Invariants of {$3$}-manifolds via link polynomials and quantum
              groups},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {103},
      YEAR = {1991},
    NUMBER = {3},
     PAGES = {547--597},
      ISSN = {0020-9910},
   MRCLASS = {57N10 (17B37 57M25 81R50)},
  MRNUMBER = {1091619},
MRREVIEWER = {Louis H. Kauffman},
       DOI = {10.1007/BF01239527},
       URL = {http://dx.doi.org/10.1007/BF01239527},
}

@book {Titchmarsh,
    AUTHOR = {Titchmarsh, E. C.},
     TITLE = {Introduction to the theory of {F}ourier integrals},
   EDITION = {Third},
 PUBLISHER = {Chelsea Publishing Co., New York},
      YEAR = {1986},
     PAGES = {x+394},
      ISBN = {0-8284-0324-4},
   MRCLASS = {42-03 (01A75)},
  MRNUMBER = {942661},
}


@book {Turaev,
    AUTHOR = {Turaev, V. G.},
     TITLE = {Quantum invariants of knots and 3-manifolds},
    SERIES = {De Gruyter Studies in Mathematics},
    VOLUME = {18},
   EDITION = {revised},
 PUBLISHER = {Walter de Gruyter \& Co., Berlin},
      YEAR = {2010},
     PAGES = {xii+592},
      ISBN = {978-3-11-022183-1},
   MRCLASS = {57M27 (57M25 57N10 57R56)},
  MRNUMBER = {2654259},
       DOI = {10.1515/9783110221848},
       URL = {http://dx.doi.org/10.1515/9783110221848},
}


@incollection {TUY,
    AUTHOR = {Tsuchiya, A. and Ueno, K. and Yamada, Y.},
     TITLE = {Conformal field theory on universal family of stable curves
              with gauge symmetries},
 BOOKTITLE = {Integrable systems in quantum field theory and statistical
              mechanics},
    SERIES = {Adv. Stud. Pure Math.},
    VOLUME = {19},
     PAGES = {459--566},
 PUBLISHER = {Academic Press, Boston, MA},
      YEAR = {1989},
   MRCLASS = {81T40 (14H15 17B67 17B81 32G15)},
  MRNUMBER = {1048605},
MRREVIEWER = {Yukihiko Namikawa},
}

@article {Wall69,
    AUTHOR = {Wall, C. T. C.},
     TITLE = {Non-additivity of the signature},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {7},
      YEAR = {1969},
     PAGES = {269--274},
      ISSN = {0020-9910},
   MRCLASS = {57.10},
  MRNUMBER = {0246311},
MRREVIEWER = {Ph. Tondeur},
       DOI = {10.1007/BF01404310},
       URL = {http://dx.doi.org/10.1007/BF01404310},
}

@book {Woodhouse,
    AUTHOR = {Woodhouse, N. M. J.},
     TITLE = {Geometric quantization},
    SERIES = {Oxford Mathematical Monographs},
   EDITION = {Second},
      NOTE = {Oxford Science Publications},
 PUBLISHER = {The Clarendon Press, Oxford University Press, New York},
      YEAR = {1992},
     PAGES = {xii+307},
      ISBN = {0-19-853673-9},
   MRCLASS = {58F06 (81S10)},
  MRNUMBER = {1183739},
MRREVIEWER = {P. L. Robinson},
}

@article {Witten,
    AUTHOR = {Witten, E.},
     TITLE = {Quantum field theory and the {J}ones polynomial},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {121},
      YEAR = {1989},
    NUMBER = {3},
     PAGES = {351--399},
      ISSN = {0010-3616},
   MRCLASS = {57M25 (17B67 57N10 58D15 58D30 81E40)},
  MRNUMBER = {990772},
MRREVIEWER = {Daniel S. Freed},
       URL = {http://projecteuclid.org/euclid.cmp/1104178138},
}

@article {Zelditch,
    AUTHOR = {Zelditch, S.},
     TITLE = {Szeg\"o kernels and a theorem of {T}ian},
   JOURNAL = {Internat. Math. Res. Notices},
  FJOURNAL = {International Mathematics Research Notices},
      YEAR = {1998},
    NUMBER = {6},
     PAGES = {317--331},
      ISSN = {1073-7928},
   MRCLASS = {32L10 (47B35)},
  MRNUMBER = {1616718},
MRREVIEWER = {Thierry Bouche},
       DOI = {10.1155/S107379289800021X},
       URL = {http://dx.doi.org/10.1155/S107379289800021X},
}






